Incentivizing Compliance with Algorithmic Instruments

Randomized experiments can be susceptible to selection bias due to potential non-compliance by the participants. While much of the existing work has studied compliance as a static behavior, we propose a game-theoretic model to study compliance as dynamic behavior that may change over time. In rounds, a social planner interacts with a sequence of heterogeneous agents who arrive with their unobserved private type that determines both their prior preferences across the actions (e.g., control and treatment) and their baseline rewards without taking any treatment. The planner provides each agent with a randomized recommendation that may alter their beliefs and their action selection. We develop a novel recommendation mechanism that views the planner's recommendation as a form of instrumental variable (IV) that only affects an agents' action selection, but not the observed rewards. We construct such IVs by carefully mapping the history -- the interactions between the planner and the previous agents -- to a random recommendation. Even though the initial agents may be completely non-compliant, our mechanism can incentivize compliance over time, thereby enabling the estimation of the treatment effect of each treatment, and minimizing the cumulative regret of the planner whose goal is to identify the optimal treatment.

==> beta-binominal.tex <==
\subsection{Beta-binomial Example}
\begin{example} (Beta-binomial Example)
Assume priors $\cP_1, \cP_2$ are independent across arms:
\begin{enumerate}
    \item $\cP_i: \theta^a \sim Beta(\alpha_i^a, \beta_i^a)$ with arm $a \in \{1,2\}$ and type $i \in \{1,2\}$; and
    \item Reward at round $t$ is $y_t \in \{0,1\}$; and 
    \item The prior mean reward of each arm $a$ for type $i$ is $\mu^a_i = \frac{\alpha_i^a}{\alpha_i^a + \beta_i^a}$
\end{enumerate}
Let the average reward of arm 1 in the first $L_2$ samples  be $\bar{y}^1 = \frac{1}{L_2} \sum_{t = 1}^{L_2} y^1_t$. Then, we have the posterior distribution for type $i$ of $\theta^1$ after observing $n$ samples is $Beta(\alpha + n\bar{y}^1, \beta_1 + n - n \bar{y}^1)$. Hence, the posterior mean reward of arm 1 for type $i$ is 
\begin{equation}
    \E_{\cP_i}[\theta^1 | S^{n}_1] = \frac{\alpha_i^1 + n \bar{y}^1}{\alpha_i^1 + \beta_i^1 + n}
\end{equation}
Then, we have if 
\begin{align*}
    &\quad\E[\theta^1 | S^{n}_1] < \mu^2_i\\
    &\Leftrightarrow \frac{\alpha_i^1 + n \bar{y}^1}{\alpha_i^1 + \beta_i^1 + n} < \mu^2_i\\
    &\Leftrightarrow \alpha_i^1 + n \bar{y}^1 < \mu^2_i (\alpha_i^1 + \beta_i^1 + n)\\
    &\Leftrightarrow n \bar{y}^1 < \mu^2_i \alpha_i^1 + \mu^2_i \beta_i^1 + \mu^2_i n - \alpha_i^1\\
    &\Leftrightarrow \bar{y}^1 < \mu^2_i - \frac{\alpha_i^1 - \mu^2_i (\alpha_i^1 + \beta_i^1)}{n}
\end{align*}
Hence, for $L_2 > \frac{\alpha_2^1 - \mu^2_2 (\alpha_2^1 + \beta_2^1)}{\mu^2_2}$, we have
\begin{align*}
    \Prob_{\cP_2}[\xi_2] &= \Prob_{\cP_2}[\E_{\cP_2}[\theta^1 | S_1^{L_2}] < \mu^2_2]\\
    &= \Prob_{\cP_2}\left[\bar{y}^1 < \mu^2_2 - \frac{\alpha_2^1 - \mu^2_2 (\alpha_2^1 + \beta_2^1)}{L_2} \right]\\
    &> 0
\end{align*}
In the first racing stage, only agents of type 2 comply with our recommendation for arm 2. Hence, when an agent of type 1 receives a recommendation for arm 2, this recommendation is not enough to convince them to take arm 2. Hence, we have
\begin{equation}
    \E_{\cP_1}[\theta^2 - \theta^1 | z_t = e_2] = \E_{\cP_i}[\theta^2 - \theta^1] < 0
\end{equation}
On the other hand, when an agent of type 2 receives a recommendation for arm 2, they would think that either arm 2 is definitely the best arm or the two arms are still racing against each other. Agents of type 2 know that the racing stage only starts when the social planner has collected sufficient samples of arm 2 in the sampling stage:
\begin{equation}
    L_2 \geq \frac{589824(\log(3T/\delta) + 3\log(2T(2 + \Upsilon^2)))}{\tau^2 (\Prob_{\cP_2}[\theta^2 - \theta^1 \geq \tau]^2)}
\end{equation}
and 
\begin{equation}
    \delta < \delta_{\tau, 2} = \frac{\tau \Prob_{\cP_2}[\theta^2 - \theta^1 \geq \tau]}{2 \tau \Prob_{\cP_2}[\theta^2 - \theta^1 \geq \tau] + 2} 
\end{equation}
The constant that the social planner needs to calculate is then $\tau \Prob_{\cP_2}[\theta^2 - \theta^1 \geq \tau]$ for some fixed constant $\tau \in [0,1]$.\\
Assume that we have beta-binomial priors. Hence, we have
\begin{equation}
    \Prob_{\cP_2}[\theta^2 - \theta^1 \geq \tau] = 1 - \Prob_{\cP_2}[\theta^2 - \theta^1 < \tau]
\end{equation}
\end{example}

==> control-treatment-nu.tex <==
\section{Setting Assumptions and Sampling Stage for Control-Treatment with Two Mixed-Preference Types}
\label{sec:two-arms-two-priors}
Assume that there are two types of agents. Let $p_i$ for $i\in\{0,1\}$ be the proportion of agents of type $i$ in the population. The types are \textit{mixed}, since agents of each type prefer different arms, i.e.
\begin{itemize}
    \item agents of type 0 initially prefer the control (arm 0), i.e. $\mu^0_0 > \mu^1_0$; and
    \item agents of type 1 initially prefer the treatment (arm 1), i.e. $\mu^0_1 < \mu^1_1$.
\end{itemize}

\swcomment{Can we say something about (1) both are always-takers and (2) handle more than two types (control-treatment with multiple types)?}



Our algorithm splits into two stages. First, in the sampling stage (\cref{alg:sampling-control-treatment}), we incentivize only type 0 agents to take all of our recommendations (see \cref{lemma:bic-sampling-control-treatment}). (Since they already prefer arm 0, the primary difficulty here is to incentivize them to take arm 1 when we recommend it.) We do so by recommending arm 0 as an ``exploitation'' arm most of the time and recommending arm 1 as an ``exploration'' arm with a low probability. Because we recommend the exploration arm with low probability, our instrument is weak and it takes a lot of rounds to get an IV estimate with a good approximation bound. So, once our approximation bound is good enough, we move to the second phase: the racing stage (\cref{alg:racing-two-types-mixed-preferences}). In the racing stage, we play Active Arms Elimination \cite{active-arms-elimination-2006} and recommend arms 0 and 1 sequentially in equal proportion. In the first part of this stage, only type 0 agents are compliant, insofar as they always follow our recommendations. Up until this point, agents of type 1 will always choose arm 1, regardless of what we recommend. However, in the second part of the racing stage, our estimate $\hat{\theta}$ is good enough so that all agents become compliant and follow our recommendations. Once one arm `wins,' we end the racing stage and recommend the winning arm for the remainder of the time horizon. At each stage, we get a confidence interval on the true treatment effect relative to our estimate $\hat{\theta}$ and approximation bound (given in \cref{thm:treatment-approximation-bound}).

\subsection{Sampling Stage for Control-Treatment with Two Mixed-Preference Types}
In the first phase of algorithm \ref{alg:sampling-control-treatment}, we let the agents pick their preferred arm. Hence, each agent chooses the better arm according to their prior: agents of types 0 will choose control (arm 0) while agents of type 1 will take treatment (arm 1). \lscomment{Is this true? It confers no information, but the agents don't necessarily know which stage of the algorithm they're in, so agents of type 3 might actually have a more complicated posterior based on which stage of the algorithm they believe they're in.} We observe the reward from these arm pulls. Assume that there are $\ell_0$ samples of arm 0 and $\ell_1$ samples of arm 1 observed in this phase. For a given type $i$, there is a non-zero chance that arm 0 performs so poorly that the posterior of arm 1 looks better than that of arm 0 conditioned on the observed samples. We define this event as 
\begin{equation}
    \xi_i = \left\{ \frac{1}{\ell_1} \sum_{t=1}^{\ell_1} y_t^1 - \frac{1}{\ell_0} \sum_{t=1}^{\ell_0} y_t^0 > 2\Upsilon + \sigma_\epsilon \sqrt{\frac{2\log(1/\delta)}{\ell_0}} + \sigma_\epsilon \sqrt{\frac{2\log(1/\delta)}{\ell_1}} + \frac{1}{2} + \nu   \right\} 
\end{equation}
where $\delta>0$ is a small failure probability and at round $t$, the term $y_t^a$ denotes the observed reward of taking arm $a$ at time $t$ (or no reward if arm $a$ is not observed at time $t$), i.e. $y_t^a = y_t\1[X_t=a]$.
  

\begin{algorithm}[H]
\SetAlgoLined
\SetKwInput{KwIn}{Input}
\KwIn{parameters $\rho, \ell_1 \in \mathbb{N}$ and $0<\delta<\delta'$, where $\delta':=\frac{\Prob_{\cP_0}[\xi_0]}{8}$}
In the first $\ell_0 + \ell_1$ rounds, let the agents pick their preferred arm. The sample average of control reward $y^0$ after $\ell_0$ pulls of arm $0$ is denoted $\bar{y}^0_{\ell_0}$. Similarly, the sample average of treatment reward $y^1$ after $\ell_1$ pulls of arm $1$ is denoted $\bar{y}^1_{\ell_1}$. After that, do the following:\\
    \eIf{$\displaystyle \bar{y}_{\ell_0}^0 - \bar{y}_{\ell_1}^1 > 2\Upsilon + \sigma_\epsilon \sqrt{\frac{2\log(1/\delta)}{\ell_0}} + \sigma_\epsilon \sqrt{\frac{2\log(1/\delta)}{\ell_1}} + \frac{1}{2} + \nu$}
    {$a^* = 0$} 
    {$a^* = 1$}
    From the set $P$ of the next $\ell_1.\rho$ agents, pick a set $Q$ of $\ell_1$ agents uniformly at random.\\
    Every agent $t \in P - Q$ is recommended arm $a^*$.\\
    Every agent $t \in Q$ is recommended arm 1.
    \caption{Sampling stage for control-treatment with two mixed-preference types}
    \label{alg:sampling-control-treatment}
\end{algorithm}

\begin{restatable}[Sampling Stage BIC for Type 0]{lemma}{bicsamplingcontroltreatment}\label{lemma:bic-sampling-control-treatment}
    \Cref{alg:sampling-control-treatment} with parameters $(\rho, \ell_0, \ell_1)$ completes in $\ell_1\rho + \ell_0 + \ell_1$ rounds. \Cref{alg:sampling-control-treatment} is BIC for all agents of type $0$ if we hold the assumption above and the parameters satisfy:
    %\vspace{-2cm}
    \begin{equation}
        \rho \geq 1 + \frac{4(\mu_0^0 - \mu_0^1 + \nu\Prob_{\cP_0}[\xi_0])}{\Prob_{\cP_0}[\xi_0]}.
    \end{equation}
\end{restatable}
For type 0, the \textit{fighting chance} event is given as
\begin{equation}
    \xi_0 = \left\{ \frac{1}{\ell_1} \sum_{t=1}^{\ell_1} y_t^1 - \frac{1}{\ell_0} \sum_{t=1}^{\ell_0} y_t^0 > 2\Upsilon + \sigma_\epsilon \sqrt{\frac{2\log(1/\delta)}{\ell_0}} + \sigma_\epsilon \sqrt{\frac{2\log(1/\delta)}{\ell_1}} + \frac{1}{2} + \nu  \right\} ,
\end{equation}
 and happens with probability at least $1-\delta$ for confidence $\delta > 0$.

\begin{proof}
    See \cref{sec:sampling-bic-proof} for a proof.
\end{proof}

\begin{restatable}[Sampling Stage Treatment Effect Confidence Interval]{theorem}{samplingestimationbound}\label{thm:sampling-estimation-bound}
    With $n$ total samples collected from \cref{alg:sampling-control-treatment} --run with exploration probability $\rho$ large enough so that our recommendations are BIC for type 0 agents (see \cref{lemma:bic-sampling-control-treatment}),-- we form an estimate $\theta_n$ of the treatment effect $\theta$. With probability at least $1-\delta$,
    \[\left|\hat{\theta}_n-\theta\right| \leq \frac{2\rho\left(\sigma_{\eps}+2\Upsilon\right)\sqrt{2n\log(5/\delta)}}{\left(np_0(1-1/\rho)-\sqrt{\frac{n(1-1/\rho)\log(5/\delta)}{2}}\right)}\]
\end{restatable}

\begin{proof}
    See \cref{sec:sampling-estimation-bound} for a proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Racing Stage and Regret Analysis}
We observe a set of $\rho \ell$ samples from the sampling stage. With large enough $\rho \ell$, we run the racing stage algorithm, which is a modification of the \textit{Active Arms Elimination}  algorithm \citep{active-arms-elimination-2006} with added BIC constraints, i.e. that agents of type 0 are compliant in the first part of the algorithm, then all agents in the second part. Finally, once an arm is found to be sub-optimal, it will be dropped from the race and the other arms ``wins''. To accelerate the sample collecting process, we employ the doubling trick \citep{besson2018doubling} to increase the phase length of the racing stage.

\subsection{Racing Stage for Control-Treatment with Two Mixed-Preference Types}
\begin{algorithm}[ht!]
\SetAlgoLined
\SetKwInput{KwIn}{Input}
\KwIn{samples $S_L:=\{x_i,z_i,y_i\}_1^L$ sampling stage sans the first phase $L \in \mathbb{N}$; time horizon $T$; minimum phase length $h$; probability $\delta$; and upper bound $\nu$ on cost function $\phi(u_t)$}
\KwIn{IV estimate of mean reward $\theta$, denoted $\hat{\theta}_L$ and approximation bound $s_L := \frac{\left(2\sigma_{\eps}+4\Upsilon\right)\sqrt{2L\log(4/\delta)}}{\left|\sum_{i=1}^L(x_i-\bar{x})(z_i-\bar{z})\right|}$ defined over samples $S_L$ from the sampling stage}
\lscomment{There was an error in the the approximation bound-- changed $2\Upsilon$ to $4\Upsilon$. Want to make sure that it's correct throughout the paper.}
    Let $\hat{\theta}_0:=\hat{\theta}_L$ and $s_0:=s_L$ and $S_0:=S_L$;\\
    Split the remainder into consecutive phases of $h2^q$ rounds each, starting $q=1$;\\
    \While{$\hat{\theta}_{q-1} \leq s_{q-1}$}
    {The next $h2^q$ agents are recommended both arms sequentially;\\
    For each arm $a \in \{0,1\}$, let $y^a_t$ be one sample reward of that arm in this phase;\\
    Let the samples gathered from round $q$ be denoted $S_q:=\{x_i,z_i,y_i\}_{L+h2^{q-1}}^{L+h2^q}$\\
    Define $S_q^{\text{BEST}}$ as the samples from the phase (including the sampling stage samples $S_L$) with the best approximation bound, i.e. $S_q^{\text{BEST}}=\argmin\limits_{S_r,\,0\leq\,r\leq\,q}\frac{2\left(\sigma_{\eps}+4\Upsilon\right)\sqrt{2|S_r|\log(4/\delta)}}{\left|\sum_{S_r}(x_i-\bar{x})(z_i-\bar{z})\right|}$;\\
    Define $\hat{\theta}_q$ and $s_q$ as the estimate and approximation bound defined over the best samples $S_q^{\text{BEST}}$;\\
    $q = q+1$;} 
    
    For all remaining agents recommend $a^*=\1\left[\hat{\theta}_q>0\right]$
    \caption{The racing stage for control-treatment with two mixed-preference types}
    \label{alg:racing-two-types-mixed-preferences}
\end{algorithm}

\begin{restatable}[Racing Stage BIC for Type 0]{lemma}{bicracingcontroltreatmentzero}\label{lemma:bic-racing-control-treatment-0}
    Fix some constant $\tau \in (0, 1)$. Remember that $\phi(u_t)\in[-\nu,\nu]$ for all $u_t$ and $\Prob_{\cP_0}[\theta>\tau]$ be the prior probability that $\theta>\tau$ for agents of type 0. Let the approximation bound $s_L$ after the sampling stage be \begin{equation}
        s_L:=\frac{\left(2\sigma_{\eps}+4\Upsilon\right)\sqrt{2L\log(4/\delta)}}{\left|\sum_{i=1}^L(x_i-\bar{x})(z_i-\bar{z})\right|}
        \leq\frac{\tau\Prob_{\cP_0}[\theta>\tau]}{4}-\frac{\nu}{2}.
    \end{equation} 
    Then, during the first phase of the racing stage, the recommendations from \cref{alg:racing-two-types-mixed-preferences} are BIC for agents of type 0.
\end{restatable}

\begin{proof}
    See \cref{sec:bic-racing-type-0} for a proof.
\end{proof}

\begin{restatable}[First Part Racing Stage Treatment Effect Confidence Interval]{theorem}{racingestimationboundfirst}\label{thm:racing-estimation-bound-first}
    With $n$ total samples collected from the first part of \cref{alg:racing-two-types-mixed-preferences} where the type 0 BIC criterion on the sampling stage approximation bound is met (see \cref{lemma:bic-racing-control-treatment-0}), form an estimate $\theta_n$ of the treatment effect $\theta$. With probability at least $1-\delta$,
    \[\left|\hat{\theta}_n-\theta\right| \leq \frac{8\left(\sigma_{\eps} + 2\Upsilon\right)\sqrt{2n\log(5/\delta)}}{np_0-\sqrt{n\log(5/\delta)}}\]
\end{restatable}

\begin{proof}
    See \cref{sec:racing-estimation-bound-first} for a proof.
\end{proof}

\begin{restatable}[Racing Stage BIC for Type 1]{lemma}{bicracingcontroltreatmentone}\label{lemma:bic-racing-control-treatment-1}
    Fix some constant $\tau \in (0, 1)$. Remember that $\phi(u_t)\in[-\nu,\nu]$ for all $u_t$ and $\Prob_{\cP_1}[\theta<-\tau]$ be the prior probability that $\theta<-\tau$ for agents of type 1. Let the approximation bound $s_{L_1}$ after the first racing stage be \begin{equation}
        s_{L_1}:=\frac{\left(2\sigma_{\eps}+4\Upsilon\right)\sqrt{2L_1\log(4/\delta)}}{\left|\sum_{i=1}^{L_1}(x_i-\bar{x})(z_i-\bar{z})\right|}
        \leq\frac{\tau\Prob_{\cP_1}[\theta < -\tau]}{4}-\frac{\nu}{2}.
    \end{equation} 
    Then, during the second part of the racing stage, the recommendations from \cref{alg:racing-two-types-mixed-preferences} are BIC for agents of type 1 (as well as for type 0).
\end{restatable}

\begin{proof}
    See \cref{sec:bic-racing-type-1} for a proof.
\end{proof}

\begin{restatable}[Second Part Racing Stage Treatment Effect Confidence Interval]{theorem}{racingestimationboundsecond}\label{thm:racing-estimation-bound-second}
    With $n$ total samples collected from the second part of \cref{alg:racing-two-types-mixed-preferences} where the BIC criterion for both types on the sampling stage approximation bound is met (see \cref{lemma:bic-racing-control-treatment-0,lemma:bic-racing-control-treatment-1}), form an estimate $\theta_n$ of the treatment effect $\theta$. With probability at least $1-\delta$,
    \[\left|\hat{\theta}_n-\theta\right| \leq \frac{8\left(\sigma_{\eps}+2\Upsilon\right)\sqrt{2n\log(5/\delta)}}{n}\]
\end{restatable}

\begin{proof}
    See \cref{sec:racing-estimation-bound-second} for a proof.
\end{proof}

\lsdelete{
\subsection{Regret Analysis}
The goal of this algorithm is to maximize the cumulative reward of all agents. We measure the algorithm's performance through the definition of regret. We are interested in minimizing the ex-post regret of the algorithm, which is the regret specific to a particular treatment effect $\theta$. Since the priors are not exactly known to the social planner, this ex-post regret is correct for any realization of the priors and treatment effect $\theta$. 
Our entire algorithm (with the sampling stage and the racing stage) achieves sub-linear ex-post regret. 
\begin{restatable}[Regret]{lemma}{expostregret}\label{lemma:expost-regret}
Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with sampling stage length parameters $\ell_1, \rho \in \NN$ achieves ex-post regret
\begin{equation}
R(T) \leq \ell_1 \rho + O(\sqrt{T\log T})
\end{equation}
where $\ell_1$ is the sampling stage's phase length and $1/\rho$ is the exploration probability in the sampling stage. 
\end{restatable}
% \begin{lemma} (Regret) 
% \label{lemma:expost-regret}
% Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves ex-post regret
% \begin{equation}
% R(T) \leq \ell_1 \rho + O(\sqrt{T\log T})
% \end{equation}
% where $\ell_1$ is the sampling stage's phase length and $1/\rho$ is the exploration probability in the sampling stage. 
% \end{lemma}
With similar analysis, we also achieve sub-linear expected regret over the randomness in the priors of the agents. Lemma \ref{lemma:expected-regret} provides a basic performance guarantee of our algorithm. 
\begin{restatable}[Expected Regret]{lemma}{expectedregret}\label{lemma:expected-regret}
Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves expected regret
\begin{align}
\E[R(T)] = O(\sqrt{T\log T})
\end{align}
\end{restatable}
% \begin{lemma} (Expected Regret)
% \label{lemma:expected-regret}
% Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves expected regret
% \begin{align}
% \E[R(T)] = O(\sqrt{T\log T})
% \end{align}
% \end{lemma}

These results are analyzed via standard technique and are comparable to the regret of the classic multi-armed bandit problem, with some added constants factors for the BIC constraints \cite{active-arms-elimination-2006}. Although the regret of our algorithm is the same as the fully incentive-compatible algorithm for both types, our algorithm can finish in a more timely manner and has smaller prior-dependent constants in the asymptotic bound.

From the analysis in Lemma \ref{lemma:expost-regret}, we can derive the type-specific regret for each type of agent. Since our algorithm does not guarantee that all agents follow our recommendation, this regret analysis is divided into two cases, depending on the best arm overall. With our assumption \ref{sec:assumptions-two-arms} that the proportions of each agent's type in the population are equal, Lemma \ref{lemma:type-specific-regret} below demonstrates the type-specific regret guarantee of our algorithm.
\begin{restatable}[Type-specific regret]{lemma}{typespecifictwoarms}\label{lemma:type-specific-regret}
Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves type-specific regrets in Table \ref{tab:type-specific-regret}.
\begin{table*}[ht]
    \centering
    \caption{Type-Specific Regret for Two Arms \& Two Types with partially BIC Algorithm}
    \begin{tabular}{ll}
    \toprule
    Best arm / Type     & Type-specific regret \\
    \midrule
    Arm 0 / Type 0     & $O\left(\frac{\log T }{(\tau \Prob_{\cP_0}[\theta \geq \tau] - \nu)^2} \right) + O(\sqrt{T\log T})$\\
    Arm 0 / Type 1      & $O\left(\frac{\log T}{(\tau \Prob_{\cP_0}[\theta \geq \tau] - \nu)^2} \right) + O\left(\frac{\log T}{(\tau\Prob_{\cP_1}[\theta < -\tau] - \nu)^2}\right) + O(\sqrt{T\log T})$ \\
    Arm 1 / Type 0      & $O\left(\frac{\log T}{(\tau \Prob_{\cP_0}[\theta \geq \tau] - \nu)^2}\right) +O(\sqrt{T\log T})$\\
    Arm 1 / Type 1      &  $O(\sqrt{T\log T})$ \\
    \bottomrule
    \end{tabular}
    
    \label{tab:type-specific-regret}
\end{table*}
\end{restatable}
We recall Lemma \ref{lemma:expost-regret}:
\expostregret*

\begin{proof}
From Theorem \ref{thm:treatment-approximation-bound}, the \textit{clean event} $\cC_1$ happens with probability at least $1 - \abs{\theta}$ for some $\abs{\theta} \in (0,1)$. Hence, the probability of $\neg \cC_1$ is at most $\abs{\theta}$. The probability of not getting an arm 1 sample in each phase, $\neg \cC_2$ is $\abs{\theta}'$. Hence, the expected ex-post regret conditional on $\neg \cC$ is at most $T (\abs{\theta} + \abs{\theta})'$.\\
Assume that $\cC$ holds. Observe that since $\cC$ holds, we have $\abs{\theta} \leq |\hat{\theta}_q| + s_q$ where $s_q$ is the decision threshold of phase $q$. Before the stopping criteria is invoked, we also have $|\hat{\theta}_q| \leq s_q$. Let $n$ be the number of samples used to estimate $\hat{\theta}_q$.
%This, combined with the fact that the number of recommendations $m$ equals the number of arms $k$, gives us that the empirical estimate $\hat{\Gamma}_t$ is the $m$-dimensional identity matrix at any round $t$. Thus, the minimum singular value $\sigma_{\min}(\hat{\Gamma}_t) = 1$. Then, during each iteration of the main loop, we have:
% \begin{align}
%     \abs{\theta} \leq 2 s_q &= 384\sqrt{\frac{\log(3T/\delta) + 3\log(2T(2+\Upsilon^2))}{q}}
%     \label{eq:delta-bound}
% \end{align}
Hence, we have: 
\begin{align*}
     &\quad\abs{\theta} \leq 2 s_q =  \frac{\left(16\sigma_{\eps}+16\Upsilon\right)\sqrt{2n\log(6T/\delta)}}{np_0-\sqrt{n\log(6T/\delta)}}\\
     \Rightarrow &\frac{\abs{\theta}}{16(\sigma_\epsilon + 2\Upsilon)\sqrt{2\log(6T/\delta)}} \leq \frac{1}{\sqrt{n} - \sqrt{\log(6T/\delta)}}\\
     \Rightarrow &n \leq \frac{512(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta}^2 p_0^2} + \frac{\log(6T/\delta)}{p_0^2}  + \frac{32\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{\abs{\theta} p_0^2}
\end{align*}
Therefore, the main loop must end by when the phase length is  
\begin{align*}
    n = \frac{512(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta}^2 p_0^2} + \frac{\log(6T/\delta)}{p_0^2}+ \frac{32\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{\abs{\theta} p_0^2}
\end{align*}
During the racing stage, each phase we give out $2h$ recommendations for the two arms sequentially, so each arm gets recommended $n/2$ times. If arm 0 is indeed the best arm, then on average, the regret for each phase is $0.75 n \abs{\theta}$. If arm 1 is the best arm, then on average, the regret for each phase is $0.25 n \abs{\theta}$. Conditional on event $\cC$, the arm $a^*$ at the end of the racing stage is the best arm so no more regret is collected after the racing stage is finished. Sine we are doubling the phase length after each phase, the total length of the racing stage is upper bounded by $2n$, where $n$ is the biggest phase length of the racing stage.  \\
Then, if arm 0 is the best arm, the total accumulated regret for the racing stage is 
\begin{align}
\label{eq:regret-arm-0}
    R_2(T) &\leq \frac{768(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta} p_0^2} + \frac{1.5\log(6T/\delta)\abs{\theta}}{p_0^2} + \frac{48\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{p_0^2}
\end{align}
On the other hand, if arm 1 is the best arm, the total accumulated regret for the racing stage is 
\begin{align}
\label{eq:regret-arm-1}
    R_2(T) &\leq \frac{256(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta} p_0^2} + \frac{0.5\log(6T/\delta) \abs{\theta}}{p_0^2} + \frac{16\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{p_0^2}
\end{align}
Observe that the ex-post regret for each round $t$ of the entire algorithm (both the sampling stage and the racing stage) is at most that of the racing stage plus $\abs{\theta}$ per each round of the sampling stage. Alternatively, we can also upper bound the regret by $\abs{\theta}$ per each round of the algorithm. Therefore, we can derive the ex-post regret for the entire algorithm:
If arm 0 is the best arm, then the total regret of both Algorithm
\ref{alg:sampling-control-treatment} and Algorithm \ref{alg:racing-two-types-mixed-preferences} is:
\begin{align}
    R(T) &\leq \min \Bigg \{L_1 \abs{\theta} + \frac{768(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta} p_0^2} + \frac{1.5\log(6T/\delta)\abs{\theta}}{p_0^2} \\
    &\hspace{2cm}+ \frac{48\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{p_0^2}, T\abs{\theta} \Bigg \}\\
    &\leq L_1 + O(\sqrt{T\log(T/\delta)}) 
\end{align}
If arm 1 is the best arm, then the total regret of both Algorithm 
\ref{alg:sampling-control-treatment} and Algorithm \ref{alg:racing-two-types-mixed-preferences} is:
\begin{align}
    R(T) &\leq \min \Bigg \{L_1 \rho \abs{\theta} + \frac{256(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta} p_0^2} + \frac{0.5\log(6T/\delta) \abs{\theta}}{p_0^2} \\
    &\hspace{2cm}+ \frac{16\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{p_0^2}, T\abs{\theta} \Bigg \}\\
    &\leq L_1 \rho + O(\sqrt{T\log(T/\delta)}) 
\end{align}
\end{proof}}

\input{regret}

==> control-treatment-sampling-stage-all-params.tex <==
\appendix
\onecolumn
\section{Supplementary Material}
\subsection{IV Estimator Proof for Control-Treatment Setting}
\label{sec:iv-estimator}
% \subsubsection{Finite Sample Analysis}
Recall that our reward model can be stated as the following equation:
\begin{equation}
    y_i = \theta x_i + g^{(u_i)}_i
\end{equation}

To analyze the Wald estimator, we introduce two conditional probabilities that an agent chooses the treatment given a recommendation $\hat{\gamma}_0$ and $\hat{\gamma}_1$, given as proportions over a set of $n$ samples $(x_i,z_i)_{i=1}^n$ and formally defined as
\begin{align*} \hat{\gamma}_0 = \hspace{-.15cm}\underset{(x_i,z_i)_{i=1}^n}{\hat{\Prob}}\hspace{-.3cm}[x_i = 1| z_i = 0] = \frac{\sum_{i=1}^n x_i(1-z_i)}{\sum_{i=1}^n (1-z_i)^2} \quad \text{and} \quad
    \hat{\gamma}_1 = \hspace{-.15cm}\underset{(x_i,z_i)_{i=1}^n}{\hat{\Prob}}\hspace{-.3cm}[x_i = 1| z_i = 1]  = \frac{\sum_{i=1}^n x_iz_i}{\sum_{i=1}^n z_i^2}
\end{align*}
Then, we can write the action choice $x_i$ as such:
\begin{align*}
    x_i 
    &= \hat{\gamma}_1 z_i + \hat{\gamma}_0 (1 - z_i) + \eta_i\\
    &= \hat{\gamma} z_i + \hat{\gamma}_0 + \eta_i
\end{align*}
where $\eta_i = x_i - \hat \gamma_1 z_i - \hat \gamma_0 (1 - z_i))$ and $\hat{\gamma} = \hat{\gamma}_1 - \hat{\gamma}_0$ is the in-sample \textit{compliance coefficient}. Now, we can rewrite the reward $y_i$ as 
\begin{align*}
    y_i &= \theta\left(\hat{\gamma} z_i + \hat{\gamma}_0 + \eta_i\right) + g^{(u_i)}_i\\
    &= \underbrace{\theta\,\hat{\gamma}}_{\beta} z_i + \theta \hat{\gamma}_0 + \theta \eta_i + g^{(u_i)}_i
\end{align*}
Let operator $\bar{\cdot}$ denote the sample mean, e.g. $\bar{y}:=\frac{1}{n}\sum_{i=1}^n y_i$ and $\bar{g}:=\frac{1}{n}\sum_{i=1}^n g^{(u_i)}_i$. $\bar{\eta} = \frac{1}{n}\sum_{i=1}^n \eta_i = 0$, by definition.

Then,
\begin{align*}
    \bar{y} &= \beta\bar{z} + \theta\hat{\gamma}_0 + \theta\bar{\eta} + \bar{g} + \bar{\epsilon}
\end{align*}
Thus, the centered reward and treatment choice at round $i$ are given as:
\begin{equation}
    \begin{cases}
    \label{eq:centered-reward-treatment-choice}
    y_i - \bar{y} = \theta(x_i-\bar{x}) + g^{(u_i)}_i-\bar{g}\\
    y_i - \bar{y} = \beta(z_i-\bar{z}) + \theta(\eta_i-\bar{\eta}) + g^{(u_i)}_i-\bar{g}\\
    x_i - \bar{x}_i = \hat{\gamma}(z_i-\bar{z}) + \eta_i-\bar{\eta}
    \end{cases}
\end{equation}
This formulation of the centered reward $y_i-\bar{y}$ allows us to express and bound the error between the treatment effect $\theta$ and its instrumental variable estimate $\hat{\theta}_n$, which we show in the following \Cref{thm:treatment-approximation-bound}.
% \subsubsection{Finite Sample Analysis}
\label{sec:approximation-bound-proof}

\treatmentapproximationbound*

\begin{proof}
Given a sample set $S=(x_i,y_i,z_i)_{i=1}^n$ of size $n$, we form an estimate of the treatment effect $\hat{\theta}_S$ via a Two-Stage Least Squares (2SLS). In the first stage, we regress $y_i-\bar{y}$ onto $z_i-\bar{z}$ to get the empirical estimate $\hat{\beta}_S$ and $x_i-\bar{x}$ onto $z_i-\bar{z}$ to get $\hat{\gamma}_S$ as such:
\begin{equation}
    \hat{\beta}_S := \frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (z_i -\bar{z})^2} \hspace{1cm}\text{and}\hspace{1cm} 
    \hat{\gamma}_S:= \frac{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})}{\sum_{i=1}^n (z_i -\bar{z})^2}
    \label{eq:beta-gamma-hat}
\end{equation}
In the second stage, we take the quotient of these two empirical estimates as the predicted treatment effect $\hat{\theta}_S$, i.e.
\begin{align}
    \hat{\theta}_S &= \frac{\hat{\beta}_S}{\hat{\gamma}_S} \nonumber\\
    &= \left(\frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (z_i -\bar{z})^2}\right) \left(\frac{\sum_{i=1}^n (z_i -\bar{z})^2}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})}\right) \nonumber\\
    &= \frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})}
\end{align}

Next, we can express the absolute value of the difference between the true treatment effect $\theta$ and the IV estimate of the treatment effect $\hat{\theta}_S$ given a sample set $S$ of size $n$ as such:
\begin{align}
    \left| \hat{\theta}_S - \theta \right|
    &= \left| \frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})} - \theta \right| \nonumber\\
    &= \left| \frac{\sum_{i=1}^n \left(\theta(x_i-\bar{x}) + g^{(u_i)}_i-\bar{g}\right)(z_i - \bar{z})}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})} - \theta \right| \tag{by \Cref{eq:centered-reward-treatment-choice}} \nonumber\\
    &= \left| \theta + \frac{\sum_{i=1}^n \left(g^{(u_i)}_i-\bar{g}\right)(z_i - \bar{z})}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})} - \theta \right| \nonumber\\
    &= \frac{\left|\sum_{i=1}^n \left(g^{(u_i)}_i-\bar{g}\right)(z_i - \bar{z})\right|}{\left|\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})\right|} \label{eq:last-line-estimator}
\end{align}


In order to complete our proof, we demonstrate an upper bound on the numerator $\displaystyle\left|\sum_{i=1}^n \left(g^{(u_i)}_i-\bar{g}\right)(z_i - \bar{z})\right|$ of \Cref{eq:last-line-estimator} in the last line above. We do so in \Cref{eq:approximation-bound-numerator}.
\end{proof}

\begin{lemma}\label{eq:approximation-bound-numerator}
For all $\delta \in (0,1)$, with probability at least $1-\delta$, we have
\begin{equation}
    \left|\sum_{i=1}^n \left(g^{(u_i)}_i-\bar{g}\right)(z_i - \bar{z})\right| \leq 2\sigma_{g}\sqrt{2n\log(2/\delta)}
\end{equation}
if \swedit{the set of $g^{(u_i)}_i$ are i.i.d. sub-Gaussian random variables with sub-Gaussian norm $\sigma_g$}.
\swdelete{
or
\begin{equation}
    \left|\sum_{i=1}^n \left(g^{(u_i)}_i-\bar{g}\right)(z_i - \bar{z})\right| \leq 4\Upsilon\sqrt{2n\log(2/\delta)}
\end{equation}
if $g^{(u_i)}_i$ is a bounded random variable, such that $|g^{(u_i)}_i|\leq\Upsilon$.}
\end{lemma}

\lscomment{Notationally, is $\E[g^{(u)}]$ fine or is $\E[g^{(u_i)}_i]$ preferred?}

\begin{proof} We can rewrite the left hand side as follows
    \begin{align*}
        &\left|\sum_{i=1}^n \left(g^{(u_i)}_i-\bar{g}\right)(z_i - \bar{z})\right|\\
        &= \left|\sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}] + \E[g^{(u)}]-\bar{g}\right)(z_i - \bar{z})\right|\\
        &= \left|\sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}]\right)z_i - \sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}]\right)\bar{z} + \sum_{i=1}^n \left(\E[g^{(u)}]-\bar{g}\right)(z_i - \bar{z})\right|\\
        &= \left|\sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}]\right)z_i - \sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}]\right)\bar{z}\right| \tag{since $\sum_{i=1}^n(z_i - \bar{z})=0$}\\
        &\leq \left|\sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}]\right)z_i\right| + \left|\sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}]\right)\right| \tag{by the triangle inequality and $|\bar{z}|\leq1$}
    \end{align*}
    Now, if $g^{(u_i)}_i$ is sub-Gaussian, then the last line in the system of inequalities above is given as:
    \begin{align*}  
        &\left|\sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}]\right)z_i\right| + \left|\sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}]\right)\right|\\
        &\ \leq \left|\sigma_g\sqrt{2n_1\log(1/\delta_1)}\right| + \left|\sigma_g\sqrt{2n\log(1/\delta_2)}\right| \tag{by Chernoff Bound, where $n_1:=\sum_{i=1}^nz_i$}\\
        &\ \leq 2\sigma_g\sqrt{2n\log(2/\delta)} \tag{since $n_1\leq\,n$ and by Union Bound, where $\delta_1 = \delta_2 = \delta/2$}
    \end{align*}
    
    This recovers the stated bound and finishes the proof for \Cref{thm:treatment-approximation-bound}. \swdelete{If $g^{(u_i)}_i$ is bounded by $\Upsilon$, i.e. $|g^{(u_i)}_i|\leq\Upsilon$, then:
    \begin{align*}  
        &\left|\sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}]\right)z_i\right| + \left|\sum_{i=1}^n \left(g^{(u_i)}_i-\E[g^{(u)}]\right)\right|\\
        &\ \leq \left|2\Upsilon\sqrt{\frac{n_1\log(1/\delta_1)}{2}}\right| + \left|2\Upsilon\sqrt{\frac{n\log(1/\delta_2)}{2}}\right| \tag{by Chernoff Bound, where $n_1:=\sum_{i=1}^nz_i$}\\
        &\ \leq 4\Upsilon\sqrt{\frac{n\log(2/\delta)}{2}} \tag{since $n_1\leq\,n$ and by Union Bound, where $\delta_1 = \delta_2 = \delta/2$}\\
        &\ \leq 4\Upsilon\sqrt{2n\log(2/\delta)} \tag{since $\frac{n\log(2/\delta)}{2} \leq 2n\log(2/\delta)$}
    \end{align*}}
\end{proof}

Next, we demonstrate a lower bound on the denominator of  \Cref{thm:treatment-approximation-bound}, in terms of the level of compliance at each phase of \Cref{alg:sampling-control-treatment,alg:racing-two-types-mixed-preferences}.

\begin{corollary}[Lower bound on $\left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|$]\label{thm:approximation-bound-denominator}
    Fix any phase. Let $p_c$ be the proportion in the population of agents who are compliant in this phase. Then, the denominator of the approximation bound given by the samples of this phase
    \[\left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right| \geq \begin{cases}
        n\bar{z}(1-\bar{z}) & \text{if the proportion $p_c=1$};\\
        \bar{z}\left(np_c(1-\bar{z})-\sqrt{\frac{n(1-\bar{z})\log(2/\delta)}{2}}\right) & \text{with probability at least $1-\delta$ otherwise}.
    \end{cases}\]
\end{corollary}
\begin{proof}
Fix any phase. Recall that $\bar{z}$ is the probability of recommending arm 1 in this phase. Also let $n_0$ and $n_1$ be the number of samples with agents of type 0 and type 1, respectively. Let $n_{0,0}$ be the number of samples with agents of type 0 with recommendations of arm 0.

\begin{align*}
    \left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|
    &= \left|\sum_{i=1}^n(x_i-\bar{x})z_i-\bar{z}\sum_{i=1}^n(x_i-\bar{x})\right|\\
    &= \left|\sum\limits_{i=1}^n(1-\bar{x})\1[z_i=1]-\bar{z}\sum_{i=1}^n(x_i-\bar{x})\right|\tag{type 0 agents always comply with  \Cref{alg:sampling-control-treatment,alg:racing-two-types-mixed-preferences} recommendations, i.e. $z_i=1\Rightarrow x_i=1$; otherwise, $z_i=0$}\\
    &= \left|\bar{z}n(1-\bar{x})-\bar{z}\sum_{i=1}^nx_i+\bar{z}\sum_{i=1}^n\bar{x}\right|\\
    &= \left|\bar{z}n-\bar{z}n\bar{x}+\bar{z}n\bar{x}-\bar{z}\sum_{i=1}^nx_i\right|\\
    &= \bar{z}\left|n-\sum_{i=1}^nx_i\right|\\
    &= \bar{z}n_{0,0}\\
\end{align*}

Now, we need to lower bound $n_{0,0}$. 
Let $p_c$ be the proportion in the population of agents who are compliant in this phase. Thus, in any round where the recommendation $z_i=0$, the probability that an agent takes the recommendation is $p_c$ and the expected value 
\[\E[n_{0,0}]=np_c(1-\bar{z}).\]

Now, there are two cases:
\begin{enumerate}
    \item If the proportion $p_c=1$, i.e. in a phase when our recommendation is compliant for all agents, then $n_{0,0}=\E[n_{0,0}]=n(1-\bar{z})$. In this case, the denominator \[\left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|=n\bar{z}(1-\bar{z})\]
    \item Otherwise, we may take a high probability bound on the number of agents $n_{0,0}$ that take our recommendation of arm 0. With probability at least $1-\delta$,
    \[n_{0,0} \geq np_c(1-\bar{z})-\sqrt{\frac{n(1-\bar{z})\log(2/\delta)}{2}}.\]

    Therefore, with probability at least $1-\delta$,
    \[\left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|\geq \bar{z}\left(np_c(1-\bar{z})-\sqrt{\frac{n(1-\bar{z})\log(2/\delta)}{2}}\right)\].
\end{enumerate}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Sampling Stage Proofs}
\subsubsection{Proof of \Cref{lemma:bic-sampling-control-treatment}: Type 0 Compliance with \Cref{alg:sampling-control-treatment}}\label{sec:sampling-bic-proof}
\bicsamplingcontroltreatment*
\begin{proof} This proof follows a similar structure to the Sampling Stage BIC proof in \cite{mansour2015bic}. We will prove that, when \Cref{alg:sampling-control-treatment} is initialized such that the exploration probability $\rho \leq 1 + \frac{\mu^{(0)}}{c_2\Prob_{\cP^{(0)}}[\xi]-\mu^{(0)}}$ and hyperparameters $c_1,c_2,c_3>0$ are chosen such that $(c_1-c_2)c_3>2$ and $c_3\delta'=\Prob_{\cP^{(0)}}[\xi]$, then agents of type 0 will comply with all recommendations in the second stage of \Cref{alg:sampling-control-treatment} (i.e. once the algorithm starts making meaningful recommendations). According to the selection function in \Cref{eq:control-treatment-selection-function}, if an agent $t$ expects the treatment effect $\theta$ to be positive, they will select the treatment $x_t=1$. Conversely, if they expect $\theta$ to be negative, they will select control $x_t=0$. Thus, proving compliance for type 0 agents entails proving that: 
\begin{enumerate}
    \item the expected treatment effect $\theta$ is non-negative according to the prior type $0$ when conditioned on a treatment recommendation $z_t=1$, i.e. $\displaystyle\E_{\cP^{(0)}}[\theta|z_t=1]\geq0$; and 
    \item the expected treatment effect $\theta$ is negative when recommended the control $z_t=0$, i.e. $\displaystyle\E_{\cP^{(0)}}[\theta|z_t=0]<0$.
\end{enumerate}

We first rewrite the expected values in (1) and (2) so that they are more manageable. Note that \Cref{alg:sampling-control-treatment} is designed in a such way that at any round $t$, there is a positive probability that the social planner recommends arm 1, i.e. $\Prob_{\cP^{(0)}}[z_t = 1] > 0$. Similarly, assume that the social also recommends arm 0 with positive probability, i.e. $\Prob_{\cP^{(0)}}[z_t = 0] > 0$. Thus, 
\begin{equation}
     \E_{\cP^{(0)}}[\theta|z_t=1]\geq0 \Leftrightarrow \E_{\cP^{(0)}}[\theta|z_t=1]\Prob_{\cP^{(0)}}[z_t=1]\geq0 
     \hspace{.25cm} \text{and} \hspace{.25cm}
     \E_{\cP^{(0)}}[\theta|z_t=0]<0 \Leftrightarrow \E_{\cP^{(0)}}[\theta|z_t=0]\Prob_{\cP^{(0)}}[z_t=0]<0.
\end{equation}

Rewritten as such, now \Cref{claim:bic-equiv} shows that (1) entails (2). Then, the rest of the proof is devoted to demonstrating (1). \lscomment{Maybe a little more outlining as to how the rest goes.}

\begin{claim}
\label{claim:bic-equiv} For any agent $t$ of type 0 in the second stage of \Cref{alg:sampling-control-treatment}, if the expected value of the treatment effect given a treatment recommendation is non-negative, then the expected value of the treatment effect given a control recommendation must be negative. Formally: $\left\{ \E_{\cP^{(0)}}[\theta|z_t = 1]\Prob_{\cP^{(0)}}[z_t = 1] \geq 0\right\}  \Rightarrow \left\{ \E_{\cP^{(0)}}[\theta|z_t = 0]\Prob_{\cP^{(0)}}[z_t = 0] < 0 \right\}$.
\end{claim}

\begin{proof}
Recall that we assume that type 0 agents prefer the control, i.e. the expected treatment effect $\displaystyle \E_{\cP^{(0)}}[\theta]< 0$. Then:
\begin{equation}
\label{eq:symmetry-proof-intermediate}
    0 > \E_{\cP^{(0)}}[\theta]
    = \E_{\cP^{(0)}}[\theta|z_t = 0]\Prob_{\cP^{(0)}}[z_t = 0] + \E_{\cP^{(0)}}[\theta|z_t = 1]\Prob_{\cP^{(0)}}[z_t = 1]
\end{equation}
Assume that $\displaystyle \E_{\cP^{(0)}}[\theta|z_t = 1]\Prob[z_t=1] \geq 0$. Thus, by \Cref{eq:symmetry-proof-intermediate}, it must be that $\displaystyle\E_{\cP^{(0)}}[\theta|z_t = 0]\Prob_{\cP^{(0)}}[z_t = 0] < 0$. Hence, $\left\{ \E_{\cP^{(0)}}[\theta|z_t = 1]\Prob_{\cP^{(0)}}[z_t = 1] \geq 0\right\}  \Rightarrow \left\{ \E_{\cP^{(0)}}[\theta|z_t = 0]\Prob_{\cP^{(0)}}[z_t = 0] < 0 \right\}$.
\end{proof}

In terms of the larger proof of \Cref{lemma:bic-sampling-control-treatment}, \Cref{claim:bic-equiv} means that showing that any agent $t$ of type 0 is compliant with the recommended treatment $z_t=1$ suffices to show that any agent $t$ of type 0 would be compliant with \textit{any} recommendation (control or treatment) in the second stage of \Cref{alg:sampling-control-treatment}.


Now, we devote the remainder of the proof to demonstrating that $\displaystyle\E_{\cP^{(0)}}[\theta|z_t = 1]\Prob_{\cP^{(0)}}[z_t = 1] \geq 0$, i.e. that for any agent $t$ of type 0, the expected treatment effect conditioned on recommendation $z_t=1$ from \Cref{alg:sampling-control-treatment} is non-negative.

Recall that for type 0, the following event $\xi$ happens with probability at least $1-\delta$ for any confidence $\delta\in(0,1)$:
\begin{equation}
    \xi = \left\{ \frac{1}{\ell_1} \sum_{t=1}^{\ell_1} y_t^1 - \frac{1}{\ell_0} \sum_{t=1}^{\ell_0} y_t^0 > \sigma_0 \sqrt{\frac{2\log(2/\delta)}{\ell_0}} + \sigma_1\sqrt{\frac{2\log(2/\delta)}{\ell_1}} + G^{(0)} + c_1 \right\},
\end{equation}
where $G^{(0)}$ is an upper bound on the difference between the prior mean of the treatment versus the control according to type $0$, i.e. $G^{(0)}>\E_{\cP^{(0)}}[g^{(1)}-g^{(0)}]$.


We first rewrite $\displaystyle\E_{\cP^{(0)}}[\theta | z_t = 1]$ in terms of the event $\xi$:
\begin{align}
&\quad	\E_{\cP^{(0)}}[\theta | z_t = 1]\Prob_{\cP^{(0)}}[z_t = 1] \nonumber\\
	&= \E_{\cP^{(0)}}[\theta |z_t = 1 \ \& \ t \not\in E]\Prob_{\cP^{(0)}}[z_t = 1 \ \& \ t \not\in E] + \E_{\cP^{(0)}}[\theta |z_t = 1 \ \& \ t \in E]\Prob_{\cP^{(0)}}[z_t = 1 \ \& \ t \in E] \tag{for explore set $E$} \nonumber\\
	&= \E_{\cP^{(0)}}[\theta |\xi \ \& \ t \not\in E]\Prob_{\cP^{(0)}}[\xi \ \& \ t \not\in E] + \E_{\cP^{(0)}}[\theta |z_t = 1 \ \& \ t \in E]\Prob_{\cP^{(0)}}[z_t = 1 \ \& \ t \in E] \tag{since the only way $z_t=1$ when exploiting ---i.e. when $t \not\in E$--- is when event $\xi$ occurs} \nonumber\\
	&= \E_{\cP^{(0)}}[\theta |\xi \ \& \ t \not\in E]\Prob_{\cP^{(0)}}[\xi \ \& \ t \not\in E] + \E_{\cP^{(0)}}[\theta |t\in E]\Prob_{\cP^{(0)}}[t \in E], \ \ \tag{$t \in E \Rightarrow z_t=1$ by definition of $E$} \nonumber\\
	&= \E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi]\Prob_{\cP^{(0)}}[t \not\in E] + \E_{\cP^{(0)}}[\theta]\Prob_{\cP^{(0)}}[t \in E] \tag{since $\theta \perp t \in E$ and $\xi\perp t \not\in E$} \nonumber\\
	&= (1 - \rho)\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi] + \rho\E_{\cP^{(0)}}[\theta] \tag{since agent $t \in E$ with probability $\rho$} \nonumber\\
	&= (1 - \rho)\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi] + \rho\mu^{(0)} \hspace{6cm}\text{(by definition, $\mu^{(0)}=\E_{\cP^{(0)}}[\theta]$)} \label{eq:part-1-compliance-proof-algo-1}
\end{align}
\lsdelete{For agents of type 0 to comply with the social planner's recommendation for arm 1, the number of phases $\rho$ (i.e. exploration probability $1/\rho$) needs to be chosen to satisfy the following inequality:
\begin{align}
    \E_{\cP^{(0)}}[\theta | z_t = 1] \Prob_{\cP^{(0)}}[z_t = 1] &\geq 0 \nonumber\\
	\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi]\left(1 - \rho \right) + \rho\mu^{(0)} &\geq 0 \tag{by \Cref{eq:part-1-compliance-proof-algo-1}} \nonumber\\
	\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi] - \rho\E_{\cP^{(0)}}[\theta |\xi] \Prob_{\cP^{(0)}}[\xi] + \rho\mu^{(0)} &\geq 0 \nonumber\\
	\rho\E_{\cP^{(0)}}[\theta |\xi]\Prob_{\cP^{(0)}}[\xi] &\geq \E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi] - \mu^{(0)} \nonumber\\
	\rho &\geq 1 - \frac{ \mu^{(0)}}{\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi]} \nonumber
	\label{eq:L-condition}
\end{align}
}%end of lsdelete

Following \Cref{eq:part-1-compliance-proof-algo-1}, we can rewrite our sought-after compliance condition $\displaystyle \E_{\cP^{(0)}}[\theta | z_t = 1] \Prob_{\cP^{(0)}}[z_t = 1] \geq 0$ as $\displaystyle 
(1 - \rho)\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi] + \rho\mu^{(0)} \geq 0$. Then, this allows us to rewrite this compliance condition strictly in terms of the exploration probability and relative to a number of constants which depend on the prior $\cP^{(0)}$. Thus, if we set $\rho$ to satisfy the following condition (in \Cref{eq:part-2-compliance-proof-algo-1}), then all agents of type 0 will comply with recommendations of \Cref{alg:sampling-control-treatment}:
\begin{align}
    \E_{\cP^{(0)}}[\theta | z_t = 1] \Prob_{\cP^{(0)}}[z_t = 1] &\geq 0 \nonumber\\
	(1 - \rho)\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi] + \rho\mu^{(0)} &\geq 0 \tag{by \Cref{eq:part-1-compliance-proof-algo-1}} \nonumber\\
	\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi] - \rho\E_{\cP^{(0)}}[\theta |\xi] \Prob_{\cP^{(0)}}[\xi] + \rho\mu^{(0)} &\geq 0 \nonumber\\
	 -\rho\E_{\cP^{(0)}}[\theta |\xi] \Prob_{\cP^{(0)}}[\xi] + \rho\mu^{(0)} &\geq -\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi] \nonumber\\
	 -\rho\left(\E_{\cP^{(0)}}[\theta |\xi] \Prob_{\cP^{(0)}}[\xi] - \mu^{(0)}\right) &\geq -\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi] \nonumber\\
	 \rho &\leq \frac{\E_{\cP^{(0)}}[\theta | \xi]\Prob_{\cP^{(0)}}[\xi]}{\E_{\cP^{(0)}}[\theta |\xi] \Prob_{\cP^{(0)}}[\xi] - \mu^{(0)}} \nonumber\\
	 \rho &\leq 1+\frac{\mu^{(0)}}{\E_{\cP^{(0)}}[\theta |\xi] \Prob_{\cP^{(0)}}[\xi] - \mu^{(0)}} \label{eq:part-2-compliance-proof-algo-1}
\end{align}
\lscomment{We can cut most lines above. It's just algebra.}

Now, we have rewritten the compliance condition to be expressed in terms of $\rho$ in \Cref{eq:part-2-compliance-proof-algo-1}. However, we may further simplify the right-hand side of to be expressed solely in terms of the probability $\Prob_{\cP^{(0)}}[\xi]$, which will complete our proof. Because type 0 agents prefer control, the prior expected treatment effect $\mu^{(0)}<0$. Thus, in order to find an upper bound on $\rho$, we must demonstrate that $\E_{\cP^{(0)}}[\theta | \xi]$ satisfies some lower bound in terms of some chosen parameters (namely, $c_2$).


First, given sets $S_0=(y^0)_{i=1}^{|S_0|}$ and $S_1=(y^1)_{i=1}^{|S_1|}$ which contain $|S_0|$ and $|S_1|$ samples of rewards from type 0 and type 1 agents in the first stage of \Cref{alg:sampling-control-treatment}, respectively, we define clean events that $|S_0|\geq\ell_0$ and $|S_1|\geq\ell_1$.

Depends on $p_0$ and $p_1$.




We define clean events $\cC_0$ and $\cC_1$ where the mean errors $\frac{1}{\ell_0}\sum_{i=1}^{\ell_0}g^{(u_i)}_i$ and $\frac{1}{\ell_1}\sum_{i=1}^{\ell_1}g^{(u_i)}_i$ are bounded (following \Cref{thm:high-prob-unbounded-chernoff}):
\begin{align}
     \cC_0 := \left \{ \frac{1}{\ell_0} \sum_{i=1}^{\ell_0} g^{(0)} \leq \sigma_0 \sqrt{\frac{2\log(1/\delta_1)}{\ell_0}} - \E_{\cP^{(0)}}[g^{(0)}]\right \}.\\
      \cC_1 := \left \{ \frac{1}{\ell_1} \sum_{i=1}^{\ell_1} g^{(1)}  \geq -\sigma_1 \sqrt{\frac{2\log(1/\delta_2)}{\ell_1}}- \E_{\cP^{(0)}}[g^{(1)}] \right \}.
\end{align}
Define another clean event $\cC$ where both $\cC_0$ and $\cC_1$ happen simultaneously. Letting $\delta_1=\delta_2=\delta/2$, the event $\cC$ occurs with probability at least $1 - \delta$ where  $\displaystyle \delta < \delta' := \frac{\Prob_{\cP^{(0)}}[\xi]}{c_3}$ for some carefully-chosen hyperparameter $c_3>0$. We can now rewrite $\E_{\cP^{(0)}}[\theta | \xi] \Prob_{\cP^{(0)}}[\xi]$ in terms of the clean event $\cC$ as such:

\lscomment{We also need some other clean event that we get $\ell_0$ and $\ell_1$ samples of control and treatment.}

\begin{align}
    \E_{\cP^{(0)}}[\theta | \xi] \Prob_{\cP^{(0)}}[\xi] &= \E_{\cP^{(0)}}[\theta | \xi, \cC] \Prob_{\cP^{(0)}}[\xi, \cC] + \E_{\cP^{(0)}}[\theta | \xi, \neg \cC] \Prob_{\cP^{(0)}}[\xi, \neg \cC] \nonumber\\
    &\geq \E_{\cP^{(0)}}[\theta | \xi, \cC] \Prob_{\cP^{(0)}}[\xi, \cC] - \delta \tag{since $\Prob_{\cP^{(0)}}[\neg \cC]<\delta$ and $\theta \geq -1$ by definition} \nonumber\\
    &= \E_{\cP^{(0)}}[\theta | \xi, \cC] \bigg(\Prob_{\cP^{(0)}}[\xi] - \Prob_{\cP^{(0)}}[\xi, \neg \cC]\bigg) - \delta \nonumber\\
    &\geq \E_{\cP^{(0)}}[\theta | \xi, \cC] \bigg(\Prob_{\cP^{(0)}}[\xi] - \Prob_{\cP^{(0)}}[\neg \cC]\bigg) - \delta \nonumber\\
    &\geq \E_{\cP^{(0)}}[\theta | \xi, \cC] \bigg(\Prob_{\cP^{(0)}}[\xi] - \delta\bigg) - \delta \nonumber\\
    &= \E_{\cP^{(0)}}[\theta | \xi, \cC] \Prob_{\cP^{(0)}}[\xi] - \delta\bigg(1 + \E_{\cP^{(0)}}[\theta | \xi, \cC]\bigg) \nonumber\\
    &\geq \E_{\cP^{(0)}}[\theta | \xi, \cC] \Prob_{\cP^{(0)}}[\xi] - 2\delta \hspace{3cm} \text{($\E_{\cP^{(0)}}[\theta | \xi, \cC]\leq1$ because $\theta\leq1$ by definition)} \label{eq:sampling-two-arm-clean-event}
\end{align}
\lscomment{We can cut down algebra above.}

This comes down to finding a lower bound on the denominator of the expression above. We can reduce the dependency of the denominator to a single prior-dependent constant $\Prob_{\cP^{(0)}}[\xi]$ if we lower bound the prior-dependent expected value $\E_{\cP^{(0)}}[\theta | \xi]$. That way, assuming we know the prior and can calculate the probability of event $\xi$, we can pick an appropriate exploration probability $\rho$ to satisfy the compliance condition for all agents of type $0$. Recall that event $\xi = \{ \bar{y}^0_{\ell_0} + B < \bar{y}^1_{\ell_1}\}$ where $B = \sigma_0\sqrt{\frac{2\log(2/\delta)}{\ell_0}} + \sigma_1\sqrt{\frac{2\log(2/\delta)}{\ell_1}} + G^{(0)} + c_1$ and $\displaystyle G^{(0)}>\E_{\cP^{(0)}}[g^{(1)}-g^{(0)}]$. Then, the expected value
\begin{align}
    &\quad \E_{\cP^{(0)}}[\theta | \xi, \cC] \nonumber\\
    &= \E_{\cP^{(0)}}\left[\theta \middle| \bar{y}^1_{\ell_1} > \bar{y}^0_{\ell_0} + \sigma_0\sqrt{\frac{2\log(2/\delta)}{\ell_0}} + \sigma_1\sqrt{\frac{2\log(2/\delta)}{\ell_1}} + G^{(0)} + c_1, \cC\right] \nonumber\\
    &= \E_{\cP^{(0)}}\left[\theta \middle| \frac{1}{\ell_1}\sum_{t=1}^{\ell_1}\theta + g^{(1)} > \frac{1}{\ell_0}\sum_{t=1}^{\ell_0}g^{(0)} + \sigma_0\sqrt{\frac{2\log(2/\delta)}{\ell_0}} + \sigma_1\sqrt{\frac{2\log(2/\delta)}{\ell_1}} + G^{(0)} + c_1, \cC\right] \nonumber\\
    &= \E_{\cP^{(0)}}\left[\theta \middle| \theta > \frac{1}{\ell_0}\sum_{t=1}^{\ell_0}g^{(0)} - \frac{1}{\ell_1}\sum_{t=1}^{\ell_1}\theta + g^{(1)} + \sigma_0\sqrt{\frac{2\log(2/\delta)}{\ell_0}} + \sigma_1\sqrt{\frac{2\log(2/\delta)}{\ell_1}} + G^{(0)} + c_1, \cC\right] \nonumber\\
    &= \E_{\cP^{(0)}}\left[\theta \middle| \theta > \sigma_0\sqrt{\frac{2\log(1/\delta_1)}{\ell_0}} - \E_{\cP^{(0)}}[g^{(0)}] - \sigma_1\sqrt{\frac{2\log(1/\delta_2)}{\ell_1}} + \E_{\cP^{(0)}}[g^{(1)}]\right.\nonumber\\
    & \hspace{6cm} \left. + \ \sigma_0\sqrt{\frac{2\log(2/\delta)}{\ell_0}} + \sigma_1\sqrt{\frac{2\log(2/\delta)}{\ell_1}} + G^{(0)} + c_1, \cC\right] \tag{by event $\cC$}\nonumber\\
    &= \E_{\cP^{(0)}}\left[\theta \middle| \theta > -\sigma_0\sqrt{\frac{2\log(2/\delta)}{\ell_0}} -\sigma_1\sqrt{\frac{2\log(2/\delta)}{\ell_1}} +\E_{\cP^{(0)}}[g^{(1)}-g^{(0)}] +\sigma_0\sqrt{\frac{2\log(2/\delta)}{\ell_0}} + \sigma_1\sqrt{\frac{2\log(2/\delta)}{\ell_1}} + G^{(0)} + c_1, \cC\right] \tag{where $\delta_1 = \delta_2 = \delta/2$ }\nonumber\\
    &= \E_{\cP^{(0)}}\left[\theta \middle| \theta > \E_{\cP^{(0)}}[g^{(1)}-g^{(0)}] + G^{(0)} + c_1, \cC\right]\nonumber\\
    &> \E_{\cP^{(0)}}\left[\theta \middle| \theta > \E_{\cP^{(0)}}[g^{(1)}-g^{(0)}] - \E_{\cP^{(0)}}[g^{(1)}-g^{(0)}] + c_1\right]\nonumber\\
    &> c_1 \label{eq:sampling-stage-two-arm-gap}
\end{align}
Hence, the term $\E_{\cP^{(0)}}[\theta | \xi] \Prob_{\cP^{(0)}}[\xi]$ satisfies the following lower bound:
\begin{align}
    \E_{\cP^{(0)}}[\theta | \xi] \Prob_{\cP^{(0)}}[\xi]
    &\geq \E_{\cP^{(0)}}[\theta | \xi, \cC']\Prob_{\cP^{(0)}}[\xi] - 2\delta \tag{by \Cref{eq:sampling-two-arm-clean-event}}\\
    &> c_1\Prob_{\cP^{(0)}}[\xi] - 2\delta \tag{by \Cref{eq:sampling-stage-two-arm-gap}}\\ 
    &= (c_1-c_2)\Prob_{\cP^{(0)}}[\xi] + c_2\Prob_{\cP^{(0)}}[\xi] - 2\delta\\
    &= (c_1-c_2)c_3\delta' - 2\delta + c_2\Prob_{\cP^{(0)}}[\xi] \tag{since $c_3\delta' = \Prob_{\cP^{(0)}}[\xi]$}\\
    &\geq (c_1c_3 - c_2c_3 - 2)\delta' + c_2\Prob_{\cP^{(0)}}[\xi] \tag{since $\delta < \delta'$}\\
    &\geq c_2\Prob_{\cP^{(0)}}[\xi] \tag{assuming we set $(c_1-c_2)c_3>2$}
\end{align}
Thus, if we set hyperparameters $c_1,c_2,c_3>0$ such that $c_3\delta'=\Prob_{\cP^{(0)}}[\xi]$ and $(c_1-c_2)c_3>2$, and ---plugging the lower bound on $\displaystyle\E_{\cP^{(0)}}[\theta | \xi] \Prob_{\cP^{(0)}}[\xi]$ into \Cref{eq:part-2-compliance-proof-algo-1}--- we set the exploration probability $\rho$:
\begin{align*}
    \rho &\leq 1 + \frac{\mu^{(0)}}{c_2\Prob_{\cP^{(0)}}[\xi]-\mu^{(0)}}
\end{align*}
then all agents of type 0 will comply in the second stage of \Cref{alg:sampling-control-treatment}.
\end{proof}

\lscomment{Previously, we set $c_1 = 1/2$. Now, we have more leeway to choose $\Prob_{\cP^{(0)}}[\xi]$ and $c_1$; but, if $c_1$ is smaller, then rho is bigger and vice versa.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Sampling Stage Treatment Effect Confidence Interval}
\lscomment{Fix this proof so the Union Bound is made more explicit and maybe change the phrase ``Estimation Bound.''}
\label{sec:sampling-estimation-bound}
\samplingestimationbound*
\begin{proof}
    Recall that the mean recommendation $\bar{z}=1/\rho$ in the sampling stage; the proportion of agents who are type 0 is $p_0$. We assume \Cref{alg:sampling-control-treatment} to be initialized with parameters (see \Cref{lemma:bic-sampling-control-treatment} for details) such that its recommendations are compliant for agents of type 0. Therefore, we may apply \Cref{thm:approximation-bound-denominator} where we let the proportion $p_c=p_0$. Finally, we combine the high probability bound on the denominator with the high probability bound on the numerator (given by \Cref{thm:treatment-approximation-bound}), taking a union bound to achieve the confidence parameters $\delta$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Racing Stage}
\subsubsection{Racing Stage Type 0 Compliant proof}
\label{sec:bic-racing-type-0}
\bicracingcontroltreatmentzero*
\begin{proof} 
Let the decision threshold $s_q$ for a phase $q$ be defined as in \Cref{alg:racing-two-types-mixed-preferences}. Assume that after the elimination, at every iteration a sample of the eliminated arm is also drawn, but not revealed to the agent.\\
We define the event $\cC_0$ as the accuracy guarantee of $\hat{\theta}$ such that:
\begin{equation}
\label{eq:event-C-1}
    \cC_0 := \left\{ \forall q \geq L: |\theta - \hat{\theta}_q| < s_q \right\}
\end{equation}
where $L$ is the number of samples after running the sampling stage.\\
Let $X^a_q$ be the number of arm $a\in\{0,1\}$ samples in phase $q$. The decision threshold $s_q$ in phase $q$ is unbounded if $X^a_q=0$ for either arm $a$. We also define event $\cC_1$ where there is at least one sample of each arm in each phase:
\begin{equation}
\label{eq:event-C-2}
    \cC_1 := \left\{\forall q\geq L,a: X^a_q \geq 1 \right\}
\end{equation}
Recall that $p_0$ of the population is of type $0$. Then, if \Cref{alg:racing-two-types-mixed-preferences} is compliant for all agents of type 0 and we recommend each arm at least $h$ times in phase $q$, we have $X^0_q>h$ and $X^0_q \sim B(h,p_0)$. Hence, we have
\begin{equation}
    \Prob[X^0_q \geq 1] = 1 - p_0^h = \delta'.
\end{equation}

Let $\tau\in(0,1)$. Fix phase $q\geq L$, and some agent $t$ in this phase. In order to prove that \Cref{alg:racing-two-types-mixed-preferences} is compliant for all agents of type 0, we want to show that 
\begin{equation}
    \label{eq:racing-bic-type0}
    \E_{\cP_0}[\theta\vert z_t=1]\Prob_{\cP_0}[z_t=1] \geq 0.
\end{equation}

Note that, by assumption, the parameter
\begin{align*}
    h &\geq \frac{\log\left(\frac{3\tau\Prob_{\cP_0}[\theta\geq\tau]+4}{4\tau\Prob_{\cP_0}[\theta\geq\tau]+4}\right)}{\log(1-p_2)}\\
    \Rightarrow \left(\frac{1}{2}
    \right)^h 
    &\geq \frac{3\tau\Prob_{\cP_0}[\theta\geq\tau]+4}{4\tau\Prob_{\cP_0}[\theta\geq\tau]+4}\\
    \Rightarrow \delta' = 1 - \left(\frac{1}{2}\right)^h 
    &\leq \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{4\tau\Prob_{\cP_0}[\theta\geq\tau]+4}.
\end{align*}

From \Cref{thm:treatment-approximation-bound}, with probability $\delta>0$ we have that
\begin{equation*}
    \Prob[\neg \cC_0 \vert G] \leq \delta
\end{equation*} 
Define event $\cC$ such that both events $\cC_0$ and $\cC_1$ hold simultaneously in a round: 
\begin{equation}
\label{eq:event-C}
    \cC := \left\{ \forall q \geq L_1: \cC_0 \  \& \ \cC_1 \right\}
\end{equation}

Using union bound, we have
\begin{align}
    \Prob[\neg \cC \vert G] &\leq \Prob[\neg \cC_0 \vert G] + \Prob[\neg \cC_1 \vert G]\\
    &\leq \delta + \delta' \nonumber\\
    &\leq \delta_{\tau} + \delta' \nonumber \\
    &\leq \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{4\tau\Prob_{\cP_0}[\theta\geq\tau]+4} + \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{4\tau\Prob_{\cP_0}[\theta\geq\tau]+4} \nonumber \\
    &= \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2\tau\Prob_{\cP_0}[\theta\geq\tau]+2} \label{eq:delta'}
\end{align}
Therefore, since $\theta\geq -1$, we have: 
\begin{align*}
\label{eq:racing-bic}
    &\quad\E_{\cP_0}[\theta|z_t=1]\Prob_{\cP_0}[z_t=1]\\
    &= \E_{\cP_0}[\theta|z_t=1, \cC]\Prob_{\cP_0}[z_t=1, \cC] + \E_{\cP_0}[\theta|z_t=1, \neg \cC]\Prob_{\cP_0}[z_t=1, \neg \cC]\\
    &\geq \E_{\cP_0}[\theta|z_t=1, \cC]\Prob_{\cP_0}[z_t=1, \cC] - \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2\tau\Prob_{\cP_0}[\theta\geq\tau]+2} 
\end{align*}
We want to upper bound the first term. This can be done by splitting it into four cases based on the value of $\theta$. We have:

\begin{equation} 
    \begin{split}
    &\quad\E_{\cP_0}[\theta|z_t=1,\cC]\Prob_{\cP_0}[z_t=1, \cC] \\
    &= 
    \E_{\cP_0}[\theta|z_t=1, \cC, \theta\geq \tau]\Prob_{\cP_0}[z_t=1, \cC, \theta\geq \tau] \\
    &\ + \E_{\cP_0}[\theta|z_t=1, \cC, 0 \leq \theta < \tau]\Prob_{\cP_0}[z_t=1, \cC, 0 \leq \theta < \tau] \\
    &\ + \E_{\cP_0}[\theta|z_t=1, \cC, -2s_q < \theta < 0]\Prob_{\cP_0}[z_t=1, \cC, -2s_q < \theta < 0] \\
    &\ + \E_{\cP_0}[\theta|z_t=1, \cC, \theta \leq -2s_q]\Prob_{\cP_0}[z_t=1, \cC, \theta\leq -2s_q] \label{eq:racing-bic-cases}
    \end{split}
\end{equation}

By definition of $s_q$, we have:
\begin{align*}
    2s_q &\leq 2s_{L}\\
    &\leq \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2}\\
    &\leq \tau
\end{align*}

% \lscomment{End: Need to edit this part to prove that $s_q\leq s_L$ for all $q>L$}

Conditional on $\cC$, the empirical estimate $\hat{\theta}_q > \theta - s_q \geq 2s_q$. Hence, when we have $\theta \geq \tau \geq 2s_q$, then $\hat{\theta}\geq s_q$ and arm 0 must have already been eliminated at phase $q \geq L_1$. This implies that the probability $\Prob_{\cP_0}[z_t=1, \cC, \theta\geq \tau] = \Prob_{\cP_0}[\cC, \theta\geq \tau]$. Similarly, when we have $\theta \leq -2s_q$, then $\hat{\theta} \leq -s_q$ and arm 1 must have already been eliminated at phase $q \geq L_1$. Hence, arm 1 could not be recommended in that case and the probability $\Prob_{\cP_0}[z_t=1, \cC, \theta\leq-2s_q] = 0$.\\
We can then rewrite equation~\eqref{eq:racing-bic-cases} as
\begin{align*} 
    &\quad\E_{\cP_0}[\theta|z_t=1, \cC]\Prob_{\cP_0}[z_t=1 ,\cC] \\
    \geq &\E_{\cP_0}[\theta|z_t=1, \cC, \theta \geq \tau]\Prob_{\cP_0}[z_t=1, \cC, \theta \geq \tau]\\
    &+ \E_{\cP_0}[\theta|z_t=1, \cC, 0 \leq \theta < \tau]\Prob_{\cP_0}[z_t=1, \cC, 0 \leq \theta < \tau]\\
    &+ \E_{\cP_0}[\theta|z_t=1, \cC, -2s_q < \theta < 0]\Prob_{\cP_0}[z_t=1, \cC, -2s_q < \theta < 0]\\
    \geq &\tau \Prob_{\cP_0}[\cC, \theta \geq \tau] + 0\cdot \Prob_{\cP_0}[z_t=1, \cC, 0 \leq \theta < \tau] -2s_q \Prob_{\cP_0}[z_t=1, \cC, -2s_q<\theta<0]\\
    \geq &\tau \Prob_{\cP_0}[\cC, \theta \geq \tau] - 2s_q\\
    \geq &\tau \Prob_{\cP_0}[\cC, \theta \geq \tau] - \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2}\\
    \geq &\tau \Prob_{\cP_0}[\cC | \theta \geq \tau] \Prob_{\cP_0}[\theta \geq \tau] - \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2}\\
    \geq &\tau (1 - (\delta + \delta')) \Prob_{\cP_0}[\theta \geq \tau] - \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2}\\
    = & \left(\frac{1}{2} - (\delta + \delta') \right) \tau \Prob_{\cP_0}[\theta \geq \tau]\\
    \geq & \left(\frac{1}{2} - \frac{\frac{1}{2} \tau \Prob_{\cP_0}[\theta \geq \tau]}{\tau \Prob_{\cP_0}[\theta \geq \tau] + 1} \right) \tau \Prob_{\cP_0}[\theta \geq \tau] \tag{by \Cref{eq:delta'}}\\
    = & \frac{1}{2} \left(\frac{\tau \Prob_{\cP_0}[\theta \geq \tau] + 1 - \tau \Prob_{\cP_0}[\theta\geq \tau]}{\tau \Prob_{\cP_0}[\theta \geq \tau] + 1} \right)\tau \Prob_{\cP_0}[\theta \geq \tau]\\
    = & \frac{1}{2} \left(\frac{\tau \Prob_{\cP_0}[\theta \geq \tau]}{\tau \Prob_{\cP_0}[\theta \geq \tau] + 1} \right)
\end{align*}
Hence, we have 
\begin{align*}
    &\quad\E_{\cP_0}[\theta|z_t=1]\Prob_{\cP_0}[z_t=1]\\
    &\geq \E[\theta|z_t=1, \cC]\Prob_{\cP_0}[z_t=1, \cC] - \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2\tau\Prob_{\cP_0}[\theta\geq\tau]+2} \\
    &\geq \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2\tau\Prob_{\cP_0}[\theta\geq\tau]+2}  -  \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2\tau\Prob_{\cP_0}[\theta\geq\tau]+2} \\
    &= 0
\end{align*}
Therefore, \Cref{alg:racing-two-types-mixed-preferences} fulfills \Cref{eq:racing-bic-type0} and is compliant for all agents of type 0.
\end{proof}

\subsubsection{Racing Stage First Part Estimation Bound}
\lscomment{Fix this proof so the Union Bound is made more explicit and maybe change the phrase ``Estimation Bound.''}
\label{sec:racing-estimation-bound-first}
\racingestimationboundfirst*
\begin{proof}
    We assume \Cref{alg:racing-two-types-mixed-preferences} to be initialized with parameters (see \Cref{lemma:bic-racing-control-treatment-0} for details) such that its recommendations are compliant for agents of type 0. Therefore, we may apply \Cref{thm:approximation-bound-denominator} where we let the proportion $p_c=p_0$. Finally, we combine the high probability bound on the denominator with the high probability bound on the numerator (given by \Cref{thm:treatment-approximation-bound}), taking a union bound to achieve the confidence parameters $\delta$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Racing Stage Type 1 Compliant Proof}
\label{sec:bic-racing-type-1}
\bicracingcontroltreatmentone*
\begin{proof} 
Let $L_1$ be the biggest phase length of the first racing stage. Let the decision threshold $s_q$ for a phase $q$ be defined as in \Cref{alg:racing-two-types-mixed-preferences}. Assume that after the elimination, at every iteration a sample of the eliminated arm is also drawn, but not revealed to the agent.\\
We define the event $\cC_0$ as the accuracy guarantee of $\hat{\theta}$ such that:
\begin{equation}
\label{eq:event-C-1}
    \cC_0 := \left\{ \forall q \geq L_1: |\theta - \hat{\theta}_q| < s_q \right\}
\end{equation}
where $L$ is the number of samples after running the sampling stage.\\
Let $X^a_q$ be the number of arm $a\in\{0,1\}$ samples in phase $q$. The decision threshold $s_q$ in phase $q$ is unbounded if $X^a_q=0$ for either arm $a$. We also define event $\cC_1$ where there is at least one sample of each arm in each phase:
\begin{equation}
\label{eq:event-C-2}
    \cC_1 := \left\{\forall q\geq L,a: X^a_q \geq 1 \right\}
\end{equation}
Recall that $p_0$ of the population is of type $0$. Then, if \Cref{alg:racing-two-types-mixed-preferences} is compliant for all agents of type 0 and we recommend each arm at least $h$ times in phase $q$, we have $X^0_q>h$ and $X^0_q \sim B(h,p_0)$. Hence, we have
\begin{equation}
    \Prob[X^0_q \geq 1] = 1 - p_0^h = \delta'.
\end{equation}

Let $\tau\in(0,1)$. Fix phase $q\geq L_1$, and some agent $t$ in this phase. In order to prove that \Cref{alg:racing-two-types-mixed-preferences} is compliant for all agents of type 1, we want to show that 
\begin{equation}
    \label{eq:racing-bic-type1}
    \E_{\cP_1}[\theta\vert z_t=0]\Prob_{\cP_1}[z_t=0] < 0.
\end{equation}

Note that, by assumption, the parameter
\begin{align*}
    h &\geq \frac{\log\left(\frac{3\tau\Prob_{\cP_1}[\theta< -\tau]+4}{4\tau\Prob_{\cP_0}[\theta<-\tau]+4}\right)}{\log(1-p_2)}\\
    \Rightarrow \left(\frac{1}{2}
    \right)^h 
    &\geq \frac{3\tau\Prob_{\cP_1}[\theta<-\tau]+4}{4\tau\Prob_{\cP_1}[\theta<-\tau]+4}\\
    \Rightarrow \delta' = 1 - \left(\frac{1}{2}\right)^h 
    &\leq \frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{4\tau\Prob_{\cP_1}[\theta<-\tau]+4}.
\end{align*}

From \Cref{thm:treatment-approximation-bound}, with probability $\delta>0$ we have that
\begin{equation*}
    \Prob[\neg \cC_0 \vert G] \leq \delta
\end{equation*} 
Define event $\cC$ such that both events $\cC_0$ and $\cC_1$ hold simultaneously in a round: 
\begin{equation}
\label{eq:event-C}
    \cC := \left\{ \forall q \geq L_1: \cC_0 \  \& \ \cC_1 \right\}
\end{equation}

Using union bound, we have
\begin{align}
    \Prob[\neg \cC \vert G] &\leq \Prob[\neg \cC_0 \vert G] + \Prob[\neg \cC_1 \vert G]\\
    &\leq \delta + \delta' \nonumber\\
    &\leq \delta_{\tau} + \delta' \nonumber \\
    &\leq \frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{4\tau\Prob_{\cP_1}[\theta<-\tau]+4} + \frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{4\tau\Prob_{\cP_1}[\theta<-\tau]+4} \nonumber \\
    &= \frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{2\tau\Prob_{\cP_1}[\theta<-\tau]+2} \label{eq:delta'-type1}
\end{align}
Therefore, since $\theta\leq 1$, we have: 
\begin{align*}
\label{eq:racing-bic}
    &\quad\E_{\cP_1}[\theta|z_t=0]\Prob_{\cP_1}[z_t=0]\\
    &= \E_{\cP_1}[\theta|z_t=0, \cC]\Prob_{\cP_1}[z_t=0, \cC] + \E_{\cP_1}[\theta|z_t=0, \neg \cC]\Prob_{\cP_1}[z_t=0, \neg \cC]\\
    &\leq \E_{\cP_1}[\theta|z_t=0, \cC]\Prob_{\cP_1}[z_t=0, \cC] + \frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{2\tau\Prob_{\cP_1}[\theta<-\tau]+2} 
\end{align*}
We want to upper bound the first term. This can be done by splitting it into four cases based on the value of $\theta$. We have:

\begin{equation} 
    \begin{split}
    &\quad\E_{\cP_1}[\theta|z_t=0,\cC]\Prob_{\cP_1}[z_t=0, \cC] \\
    &= 
    \E_{\cP_1}[\theta|z_t=0, \cC, \theta \geq  2s_q]\Prob_{\cP_1}[z_t=0, \cC, \theta \geq 2s_q] \\
    &\ + \E_{\cP_1}[\theta|z_t=0, \cC, 0 \leq \theta < 2s_q]\Prob_{\cP_1}[z_t=0, \cC, 0 \leq \theta < 2s_q] \\
    &\ + \E_{\cP_1}[\theta|z_t=0, \cC, -\tau \leq \theta < 0]\Prob_{\cP_1}[z_t=0, \cC, -\tau \leq \theta < 0] \\
    &\ + \E_{\cP_1}[\theta|z_t=0, \cC, \theta \leq -\tau]\Prob_{\cP_1}[z_t=0, \cC, \theta < -\tau] \label{eq:racing-bic-cases-type1}
    \end{split}
\end{equation}

By definition of $s_q$, we have:
\begin{align*}
    2s_q &\leq 2s_{L_1}\\
    &\leq \frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{2}\\
    &\leq \tau
\end{align*}

% \lscomment{End: Need to edit this part to prove that $s_q\leq s_L$ for all $q>L$}

Conditional on $\cC$, the empirical estimate $\hat{\theta}_q > \theta - s_q \geq 2s_q$. Hence, when we have $\theta \geq 2s_q$, then $\hat{\theta}\geq s_q$ and arm 0 must have already been eliminated at phase $q \geq L_1$. This implies that the probability $\Prob_{\cP_1}[z_t=0, \cC, \theta\geq 2s_q] = 0$. Similarly, when we have $\theta \leq -\tau \leq -2s_q$, then $\hat{\theta} \leq -s_q$ and arm 1 must have already been eliminated at phase $q \geq L_1$. Hence, arm 1 could not be recommended in that case and the probability $\Prob_{\cP_1}[z_t=0, \cC, \theta < -\tau] = \Prob_{\cP_1}[\cC, \tau < -\tau]$.\\
We can then rewrite equation~\eqref{eq:racing-bic-cases-type1} as
\begin{align*} 
    &\E_{\cP_1}[\theta|z_t=0, \cC]\Prob_{\cP_1}[z_t=0 ,\cC] \\
    = &\E_{\cP_1}[\theta|z_t=0, \cC, 0 \leq \theta < 2s_q]\Prob_{\cP_1}[z_t=0, \cC, 0 \leq \theta < 2s_q]\\
    &+ \E_{\cP_1}[\theta|z_t=0, \cC, -\tau \leq \theta < 0]\Prob_{\cP_1}[z_t=0, \cC, -\tau \leq \theta < 0]\\
    &+ \E_{\cP_1}[\theta|z_t=0, \cC, \theta < -\tau]\Prob_{\cP_1}[z_t=0, \cC, \theta < -\tau]\\
    \leq &-\tau \Prob_{\cP_1}[\cC, \theta < -\tau] + 0\cdot \Prob_{\cP_0}[z_t=1, \cC, -\tau \leq \theta < 0] + 2s_q \Prob_{\cP_1}[z_t=0, \cC, 0 \leq \theta < 2s_q]\\
    \leq &2s_q - \tau \Prob_{\cP_1}[\cC, \theta \leq -\tau]\\
    \leq &\frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{2} - \tau \Prob_{\cP_1}[\cC, \theta < -\tau] \\
    \leq &\frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{2} - \tau \Prob_{\cP_1}[\cC | \theta < -\tau] \Prob_{\cP_1}[\theta < -\tau]\\
    \leq &\frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{2} - \tau (1 - \delta - \delta') \Prob_{\cP_1}[\theta < -\tau]\\
    = & \left(\frac{-1}{2} + \delta + \delta' \right) \tau \Prob_{\cP_1}[\theta < -\tau]\\
    \leq & \left(\frac{-1}{2} + \frac{\tau \Prob_{\cP_1}[\theta < -\tau]}{2\tau \Prob_{\cP_1}[\theta < -\tau] + 2} \right) \tau \Prob_{\cP_1}[\theta < -\tau] \tag{by \Cref{eq:delta'-type1}}\\
    = & \frac{-1}{2} \left(\frac{\tau \Prob_{\cP_1}[\theta < -\tau] + 1 - \tau \Prob_{\cP_1}[\theta < -\tau]}{\tau \Prob_{\cP_1}[\theta < -\tau] + 1} \right)\tau \Prob_{\cP_1}[\theta < -\tau]\\
    = & \frac{-1}{2} \left(\frac{\tau \Prob_{\cP_1}[\theta < -\tau]}{\tau \Prob_{\cP_1}[\theta < -\tau] + 1} \right)
\end{align*}
Hence, we have 
\begin{align*}
    &\quad\E_{\cP_1}[\theta|z_t=0]\Prob_{\cP_1}[z_t=0]\\
    &\leq \E[\theta|z_t=0, \cC]\Prob_{\cP_1}[z_t=0, \cC] + \frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{2\tau\Prob_{\cP_1}[\theta<-\tau]+2} \\
    &\leq \frac{-\tau\Prob_{\cP_1}[\theta<-\tau]}{2\tau\Prob_{\cP_1}[\theta<-\tau]+2}  +  \frac{\tau\Prob_{\cP_1}[\theta<-\tau]}{2\tau\Prob_{\cP_1}[\theta<-\tau]+2} \\
    &= 0
\end{align*}
Therefore, \Cref{alg:racing-two-types-mixed-preferences} fulfills \Cref{eq:racing-bic-type1} and is compliant for all agents of type 1.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Racing Stage Second Part Estimation Bound}
\lscomment{Fix this proof so the Union Bound is made more explicit and maybe change the phrase ``Estimation Bound.''}
\label{sec:racing-estimation-bound-second}
\racingestimationboundsecond*
\begin{proof}
    We assume \Cref{alg:racing-two-types-mixed-preferences} to be initialized with parameters (see \Cref{lemma:bic-racing-control-treatment-0,lemma:bic-racing-control-treatment-1} for details) such that its recommendations are compliant for all agents. Therefore, we may apply \Cref{thm:approximation-bound-denominator} where we let the proportion $p_c=1$. Finally, we combine the high probability bound on the denominator with the high probability bound on the numerator (given by \Cref{thm:treatment-approximation-bound}), taking a union bound to achieve the confidence parameters $\delta$.
\end{proof}

==> files/general-case/finite-sample-analysis.tex <==
\section{IV Estimator Proof}
\subsection{Model}

The equations central to our model are expressed as such:

\begin{equation}
\left\{ \begin{array}{l}
            y_i = \langle \theta, x_i\rangle + g(u_i) + \epsilon_i\\
            x_i = f(u_i, z_i)
        \end{array}
\right.
\end{equation}
Here $y_i$ is the reward, given by treatment $x_i$, treatment effect $\theta$, zero-mean noise $\epsilon_i$, and unobserved confounding variable $g(u_i)$, which itself is a function of type $u_i$ for the agent in sample $i$. The treatment $x_i$ is given by instrument $z_i$ and unknown selection function $f(z_i, u_i)$. Our goal is to consistently estimate the treatment effect $\theta$. This is complicated by the unobserved confounding variable $g(u_i)$ and its correlation to the treatment $x_i$.

 We model a linear relationship between $x_i$ and $z_i$ by introducing a population mean choice matrix $\Gamma$ (as expressed in equation~\eqref{eq:gamma}). We can rewrite our equation modeling $x_i$ as such:
\begin{align*} 
    x_i 
    = \Gamma^\intercal z_i - \left(\Gamma^\intercal z_i - f(u_i, z_i) \right) 
    &= \Gamma^\intercal z_i + \eta_i\\
    &= \hat{\Gamma}^\intercal z_i + \left(\Gamma^\intercal z_i -  \hat{\Gamma}^\intercal z_i \right) + \eta_i,
\end{align*}
    where $\eta_i = f(u_i, z_i)-\Gamma^\intercal z_i$ and $\hat{\Gamma}$ is an empirical estimate of $\Gamma$ (see equation~\eqref{eq:gammahat}). Now $y_i$ is given as such:
\begin{align} 
    y_i &= \theta^\intercal \left( \hat{\Gamma}^\intercal z_i + \left(\Gamma^\intercal z_i -  \hat{\Gamma}^\intercal z_i \right) + \eta_i \right) + g(u_i) + \epsilon_i\\
    &= \beta^\intercal z_i + \nu_i + \theta^\intercal \eta_i + g(u_i) + \epsilon_i\\
    &= \beta^\intercal z_i + \E[g(u)]\cdot\mathbf{1} + \gamma_i + \nu_i \\
    &= (\beta^*)^\intercal \tilde{z}_i + \gamma_i + \nu_i \label{eq:y}
\end{align}
where $\beta = \hat{\Gamma} \theta$ and $\gamma_i = \theta^\intercal \eta_i + g(u_i) - \E[g(u)] + \epsilon_i$ and $\nu_i = \theta^\intercal (\Gamma - \hat{\Gamma})^\intercal z_i$ and $\beta^* = (\beta, \E[g(u)])$ and $\tilde{z}_i = (z_i, 1)$.\\


\subsection{Finite Sample Analysis} 
Given $n \in \mathbbm{R}$ samples $(z, X, y)_n$, we would like to bound the difference between the predicted exogenous mean treatment effect, denoted $\hat{\theta}_n$, and the true exogenous mean treatment effect $\theta$, i.e. we want to bound $\norm{\hat{\theta}_n -\theta}_2.$

\begin{theorem}
\label{thm:finite-sample}
    Given a sample set $(z_i, x_i, y_i)_n$, which contains $n$ samples of instrument $z$, treatment $X$, and reward $y$, we bound the difference between the true mean treatment effect $\theta$ and the mean treatment effect $\hat{\theta}_n$ derived via IV regression over $(z_i, x_i, y_i)_n$. Let $k$ be the number of arms and $\Upsilon$ be an upper bound on the confounding term $g(u_t)$. Suppose among the $n$ observations $p$ is the proportion of agents that follow our recommendations. For some confidence $\delta>0$, with probability at least $1 - \delta$:
    \begin{align*}
    \norm{\hat{\theta}_n - \theta}_2 
    \leq \frac{4\sqrt{\lambda (k + \Upsilon^2)} + 16\sqrt{2\log\left(3/\delta\right) + (k+1)\log\left( 1 + \frac{2n}{\lambda(k+1)}\right)}}{p\sqrt{2n_{\min}}}.
    \end{align*}
\end{theorem}

\begin{corollary}
\label{cor:finite-sample}
Given a sample set $(z_i, x_i, y_i)_n$, which contains $n$ samples of instrument $z$, treatment $X$, and reward $y$, we bound the difference between the true mean treatment effect $\theta$ and the mean treatment effect $\hat{\theta}_n$ derived via IV regression over $(z_i, x_i, y_i)_n$. Let $k$ be the number of arms and $\Upsilon$ be a upper bound on the confounding term $g(u_t)$. Suppose among the $n$ observations $p$ is the proportion of agents that follow our recommendations. For some confidence $\delta>0$, with probability at least $1 - \delta$:
    \begin{align*}
    \norm{\hat{\theta}_n - \theta}_2 
    \leq \frac{12\sqrt{2\log\left(3/\delta\right) + (k+1)\log (2n(k + \Upsilon^2))}}{p\sqrt{2n_{\min}}}.
    \end{align*}
\end{corollary}

We can estimate $\hat{\theta}_n$ via a generalization of Two-Stages Least Squares (2SLS). In this method, we let $\beta'=\Gamma\theta$. We get an empirical estimate of $\Gamma$, denoted $\hat{\Gamma}$, as in equation~\eqref{eq:gammahat}. Then, we get an estimate for $\beta=\hat{\Gamma}\theta$, denoted $\hat{\beta}_n$, via ridge regression.\\

From here, we can calculate $\hat{\theta}_n = \hat{\Gamma}_n^{-1} \hat{\beta}_n.$ Thus, we express the bound $\norm{\hat{\theta}_n -\theta}_2$ as such: 
\begin{align*}
    \norm{\hat{\theta}_n - \theta}_2
    &= \norm{\hat{\Gamma}_n^{-1}\hat{\beta}_n  - \hat{\Gamma}_n^{-1}\beta }_2\\
    &= \norm{\hat{\Gamma}_n^{-1} \left(\hat{\beta}_n  - \beta\right) }_2\\
    &\leq \norm{\hat{\Gamma}_n^{-1}}_2 \norm{\hat{\beta}_n  - \beta}_2\\
    &= \sigma_{\max}\left\{\hat{\Gamma}_n^{-1}\right\} \norm{\hat{\beta}_n  - \beta}_2\\
    &= \frac{1}{\sigma_{\min}\left\{\hat{\Gamma}_n\right\}} \norm{\hat{\beta}_n  - \beta}_2,\\
\end{align*}
where $\sigma_{\max}$ and $\sigma_{\min}$ are the maximum and minimum singular values of a matrix, respectively and $\hat{\Gamma}_n$ is full rank.\\

Thus, we need to find two bounds in order to upper bound $\norm{\hat{\theta}_n-\theta}_2$:
\begin{enumerate}
    \item find a lower bound for $\sigma_{\min} \{ \hat{\Gamma}\}$ (given by \cref{lemma:sigma-min-bound}); and
    \item find an upper bound for $\left|\left| \hat{\beta}_n - \beta \right|\right|_2$ (given by \cref{thm:beta-bound}).
\end{enumerate}

\begin{lemma}\label{lemma:sigma-min-bound}(Lower bound for $\sigma_{\min}(\hat{\Gamma})$ in the two arm case for two types of agents) For a bandit algorithm with two types of agents and two arms, where $p_1$ of the population is agent of type 1, $p_2$ of the population is agent of type 2, at round $t \geq \frac{12}{p_2}\log(1/\delta)$, with probability at least $1 - \delta$, 
\begin{equation}
    \sigma_{\min}(\hat{\Gamma}) \geq \frac{\sqrt{2}}{4}p_2
\end{equation}
\end{lemma}

\begin{proof}
In our algorithm, we guarantee that agents of type 2 will always follow our recommendations. On the other hand, agents of type 1 will always pick arm 1 during the sampling stage and the first racing stage. Let the actual proportion of agents showing up being type 1 and type 2 are $\hat{p}_1$ and $\hat{p}_2$, respectively. We have 
\begin{equation}
    \hat{\Gamma} = \hat{p}_1\begin{pmatrix}
       1 & 0\\
       1 & 0
    \end{pmatrix} + \hat{p}_2\begin{pmatrix}
       1 & 0\\
       0 & 1
    \end{pmatrix} = \hat{p}\begin{pmatrix}
       1 & 0\\
       1 & 0
    \end{pmatrix} + \hat{p}_2 I
\end{equation}
Hence, we have the outer product
\begin{align*}
    \hat{\Gamma} \hat{\Gamma}^\intercal  &=  
    (\hat{p}_1\begin{pmatrix}
       1 & 0\\
       1 & 0
    \end{pmatrix} + \hat{p}_2 I) (\hat{p}_1\begin{pmatrix}
       1 & 0\\
       1 & 0
    \end{pmatrix} + \hat{p}_2 I)^\intercal\\
    &= \hat{p}_1^2 \begin{pmatrix}
        1 & 1\\
        1 & 1
    \end{pmatrix} + \hat{p}_2^2 I + \hat{p}_1 \hat{p}_2 \begin{pmatrix}
        1 & 0\\
        1 & 0
    \end{pmatrix} + \hat{p}_1 \hat{p}_2 \begin{pmatrix}
        1 & 1\\
        0 & 0
    \end{pmatrix}\\
    &= \begin{pmatrix}
        \hat{p}_1^2 + 2 \hat{p}_1\hat{p}_2 + \hat{p}_2^2 & \hat{p}_1 \hat{p}_2 + \hat{p}_1^2\\
        \hat{p}_1\hat{p}_2 + \hat{p}_1^2 & \hat{p}_1^2 + \hat{p}_2^2
    \end{pmatrix}
\end{align*}
Thus, the minimum singular value of $\hat{\Gamma}$ is 
\begin{align*}
    \sigma_{\min}(\hat{\Gamma}) &= \sqrt{\lambda_{\min}(\hat{\Gamma} \hat{\Gamma}^\intercal)}\\
    &= \sqrt{\hat{p}_1^2 + \hat{p}_1 \hat{p}_2 + \hat{p}_2^2 - \hat{p}_1\sqrt{\hat{p}_1^2 + 2 \hat{p}_1\hat{p}_2 + 2 \hat{p}_2^2}}
\end{align*}
Given that $\hat{p}_1 = 1 - \hat{p_2}$, we have that 
\begin{align*}
    \sigma_{\min}(\hat{\Gamma})  &= \sqrt{(1 - \hat{p}_2)^2 + (1 - \hat{p}_2)\hat{p}_2 + \hat{p}_2^2 - (1 - \hat{p}_2) \sqrt{(1 - \hat{p}_2)^2 + 2(1 - \hat{p}_2)\hat{p}_2 + 2 \hat{p}_2^2}}\\
    &= \sqrt{\hat{p}_2^2 - (1 - \hat{p}_2)\sqrt{ (\hat{p}_2^2 + 1)} - \hat{p}_2 + 1}
\end{align*}
We have 
\begin{align*}
    - (1 - \hat{p}_2)\sqrt{\hat{p}_2^2 + 1} - \hat{p}_2 + 1 &= (\hat{p}_2 - 1)( \sqrt{\hat{p}_2^2 + 1} - 1)\\
    &= \frac{(\hat{p}_2 - 1)(\sqrt{\hat{p}_2^2 + 1} - 1)(\sqrt{\hat{p}_2^2 + 1} + 1)}{\sqrt{\hat{p}_2^2 + 1} + 1}\\
    &= \frac{(\hat{p}_2 - 1)((\hat{p}_2^2 + 1) - 1)}{1+ \sqrt{\hat{p}_2^2 + 1}}\\
    &= \frac{(\hat{p}_2 - 1)(\hat{p}_2^2)}{1+ \sqrt{\hat{p}_2^2 + 1}}\\
    &= \hat{p}_2^2\frac{\hat{p}_2 - 1}{1 + \sqrt{\hat{p}_2^2 + 1}}
\end{align*}
Thus, we have 
\begin{align*}
    \sigma_{\min}(\hat{\Gamma}) &= \sqrt{\hat{p}_2^2 - \sqrt{(\hat{p}_2 - 1)^2 (\hat{p}_2^2 + 1)} - \hat{p}_2 + 1}\\
    &= \sqrt{\hat{p}_2^2 + \hat{p}_2^2\frac{\hat{p}_2 - 1}{1 + \sqrt{\hat{p}_2^2 + 1}}}\\
    &= \sqrt{\hat{p}_2^2 \left( 1 + \frac{\hat{p}_2 - 1}{1 + \sqrt{\hat{p}_2^2 + 1}} \right)}\\
    &= \sqrt{\hat{p}_2^2 \left( \frac{1 + \sqrt{\hat{p}_2^2 + 1} + \hat{p}_2 - 1}{1 + \sqrt{\hat{p}_2^2 + 1}} \right)}\\
    &= \sqrt{\hat{p}_2^2 \left( \frac{\sqrt{\hat{p}_2^2 + 1} + \hat{p}_2}{1 + \sqrt{\hat{p}_2^2 + 1}} \right)}\\
    &\geq \sqrt{\frac{1}{2}\hat{p}_2^2} = \frac{\sqrt{2}}{2}\hat{p}_2
\end{align*}

Next, by Corollary~\ref{cor:multiplicative-chernoff}, with probability at least $1 - \delta$, the empirical proportion of type 2 agents $\hat{p}_2 \geq \frac{p_2}{2}$ at round $t \geq \frac{12}{p_2}\log(1/\delta)$. Thus, the minimum singular value 
\[\sigma_{\min}(\hat{\Gamma}) \geq \frac{\sqrt{2}}{4}p_2\]
\end{proof}


\begin{proof}
In our sampling stage algorithm, we guarantee that $p_1$ of the population will always follow our recommendations. Similarly, in the racing stage, we guarantee that $p_2$ of the population will follow our recommendations. Let the proportion of agents that follow our recommendations in both stages algorithm be $p$. At round $t$, we have
\begin{align}
    p = \frac{L_1 (\rho + 1) p_1 + (q - L_1) p_2}{t}
\end{align}
where $L_1(\rho + 1)$ is the length of the sampling stage and $q$ is the current phase in the racing stage. 
Let the actual numbers of agents that follow our recommendations in both stages be $\hat{p}$.
We have 
\begin{equation}
    \hat{\Gamma} = (1 - \hat{p})\begin{pmatrix}
       1 & 0\\
       1 & 0
    \end{pmatrix} + \hat{p}\begin{pmatrix}
       1 & 0\\
       0 & 1
    \end{pmatrix} = (1 - \hat{p})\begin{pmatrix}
       1 & 0\\
       1 & 0
    \end{pmatrix} + \hat{p} I
\end{equation}
Hence, we have the outer product
\begin{align*}
    \hat{\Gamma} \hat{\Gamma}^\intercal  &=  
    ((1 - \hat{p})\begin{pmatrix}
       1 & 0\\
       1 & 0
    \end{pmatrix} + \hat{p} I) ((1 - \hat{p})\begin{pmatrix}
       1 & 0\\
       1 & 0
    \end{pmatrix} + \hat{p} I)^\intercal\\
    &= (1 - \hat{p})^2 \begin{pmatrix}
        1 & 1\\
        1 & 1
    \end{pmatrix} + \hat{p}^2 I +(1 - \hat{p}) \hat{p} \begin{pmatrix}
        1 & 0\\
        1 & 0
    \end{pmatrix} + (1 - \hat{p})\hat{p} \begin{pmatrix}
        1 & 1\\
        0 & 0
    \end{pmatrix}\\
    &= \begin{pmatrix}
        (1 - \hat{p})^2 + 2 (1 - \hat{p})\hat{p} + \hat{p}^2 &(1 - \hat{p}) \hat{p} + \hat{p}^2\\
        (1 - \hat{p})\hat{p} + \hat{p}^2 & (1 - \hat{p})^2 + \hat{p}^2
    \end{pmatrix}
\end{align*}
Thus, the minimum singular value of $\hat{\Gamma}$ is 
\begin{align*}
    \sigma_{\min}(\hat{\Gamma}) &= \sqrt{\lambda_{\min}(\hat{\Gamma} \hat{\Gamma}^\intercal)}\\
    &= \sqrt{(1 - \hat{p})^2 + (1 - \hat{p}) \hat{p} + \hat{p}^2 - (1 - \hat{p})\sqrt{(1 - \hat{p})^2 + 2 (1 - \hat{p})\hat{p} + 2 \hat{p}^2}}\\
    &= \sqrt{\hat{p}^2 - (1 - \hat{p})\sqrt{ (\hat{p}^2 + 1)} - \hat{p} + 1}
\end{align*}
We have 
\begin{align*}
    - (1 - \hat{p})\sqrt{\hat{p}^2 + 1} - \hat{p} + 1 &= (\hat{p} - 1)( \sqrt{\hat{p}^2 + 1} - 1)\\
    &= \frac{(\hat{p} - 1)(\sqrt{\hat{p}^2 + 1} - 1)(\sqrt{\hat{p}^2 + 1} + 1)}{\sqrt{\hat{p}^2 + 1} + 1}\\
    &= \frac{(\hat{p} - 1)((\hat{p}^2 + 1) - 1)}{1+ \sqrt{\hat{p}^2 + 1}}\\
    &= \frac{(\hat{p} - 1)(\hat{p}^2)}{1+ \sqrt{\hat{p}^2 + 1}}\\
    &= \hat{p}^2\frac{\hat{p} - 1}{1 + \sqrt{\hat{p}^2 + 1}}
\end{align*}
Thus, we have 
\begin{align*}
    \sigma_{\min}(\hat{\Gamma}) &= \sqrt{\hat{p}^2 - \sqrt{(\hat{p} - 1)^2 (\hat{p}^2 + 1)} - \hat{p} + 1}\\
    &= \sqrt{\hat{p}^2 + \hat{p}^2\frac{\hat{p} - 1}{1 + \sqrt{\hat{p}^2 + 1}}}\\
    &= \sqrt{\hat{p}^2 \left( 1 + \frac{\hat{p} - 1}{1 + \sqrt{\hat{p}^2 + 1}} \right)}\\
    &= \sqrt{\hat{p}^2 \left( \frac{1 + \sqrt{\hat{p}^2 + 1} + \hat{p} - 1}{1 + \sqrt{\hat{p}^2 + 1}} \right)}\\
    &= \sqrt{\hat{p}^2 \left( \frac{\sqrt{\hat{p}^2 + 1} + \hat{p}}{1 + \sqrt{\hat{p}^2 + 1}} \right)}\\
    &\geq \sqrt{\frac{1}{2}\hat{p}^2} = \frac{\sqrt{2}}{2}\hat{p}
\end{align*}
\lscomment{Not sure if we need to show that last line (i.e. show the derivative / minimized at $\hat{p}=0$).}

Next, by Corollary~\ref{cor:multiplicative-chernoff}, the empirical proportion of agents following our recommendation $\hat{p} \geq 
\frac{p}{2}$ at round $t \geq \frac{12}{p} \log(1/\delta)$. Thus, the minimum singular value 
\begin{align}
    \sigma_{\min}(\hat{\Gamma}) &\geq \frac{\sqrt{2}}{4}p\\
&= \frac{\sqrt{2}}{4}\left(\frac{L_1 (\rho + 1) p_1 + (q-L_1) p_2}{t} \right)
\end{align}

\end{proof}

In the following, we will demonstrate an upper bound on $\norm{\hat{\beta}_n - \beta}_2$.
\begin{lemma}
\label{lemma:mahalanobis-bound} For some $\delta \in (0,1)$, with probability at least $1-\delta$,
\begin{align}
    \norm{\tilde{\beta} - \beta^*}_{\Sigma + \lambda \bI} \leq \sqrt{\lambda (m + \Upsilon^2)} + 2\sqrt{2\log\left(\frac{2}{\delta_2}\right) + (m+1)\log\left( 1 + \frac{2n}{\lambda(m+1)}\right)}
\end{align}
where $\abs{\E[g(u)]} \leq \Upsilon$.
\end{lemma}
\begin{proof}
We have:
\begin{align*}
    \tilde{\beta} - \beta^* = - (\Sigma + \lambda \bI)^{-1} \lambda \beta^* + (\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n \tilde{z}_i\gamma_i \right) + (\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n\tilde{z}_i \nu_i \right)
\end{align*}
Observe that 
\begin{align*}
    \norm{(\Sigma + \lambda \bI)^{-1} \lambda \beta^*}_{\Sigma + \lambda \bI} &= \sqrt{\lambda (\beta^*)^\intercal ((\Sigma + \lambda \bI)^{-1})^\intercal (\Sigma + \lambda \bI) (\Sigma + \lambda \bI)^{-1} \lambda \beta^*} \\
    &= \sqrt{\lambda (\beta^*)^\intercal ((\Sigma + \lambda \bI)^{-1})^\intercal \lambda \beta^*} \\
    &\leq \lambda \sqrt{\norm{\beta^*}_2^2 \norm{(\Sigma + \lambda \bI)^{-1}}}_2 \ \tag{by Theorem~\eqref{thm:cauchy-schwarz}}\\
    &= \lambda \norm{\beta^*}_2 \sqrt{\lambda_{\max}\left\{(\Sigma + \lambda \bI)^{-1}\right\}}\\
    &= \lambda \norm{\beta^*}_2 \frac{1}{\sqrt{\lambda_{\min}\left\{\Sigma +
    \lambda \bI \right\}}}\\
    &\leq \lambda \norm{\left(\beta, \E_u[g(u)] \right)}_2 \frac{1}{\sqrt{\lambda}}\\
    &= \sqrt{\lambda \left(\norm{\beta}_2^2 + \left(\E_u[g(u)]\right)^2 \right)}\\
    &\leq \sqrt{\lambda(m + \Upsilon^2)}
\end{align*}
We also have that, for some confidence $\delta_1>0$, with probability at least $1-\delta_1$
\begin{align*}
    \norm{(\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n \tilde{z}_i\gamma_i \right)}_{\Sigma + \lambda \bI} &= \sqrt{\left((\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n \tilde{z}_i\gamma_i \right)\right)^\intercal (\Sigma + \lambda \bI) (\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n \tilde{z}_i\gamma_i \right)}\\
    &= \sqrt{\left(\sum_{i=1}^n \tilde{z}_i\gamma_i \right)^\intercal ((\Sigma + \lambda \bI)^{-1}) ^\intercal \left(\sum_{i=1}^n \tilde{z}_i\gamma_i \right)}\\
    &= \norm{\sum_{i=1}^n \tilde{z}_i\gamma_i}_{((\Sigma + \lambda \bI)^{-1}) ^\intercal}\\
    &\leq \sqrt{2\log\left(\frac{1}{\delta_1}\right) + \log\left(\frac{\det(\Sigma + \lambda \bI)}{\lambda^{m+1}}\right)} \ \tag{by Theorem~\ref{thm:mahalanobis-norm-bound}}\\
    &\leq \sqrt{2\log\left(\frac{1}{\delta_1}\right) + (m+1)\log\left( 1 + \frac{2n}{\lambda(m+1)}\right)} \ \tag{by Lemma~\eqref{lemma:epl}}
\end{align*}

Finally, we want to bound $\norm{(\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n\tilde{z}_i \nu_i \right)}_{\Sigma + \lambda \bI}$. We will do so by invoking Theorem~\eqref{thm:mahalanobis-norm-bound}, as above. However, in order to show that this theorem applies, we first have to reduce the sum $\sum_{i=1}^n \tilde{z}_i \nu_i$ is mean-zero. Let $n_j = e_j^\intercal \sum_{i=1}^n z_i$ and $\tilde{e}_j = (e_j, 1)$. We have:
\begin{align*}
    \sum_{i=1}^n \tilde{z}_i \nu_i &= \sum_{i=1}^n \tilde{z}_i \theta^\intercal (\Gamma - \hat{\Gamma})^\intercal z_i\\
    &= \sum_{i=1}^n \tilde{z}_i \theta^\intercal \Gamma^\intercal z_i - \sum_{i=1}^n \tilde{z}_i \theta^\intercal \hat{\Gamma}^\intercal z_i\\
    &= \sum_{i=1}^n \tilde{z}_i \theta^\intercal \Gamma^\intercal z_i - \sum_{j=1}^m n_j \tilde{e}_j \theta^\intercal \hat{\Gamma}_j^\intercal \ \text{(where $\hat{\Gamma}_j$ is the j-th row of $\hat{\Gamma}$)}\\
    &= \sum_{i=1}^n \tilde{z}_i \theta^\intercal \Gamma^\intercal z_i - \sum_{j=1}^m n_j \tilde{e}_j \theta^\intercal \left(\frac{1}{n_j} \sum_{i=1}^n \1[z_i = e_j]x_i \right)\\
    &= \sum_{i=1}^n \tilde{z}_i \theta^\intercal \Gamma^\intercal z_i - \sum_{j=1}^m \tilde{e}_j \theta^\intercal \sum_{i=1}^n \1[z_i = e_j]x_i\\
    &= \sum_{i=1}^n \tilde{z}_i \theta^\intercal \Gamma^\intercal z_i - \sum_{i=1}^n \tilde{z}_i \theta^\intercal x_i\\
    &= \sum_{i=1}^n \tilde{z}_i ( \theta^\intercal \Gamma^\intercal z_i - \theta^\intercal x_i)
\end{align*}

This term is mean-zero. Hence, for confidence $\delta_2>0$, with probability at least $1-\delta_2$, we have:
\begin{align*}
    \norm{(\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n\tilde{z}_i \nu_i \right)}_{\Sigma + \lambda \bI} &= \sqrt{\left((\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n\tilde{z}_i \nu_i \right) \right)^\intercal (\Sigma + \lambda \bI) (\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n\tilde{z}_i \nu_i \right)}\\
    &= \sqrt{ \left(\sum_{i=1}^n\tilde{z}_i \nu_i \right)^\intercal \left((\Sigma + \lambda \bI)^{-1} \right)^\intercal \left(\sum_{i=1}^n\tilde{z}_i \nu_i \right)}\\
    &= \norm{\sum_{i=1}^n\tilde{z}_i \nu_i}_{\left((\Sigma + \lambda \bI)^{-1} \right)^\intercal}\\
    &\leq \sqrt{2\log\left(\frac{1}{\delta_2}\right) + \log\left(\frac{\det(\Sigma + \lambda \bI)}{\lambda^{m+1}}\right)} \ \tag{by Theorem~\eqref{thm:mahalanobis-norm-bound}}\\
    &\leq \sqrt{2\log\left(\frac{1}{\delta_2}\right) + (m+1)\log\left( 1 + \frac{2n}{\lambda(m+1)}\right)} \ \tag{by Lemma~\eqref{lemma:epl}}
\end{align*}

Combining these three bounds, we get that, for confidence $\delta>0$, with probability at least $1-\delta$,
\[ \norm{\tilde{\beta} - \beta^*}_{\Sigma + \lambda \bI} \leq \sqrt{\lambda (m + \Upsilon^2)} + 2\sqrt{2\log\left(\frac{2}{\delta}\right) + (m+1)\log\left( 1 + \frac{2n}{\lambda(m+1)}\right)} \tag{by Lemma~\eqref{thm:union}}\]
\end{proof}

\begin{lemma}
\label{lemma:min_sigma}
The minimum eigenvalue
\[ \displaystyle \lambda_{\min} \left\{\sum_{i=1}^n z_i z_i^{\intercal} \right\} = n_{\min},
\]
the minimum frequency at which any arm is recommended
from the sample set $(z,X,y)_n$.
\end{lemma} 

\begin{proof}
Consider for arbitrary fixed $i$, the vector
$z_i = \left(0, \ \cdots, \ 0, 1, 0, \ \cdots, \ 0 \right)$, where the position of the single $1$ corresponds to the arm $a_i$ recommended in the $i^{\text{th}}$ sample, e.g. if we recommend arm $1$ in the $i^{\text{th}}$ sample, then $z_i = \left( 1, 0, \ \cdots, \ 0 \right).$ 
Then, the normalized sum 
\[  \sum_{i=1}^n z_i z_i^{\intercal} =  \sum_{i=1}^n \diag(z_i) = \diag\left( \sum_{i=1}^n \ind[z_i = \e_1],\ \cdots \ ,  \sum_{i=1}^n \ind[z_i = \e_m] \right),
\]

where \[\diag(a_1, a_2, \cdots, a_n) := 
\begin{pmatrix}
    a_1 & 0 & \cdots & 0\\
    0 & a_2 & \cdots & 0\\
    \vdots & \vdots & \ddots & \vdots \\
    0 & 0 & \cdots & a_n
\end{pmatrix}.\]
For a single arm $j \in [1,m]$, the term $ \sum_{i=1}^n \ind[z_i = \e_j]$ corresponds to the frequency at which treatment $j$ is recommend out of all $n$ samples. 
Let $n_{\min}$ be the minimum number of times that any one arm is recommended such that
\[
n_{\min} := \min_j \sum_{i=1}^n \ind[z_i = \e_j].
\]

With this, we may express the smallest diagonal entry in the matrix as $n_{\min}$. 

Since $\sum_{i=1}^n z_i z_i^{\intercal}$ is a non-negative semidefinite diagonal matrix, its eigenvalues are simply the entries of the diagonal. Thus, 
\[\lambda_{\min} \left\{ \sum_{i=1}^n z_i z_i^{\intercal} \right\} = n_{\min}. \]
\end{proof} 
\begin{theorem} 
\label{thm:beta-bound}
For some $\delta \in (0,1)$, with probability at least $1-\delta$,
\begin{align*}
    \norm{\hat{\beta} - \beta}_2 \leq \frac{\sqrt{\lambda (m + \Upsilon^2)} + 2\sqrt{2\log\left(\frac{2}{\delta}\right) + (m+1)\log\left( 1 + \frac{2n}{\lambda(m+1)}\right)}}{\sqrt{n_{\min}}}
\end{align*}
where $n_{\min}$ is the minimum number of times any arm is recommended, i.e. $\displaystyle n_{\min} := \argmin_j \sum_{i=1}^n \ind[z_i = \e_j]$.
\end{theorem}
\begin{proof}

Let $\Sigma = \sum_{i=1}^n \tilde{z}_i \tilde{z}_i^\intercal$ where $\tilde{z}_i = (z_i,1)$. Let $\lambda\geq0$ be some non-negative constant. Remember that $\beta^* = (\beta, \E[g(u)])$. Using ridge regression, we estimate the relationship between $y_i$ and $\tilde{z}_i$ as:
\begin{align*}
    \tilde{\beta} &= (\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n \tilde{z}_i y_i \right)\\
    &= (\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n \tilde{z}_i (\tilde{z}_i^\intercal \beta^* + \gamma_i + \nu_i) + \lambda \beta^* - \lambda \beta^* \right) \ \tag{by Equation \ref{eq:y}}\\
    &= \beta^* - (\Sigma + \lambda \bI)^{-1} \lambda \beta^* + (\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n \tilde{z}_i\gamma_i \right) + (\Sigma + \lambda \bI)^{-1} \left(\sum_{i=1}^n\tilde{z}_i \nu_i\right)
\end{align*}
Let $\hat{\beta}$ be such that $\tilde{\beta} = \left( \hat{\beta}, \hat{\E}[g(u)] \right)$ where $\hat{\E}[g(u)]$ estimates $\E[g(u)]$ and $\hat{\beta}$ estimates $\beta$.\\

Now, let $\norm{x}_M \triangleq \sqrt{x^\intercal M x}$ for any real matrix $M$ and vector $x$ (see lemma~\ref{thm:mahalanobis-norm}). We have 
\begin{align*}
    \norm{\tilde{\beta} - \beta^*}^2_{\Sigma + \lambda \bI} &\geq \norm{(\hat{\beta}, 0) - (\beta, 0)}^2_{\Sigma + \lambda\bI}\\
    &= (\hat{\beta} - \beta, 0)^\intercal (\Sigma + \lambda \bI) (\hat{\beta} - \beta, 0)\\
    &= (\hat{\beta} - \beta, 0)^\intercal \Sigma (\hat{\beta} - \beta, 0) + \lambda\norm{\hat{\beta} - \beta}_2^2\\
    &= \sum_{i=1}^n (\langle(\hat{\beta} - \beta, 0), (z_i, 1))\rangle)^2 + \lambda \norm{\hat{\beta} - \beta}_2^2\\
    &= \sum_{i=1}^n (\langle\hat{\beta} - \beta, z_i\rangle)^2 + \lambda \norm{\hat{\beta} - \beta}_2^2\\
    &= (\hat{\beta} - \beta)^\intercal \left( \sum_{i=1}^n z_i z_i^\intercal \right) (\hat{\beta} - \beta) + \lambda \norm{\hat{\beta} - \beta}_2^2\\
    &\geq \lambda_{\min}\left\{\sum_{i=1}^n z_i z_i^\intercal \right\} \norm{\hat{\beta} - \beta}_2^2 + \lambda \norm{\hat{\beta} - \beta}_2^2 \tag{see proof of Lemma~\eqref{lemma:min_sigma}}\\
    &= (n_{\min} + \lambda) \norm{\hat{\beta} - \beta}_2^2, \ \tag{by Lemma~\eqref{lemma:min_sigma}}
\end{align*}
where $n_{\min}$ is the minimum number of times any arm is recommended, i.e. $\displaystyle n_{\min} := \argmin_j \sum_{i=1}^n \ind[z_i = \e_j]$.
Hence, for some $\delta \in (0,1)$, with probability at least $1 - \delta$:
\begin{align*}
    \norm{\hat{\beta} - \beta}_2 &\leq \frac{\sqrt{\lambda (m + \Upsilon^2)} + 2\sqrt{2\log\left(\frac{2}{\delta}\right) + (m+1)\log\left( 1 + \frac{2n}{\lambda(m+1)}\right)}}{\sqrt{n_{\min}}} \ \tag{by Lemma~\eqref{lemma:mahalanobis-bound}}
\end{align*}
\end{proof}





==> files/general-case/many-arms-many-types.tex <==
\newpage
\section{Heterogeneous Priors with Many Types and Many Arms}

\paragraph{General Algorithm.} Following the structure of the detail free algorithm in \cite{mansour2015bic}, we split our algorithm into two \textit{stages}, the \textit{sampling} and the \textit{racing} stages. Stages are separated into \textit{phases}, which are made up of a number of \textit{rounds} each. The first stage of the algorithm is the \textit{sampling stage}, which is a sub-algorithm that collects $L_1$ samples of each arm. In the first phase, the algorithm collects $L_1$ samples of the arm which all agents favor. Then, it leverages these samples to incentivize agents of at least one type to comply with all our recommendations. \ls{Maybe go more into how the algorithm incentivizes this, but in a very concise way.} By relying on this group of compliant agents, we are able to collect $L_1$ samples of each arm with a high probability.

Once we have these samples, we then use them as input parameters for the \textit{racing stage} sub-algorithm. In addition to \cite{mansour2015bic}, this algorithm is based on the \textit{active arms elimination} algorithm of \cite{active-arms-elimination-2006}. During each phase of the racing stage, we recommend every arm one-by-one. From the first phase, at least one type is fully compliant. At each phase of the racing stage, agents are able to deduce about how many samples of each arm has been collected \ls{this isn't right, needs better wording}; through this, it is possible that more types become fully compliant at different points in the racing stage. Through this, we are able to collect samples of each arm more efficiently than in the sampling stage.

Our algorithm differs from the incentive-compatible algorithm of \cite{mansour2015bic} insofar as we do not enforce fully compliance with our recommendations throughout all rounds. Rather, we only necessitate compliance for a subset of agents. As we will demonstrate in Remark~\ref{remark:regret-comparison-2-arm}, this difference leads to improvements in regret in a number of settings. 

We can calculate the minimum exploration probability $\rho_i$ to make the sampling stage algorithm BIC for all agents of type $i \in [1, r]$. Then, we can order the the types $1, \dots, r$ by largest to smallest exploration probabilities, i.e. $\rho_1 > \dots > \rho_r$. Suppose that we know some lower bound on the prior dependent constant for a type $\kappa$. Then, we can partition the set of agents' types into two smaller subsets: agents of type $i$ where $i \leq \kappa$ and agents of type $j$ where $j > \kappa$. Since the types are ordered by the exploration probability needed to make them comply with our recommendations in the sampling stage, if we can convince agents of type $pi$ to follow our recommendations, other agents in the first subset would also comply. Hence, similar to the simple setting of two arms, we will rely on the agents in the first subset to take our recommendations and collect samples of all arms. We simply run the sampling stage algorithm above by inputting the largest exploration probability of the first group $\rho_\kappa$ into Algorithm~\ref{alg:general-sampling}. Thus, the sampling stage (using Algorithm~\ref{alg:general-sampling}) will be BIC for agents of all types $i \leq \kappa$ in the first subset only.\\

\subsection{General Model}
\paragraph{} We extend the binary treatment model to a general model with many arms and many types of agents. As before, we study a sequential game between a \textit{social planner} and a sequence of \textit{agents} over $T$ rounds, where $T$ is known to the social planner. There are $k$ actions to choose from. In each round $t$, an entirely new agent indexed by $t$ arrives with their \emph{private type} $u_t$ drawn independently from a distribution $\cU$ defined over the set $U$ of all privates types. Each agent $t$ receives an action recommendation $z_t\in\{0,1\}^k$ from the planner and then selects an action $x_t\in\{0,1\}^k$ --where if action $i$ is chosen in round $t$, then $x_t = \e_i$, the unit vector in the $i$th dimension-- and receives a reward $y_t\in\mathbb{R}$.

\paragraph{Reward} Given the choice of $x_t\in\{0,1\}^k$ the observed outcome $y_t$ for each agent $t$ is given by 
\begin{equation}
    \label{eq:general-reward-model}
    y_t = \langle \theta, x_t \rangle + g(u_t) + \epsilon_t
\end{equation}
where $\theta\in[-1,1]^k$ denotes the unknown exogenous \emph{treatment effect}, the term $g(u_t)$ denotes a \emph{baseline reward} that depends on the agent's private type $u_t$, and the term $\epsilon_t$ denotes an independent reward noise with a subgaussian norm of $\sigma_{\epsilon}$ and conditional expectation $\E[\epsilon_t \mid x_t, u_t] = 0$. \lsedit{We assume without loss of generality that the expected value of the confounding error term $\E[g(u_i)]=0$, through $g(u_i)$ is correlated with $x_i$ through $u_i$.} Furthermore, we assume that for all rounds $t$, the confounding term $|g(u_t)| \leq \Upsilon$ for some constant $\Upsilon$. Both $g(u_t)$ and $\epsilon_t$ are unobserved by the social planner. The social planner's objective is to maximize the total observed reward of all agents over all $T$ rounds.\\

The utility for an agent $t$ is different than the observed reward insofar as the agent incurs some cost for taking the treatment that is not accounted for in the observed reward. Let the utility for agent $t$ be:
\begin{equation}
    \label{eq:general-reward-model-agent}
    y_t^{\text{agent}} 
    :=\, y_t - \phi(u_t)x_t
    =\, \theta{x_t} - \phi(u_t)x_t + g(u_t) + \epsilon_t
\end{equation}
where $\phi(u_t)$ denotes the cost to an agent of type $u_t$ for taking the treatment for cost function $\phi: U \rightarrow  [-\nu, \nu]$. The social planner observes neither cost function $\phi$ nor agent reward $y_t^{\text{agent}}$.

Agents are self-interested individuals who aim to maximize their own expected reward $y_t^{\text{agent}}$, while the social planner aims to maximize the long-term cumulative rewards across all agents.
\lsdelete{Formally, let $\theta^{a^*} = \max_a \theta^a$. Then the social planner aims to induce a sequence of action selections $x_1, \ldots , x_T$ to minimize \emph{regret}, defined as:
\begin{equation}
    R(T) = T\, \theta^{a^*}  - \sum_{t=1}^T \theta^{x_t}_t.
\end{equation}

We are also interested in type-specific regret. In particular, the regret accumulated by agents of type $u$ is defined as
\begin{equation}
    R^{u}(T) = \sum_{t=1}^T \left(\theta^{a^*}-\theta^{x_t}_t\right)\1[u_t = u].
\end{equation}}



\xhdr{History and recommendation policy}
The interaction between the planner and the agent $t$ is given by the tuple $(z_t, x_t, y_t)$. 
For each $t$, let $H_t$ denote the history from round 1 to $t$, that is the sequence of interactions between the social planner and first $t$ agents: $\left((z_1, x_1, y_1), \ldots ,(z_t, x_t, y_t) \right)$. 
Before the game starts, the social planner commits to a recommendation policy $\pi = (\pi_t)_{t=1}^T$ where each $\pi_t \colon \left(\{0,1\}^k\times \{0,1\}^k \times \mathbb{R}\right)^{t-1} \rightarrow \Delta(\{0,1\}^k)$ is a randomized mapping from the history $H_{t-1}$ to a recommendation $z_t$. The policy $\pi$ is fully known to the agents.


\paragraph{Beliefs, incentives, and action choices}
%\label{def:bic}
Each agent $t$ knows their place $t$ in the sequential game. As part of their private type $u_t$, each agent $t$ has a \emph{prior belief distribution} $\cP_{t}$, which is a joint distribution over the treatment effect $\theta$, the agents' private types, and their reward noise.

In round $t$, the action $x_t$ chosen is given by a selection function $f$ that takes the following form:
\begin{equation}
    \label{eq:general-selection-function}
    x_t = f(u_t, z_t, t) := \argmax_{x_i\in\{0,1\}^k}\left[ \E_{\mathcal{P}_t}\left[\langle\theta,x_i\rangle \ | \ u_t, z_t, t \right] - \phi_i(u_t) \right],
\end{equation}
where, as above, $\phi_i(u_t)$ denotes the cost to an agent of type $u_t$ for taking arm $i$, for some bounded function $\phi_i: U \rightarrow  [-\nu, \nu]$.

We say that the recommendation is \emph{Bayesian incentive compatible (BIC)} for agent $t$ if $x_t = z_t$.

\subsection{Finite Sample IV Estimate Bound for General Setting}
\subsubsection{Model}
We present our model as a system of linear equations expressed as such
\begin{equation}
    \begin{cases}
    y_i = \langle \theta, x_i \rangle + g(u_i) + \epsilon_i\\
    x_i = f(u_i, z_i)
    \end{cases}
\end{equation}
We model a linear relationship between the action $x_i$ and the recommendation $z_i$ by introducing a \textit{compliance matrix} $\Gamma$ that captures the probability that any agent in the population chooses an action given a recommendation, formally, the $jk$-th term of $\Gamma$ is defined as such:
\begin{equation*}
    \Gamma_{jk} := \Prob[x_i = \e_j| z_i = \e_k]
\end{equation*}
Then, we can rewrite our equation modelling $x_i$ as such:
\begin{align*}
    x_i &= \Gamma z_i + \left(f(u_i, z_i) - \Gamma z_i \right)\\
    &= \Gamma z_i + \eta_i
\end{align*}
where $\eta_i = f(u_i, z_i) - \Gamma z_i$ is a mean-zero random vector-valued variable. Now, we can rewrite the reward $y_i$ as 
\begin{align*}
    y_i &= \langle \theta, \Gamma z_i + \eta_i \rangle + g(u_i) + \epsilon_i\\
    &= \langle\Gamma\theta,z_i\rangle + \langle\theta,\eta_i\rangle + g(u_i) + \epsilon_i\\
    &= \langle\beta,z_i\rangle + \langle\theta,\eta_i\rangle + g(u_i) + \epsilon_i, \tag{where $\Gamma\theta=\beta$}
\end{align*}

\subsection{Finite Sample Analysis}

\begin{restatable}[Treatment effect approximation bound for General Model]{theorem}{generaltreatmentapproximationbound}\label{thm:general-treatment-approximation-bound}
        Given a sample set $(z_i, x_i, y_i)_n$, which contains $n$ samples of instrument $z\in\RR^k$, treatment $x\in\RR^k$, and reward $y\in\RR$, we bound the difference between the true treatment effect $\theta\in\RR^k$ and the predicted treatment effect $\hat{\theta}_n$ derived via IV regression over $(z_i, x_i, y_i)_n$. Let $\Upsilon$ be a upper bound on the confounding term $g(u_i)$. For some confidence $\delta>0$, with probability at least $1 - \delta$:
    \[\norm{\hat{\theta}_n-\theta}_2 \leq \frac{(2\Upsilon+\sigma_{\eps})\sqrt{2nk\log(2k/\delta)}}{\sigma_{\min}\left\{\sum_{i=1}^n z_ix_i^{\intercal}\right\}},\]
where $\sigma_{\min}(\cdot)$ denotes the smallest non-zero singular value.
\end{restatable}

\begin{proof}
    See \cref{sec:general-approximation-bound-proof} for a proof.
\end{proof}

\input{files/appendix/expected-g-zero-without-centering}

\subsection{Setting Assumptions}
Before we present our algorithm, we present our background assumptions.
\begin{assumption}
There are $k$ arms, each with a true mean reward vector, namely $\theta^1, \dots, \theta^k$. The entire population of agents has $r$ types, i.e. type 1, \dots, type $r$. Each type $i$ has a Bayesian prior, namely $\cP_i$, over the distribution of the mean reward vector $\theta$. For each type $i$, the prior mean reward of arm $a$ is given by $\mu^a_i := \E_{\cP_i}[\theta^a]$. We assume that the arms are ordered according to their prior mean rewards and that this ordering is shared across types, i.e. $\mu^1_i > \dots > \mu^k_i$ for all types $i \in [1, r]$.\footnote{This ordering assumption is shared by \citep{mansour2015bic}.}
\end{assumption}

% Assumptions:
% \begin{itemize}
%     \item The social planner knows a bound $\Upsilon$ on the confounding error term $g(u_t)$, i.e. $\abs{g(u_t)} \leq \Upsilon$. 
%     \item The entire population of agents has $r$ types, each with its own common prior, namely $\cP_1, \dots , \cP_r$ on the distribution of the mean reward vector $\theta$. (The ordering of the priors is arbitrary unless specified otherwise.)
%     \item There are $m$ arms, each with a true mean reward vector, namely $\theta^1, \dots, \theta^m$, each drawn i.i.d. from a true distribution $\cP$.
%     \item For a given prior $\cP_i$ prior mean reward of arms $1$ through $m$ are $\mu_i^1,\ \mu_i^2,\ \dots,\ \mu_i^m$. These prior mean rewards are ordered such that $\mu_i^1 > \mu_i^2 > \dots, > \mu_i^m$ for the priors of all types.
%     \item The social planner knows the ordering of the arms according to their prior mean rewards.
% \end{itemize}
Denote $C = \Upsilon + \sigma_{\epsilon}\sqrt{\frac{2\ln(1/\delta)}{L_1}} + \frac{1}{4}$, where $\sigma_{\epsilon}$ is the variance parameter for the distribution from which the error $\epsilon_t$ is drawn.\\

\begin{algorithm}[ht] 
\SetAlgoLined 
\SetKwInput{KwIn}{Input}
\KwIn{Parameters $\ell_1,\rho\in\mathbb{N}$ and specified type $1\leq\kappa^*\leq\,r$}
\KwIn{Sample average of reward $\bar{y}_{L_1}^1$ after $L_1$ pulls of arm $1$ }
    \For{each arm $i > 1$ in increasing lexicographic order}{
    \eIf{$\bar{y}^1_{\ell_1} + C < \bar{y}^j_{\ell_1} - C$ and $\bar{y}^j_{\ell_1}+C<\mu^i_{\kappa^*}$ for all arms $j<i$} 
    {$a^*_i = i$} 
    {$a^*_i = 1$}
    From the set $P$ of the next $\ell_1\rho$ agents, pick a set $Q$ of $\ell_1$ agents uniformly at random.\\
    Every agent $t\in\,P-Q$ is recommended arm $a_i^*$.\\
    Every agent $t\in\,Q$ is recommended arm $i$.\\
    Let $\bar{y}^i_{\ell_1}$ be the average reward among the agents in $Q$.
    }
    \caption{Sampling stage for many arms and types (BIC for one subset of types throughout)}
    \label{alg:general-sampling} 
\end{algorithm}
We prove in \cref{lemma:bic-general-sampling} that \cref{alg:general-sampling} is BIC for agents of type $\kappa\leq\kappa^*$ as long as the number of phases $\rho$ when we collect samples from each arm is larger than some prior-dependent constant. Similar to the simple setting with two arms, when an agent of type $\kappa\leq\kappa^*$ receives a recommendation for arm $a$, they do not know whether it is due to exploration or exploitation. However, with large enough number of phases $\rho$, the exploration probability for arm $a$, which is $1/\rho$, is low enough that the expected gain from exploiting exceeds the expected loss from exploring and the agent is sufficiently incentivized to take arm $a$.

\begin{restatable}[General Sampling Stage is BIC for Type $\kappa$]{lemma}{bicgeneralsampling}\label{lemma:bic-general-sampling} Consider partially-BIC bandit exploration with $k$ arms and $r$ types. Algorithm~\ref{alg:general-sampling} above with parameters $(\rho_{\kappa}, \ell_1)$ completes in  $\ell_1\rho_{\kappa}(k-1) + \ell_1$ rounds. \ls{Not sure how the proportion of type 1 plays into the how long the sampling stage should be.} For a given type $\kappa$ and an arm $i$, let the event $\xi^i_\kappa$ be defined as such:
\begin{equation}
    \label{eq:xi-type-arm}
    \xi^i_{\kappa} := \left\{ \bar{y}_{\ell_1}^1 + C \leq \min_{1<j<i} \bar{y}_{\ell_1}^j - C \ \text{ and } \ \max_{1<j<i} \bar{y}_{\ell_1}^j + C \leq \mu_{\kappa}^i \right\}
\end{equation}
\dncomment{and let event $\xi := \xi_{i^*},$ where $i^* := \argmin_{i} \Prob[\xi_i]$ not sure this notation is still needed} . 

\Cref{alg:general-sampling} is BIC for agents of type $i: 1 \leq i \leq \kappa$ if we hold the assumptions above, each prior mean $\mu^i_{\kappa}>0$ for all $1<i\leq k$, and the parameters satisfy the following:
\begin{equation}
    \rho_{\kappa} \geq 1 + \frac{8(\mu_{\kappa}^j - \mu_{\kappa}^j)}{\Prob_{\cP_{\kappa}}[\xi^i_{\kappa}]}
\end{equation}
\end{restatable}

\subsection{Racing Stage}
We provide an extension of \cref{alg:racing-two-types-mixed-preferences} to $k\geq2$ arms and $r\geq2$ types with the same preferences, i.e. the ordering of all $k$ arms over all priors are the same. Similar to the Active Arm Elimination algorithm proposed in \cite{active-arms-elimination-2006}, the arms race against each other. Once an arm is determined with high confidence to be sub-optimal, it will drop out of the race, until there is only one remaining arm. Initially, all arms are considered in the race, but each arm can be eliminated from the race once its IV estimate is sufficiently worse than the current "best" arm with high confidence. In this setting, the racing stage is still split into two parts based on some type $\kappa^*<r$, which is input as a parameter into \cref{alg:racing-many-types-two-phases}. If we were to order the types by how ``hard'' they are to persuade to become incentive-compatible, then all types less than $\kappa^*$ are incentive-compatible in the first part of the algorithm. All types greater than or equal to $\kappa^*$ are incentive-compatible only in the second part of the algorithm.


We restrict the priors of these types by assuming that all types become incentive-compatible before the racing stage declares a winner i.e. before the difference in IV estimates determine the best arm overall with high confidence.

% First, we want to determine the threshold needed to eliminate one arm from the "active" pool with high confidence. Since an arm $a$ is determined to be sub-optimal by comparing its estimate $\hat{\theta}^a$ to the estimate of the current "best" arm $\hat{\theta}^{a^*}$, we use the same threshold in Lemma \ref{lemma:stopping criteria} for the simple setting of two arms and two types. We drop arm $a$ from the race once the confidence intervals of the IV estimates $\hat{\theta}^a$ and $\hat{\theta}^{a^*}$ stop overlapping, where $a^*$ is the current "best" arm (with lexicographic tie-breaking, if needed).

\dncomment{
\begin{algorithm}[ht!]
\SetAlgoLined
\SetKwInput{KwIn}{Input}
\KwIn{parameters $L_1 \in \mathbb{N}$; time horizon $T$; type $\kappa \leq r$ (which serves as the breaking point between the two loops of this algorithm); number of recommendations for a single arm $h$ in a phase}
\KwIn{IV estimates of mean reward $\theta^1, \dots, \theta^k$, denoted $\hat{\theta}^1_{L_1}, \dots, \hat{\theta}^k_{L_1}$}
    Let $\hat{\theta}^1_{L_1}, \dots, \hat{\theta}^k_{L_1}$ be the IV estimates of the mean rewards of $\theta^1, \dots, \theta^k$, respectively, after $L_1\rho$ rounds of Algorithm;\\
    Initialize set of active arms: B = \{ all arms \}.\\
    Split remainder into consecutive phases of $100$ rounds each, starting from phase $q = L_1$;\\
    Let $\hat{\theta}^i_{q}$ be the IV estimate of the reward of each arm $i \in \{1,\dots,m\}$ for the racing stage up to and including phase $q$;\\
    \While{$L_1 < \frac{2304(\log(3T/\delta) + (k+1)\log(2T(k+\Upsilon^2)))}{\left(\sigma_{\min}\left(\hat{\Gamma}\right)\right)^4 \tau^2 (\Prob_{\cP_{\kappa}}[G \geq \tau]^2)}$}{
    Let $\hat{\theta}_q^* := \max_{i\in B} \hat{\theta}_q^i$ be the largest estimated mean reward so far;\\
    Recompute $B = \left\{ \text{arms } i: |\hat{\theta}_q^* - \hat{\theta}_q^i| \leq \frac{12\sqrt{\log(2T/\delta) + (k+1)\log(2T(k+\Upsilon^2))}}{\left(\sigma_{\min}\left(\hat{\Gamma}\right)\right)^2 \sqrt{q}} \right\}$\\
    The next $|B|h$ agents are recommended each arm $i\in B$ sequentially in lexicographic order;\\ 
    $q=q+1$;}
    \While{$|B|>1$}
    {
    Let $\hat{\theta}_q^* := \max_{i\in B} \hat{\theta}_q^i$ be the largest estimated mean reward so far;\\
    Recompute $B = \left\{ \text{arms } i: \hat{\theta}_q^* - \hat{\theta}_q^i \leq \frac{12\sqrt{\log(3T/\delta) + (k+1)\log(2T(k+\Upsilon^2))}}{\left(\sigma_{\min}\left(\hat{\Gamma}\right)\right)^2 \sqrt{q}} \right\}$\\
    The next $|B|h$ agents are recommended each arm $i\in B$ sequentially in lexicographic order;\\ 
    $q=q+1$;
    }
    For all remaining agents recommend $a^*$ that remains in $B$.
    \caption{The racing stage for many arms and many heterogeneous types split into two phases}
    \label{alg:racing-many-types-two-phases}
\end{algorithm}
}

\begin{algorithm}[ht!]
\SetAlgoLined
\SetKwInput{KwIn}{Input}
\KwIn{Samples $S_L := \{x_i, z_i, y_i\}^L_{1}$ from the sampling stage sans the first phase $L \in \mathbbm{N}$; time horizon $T$; type $\kappa \leq r$ (which serves as the breaking point between the two loops of this algorithm); number of recommendations for a single arm $h$ in a phase}
\KwIn{IV estimates of mean reward $\theta^1, \dots, \theta^k$, denoted $\hat{\theta}^1_{L_1}, \dots, \hat{\theta}^k_{L_1}$ and approximation bound $s_{L_1} := \frac{12\sqrt{\log(2T/\delta) + (k+1)\log(2T(k+\Upsilon^2))}}{\left(\sigma_{\min}\left(\hat{\Gamma}\right)\right)^2 \sqrt{L_1}}$}
    Let $\hat{\theta}^1_{L_1}, \dots, \hat{\theta}^k_{L_1}$ be the IV estimates of the mean rewards of $\theta^1, \dots, \theta^k$, respectively, after $L_1\rho$ rounds of Algorithm;\\
    Initialize set of active arms: B = \{ all arms \}.\\
    Split remainder into consecutive phases of $h2^q$ rounds each, starting from phase $q = 1$;\\
    Let $\hat{\theta}^i_{q}$ be the IV estimate of the reward of each arm $i \in \{1,\dots,m\}$ for the racing stage up to and including phase $q$;\\
    \While{$\abs{\theta - \hat{\theta}}_{q-1} < s_{q-1}$}{
    Let $\hat{\theta}_q^* := \max_{i\in B} \hat{\theta}_q^i$ be the largest estimated mean reward so far;\\
    Recompute $B = \left\{ \text{arms } i: |\hat{\theta}_q^* - \hat{\theta}_q^i| \leq \frac{12\sqrt{\log(2T/\delta) + (k+1)\log(2T(k+\Upsilon^2))}}{\left(\sigma_{\min}\left(\hat{\Gamma}\right)\right)^2 \sqrt{q}} \right\}$\\
    The next $|B|h$ agents are recommended each arm $i\in B$ sequentially in lexicographic order;\\ 
    Define $S_q^{\text{BEST}}$ as the samples from the phase with best approximation bound, i.e. $S_q^{\text{BEST}}=\argmin\limits_{S_r,\,0\leq\,r\leq\,q}\frac{12\sqrt{\log(2T/\delta) + (k+1)\log(2T(k+\Upsilon^2))}}{\left(\sigma_{\min}\left\hat{\Gamma}\right)\right)^2 \sqrt{r}}$\\ 
    Define $\hat{\theta}_q$ and $s_q$ as the estimate and approximation bound defined over the best samples $S_q^\text{BEST}$\\
    $q=q+1$;}
    For all remaining agents recommend $a^*$ that remains in $B$.
    \caption{The racing stage for many arms and many heterogeneous types split into two phases}
    \label{alg:racing-many-types-two-phases}
\end{algorithm}
\subsection{Racing stage BIC}
% First, we want to determine the threshold needed to declare the winner of the racing stage the best arm overall with high confidence. Similar to the technique used in \cite{active-arms-elimination-2006}, this threshold is determined through the accuracy guarantee of our treatment effect estimate in Theorem \ref{thm:finite-sample}. We use it to find a winner arm. We start with all arms activated. Then, at a given phase $q$ and for any arm $i$, once the confidence interval of the estimates $\hat{\theta}_q^*$ and $\hat{\theta}_q^i$ stop overlapping, we can inactivate arm $i$. Details of this analysis are in Lemma $\ref{lemma:inactivation-criterion-many-types}$ below. 
% \begin{lemma} (Inactivation Criterion)
% \label{lemma:inactivation-criterion-many-types}
% Given samples of the instrumental variable $z_t$ and the response variable $y_t$ from each round $t$ of the racing stage, we can derive the criterion for eliminating any arm $i$ from the running for the winning arm in Algorithm~\eqref{alg:racing-many-types-two-phases} at phase $q$:
% \begin{align} 
%     |\hat{\theta}^*_q - \hat{\theta}^i_q| \leq \frac{12\sqrt{\log(2T/\delta) + 3\log(2n(2+\Upsilon^2))}}{\left(\sigma_{\min}\{\hat{\Gamma}\}\right)^2 \sqrt{q}}
% \end{align}
% where $\hat{\theta}^*_q$ is the largest estimated mean reward of some arm $a^*$ $\hat{\theta}^i_q$ is the estimated mean reward of any arm $i$ at phase $q$.
% \end{lemma}
% \begin{proof}
% For Algorithm~\eqref{alg:racing-many-types-two-phases} to successfully find the best arm, we need to first express the deviation bound on the mean reward of arms $a^*$ and $i$. Let round $q$ be the last round that arm $i$ is still active. We have that:
% \begin{align}
%     \abs{\hat{\theta}^*_q - \hat{\theta}^i_q} \leq r_q^* + r_q^i
% \end{align}
% where $r_q^i$ is the deviation radius of arm $i$ and $r_q^*$ is the deviation radius of the best arm $a^*$ at round $q$.
% We also have:
% \begin{align*}
%     r_q^* + r_q^i &= |\hat{\theta}^*_q - \theta^*| + |\hat{\theta}^i_q - \theta^i|\\
%     &\leq \norm{\hat{\theta}_q - \theta}_\infty\\
%     &\leq 2\norm{\hat{\theta}_q - \theta}_2
% \end{align*}
% From Corollary ~\eqref{cor:finite-sample}, we have:
% \begin{align*}
%     \norm{\hat{\theta}_q - \theta}_2 &\leq  \frac{6\sqrt{\log(2T/\delta) + (m+1)\log(2n(m+\Upsilon^2))}}{\left(\sigma_{\min}\{\hat{\Gamma}\}\right)^2 \sqrt{n_{\min}}}\\
%     \Rightarrow |\hat{\theta}^*_q - \hat{\theta}^i_q| &\leq \frac{12\sqrt{\log(2T/\delta) + (m+1)\log(2n(m+\Upsilon^2))}}{\left(\sigma_{\min}\{\hat{\Gamma}\}\right)^2 \sqrt{q}} \tag{since $n_{\min} >= q$}\\
% \end{align*}
% Therefore, the inactivation criterion can be rewritten as:
%     \begin{equation}
%         |\hat{\theta}^*_q - \hat{\theta}^i_q| \leq \frac{12\sqrt{\log(2T/\delta) + (m+1)\log(2n(m+\Upsilon^2))}}{\left(\sigma_{\min}\{\hat{\Gamma}\}\right)^2 \sqrt{q}}.
%     \end{equation} 
% \end{proof}
We prove that \cref{alg:racing-many-types-two-phases} is BIC for agents of types $i<\kappa$ as long as we have collected sufficient samples of all arms in the sampling stage and our estimate of $\theta$ is close to the true treatment effect. Due to information asymmetry, when an agent is recommended an arm $a$, they do not know whether the arms are still racing each other or if the best arm has been found. However, with a low enough threshold, the expected gain from exploiting the best arm exceed the expected loss from exploring a random arm and the agents of type $i<\kappa$ would follow our recommendation. 

\begin{restatable}[General Racing Stage BIC for Types $\kappa< \kappa^*$]{lemma}{bicracingmanytypesfirst}\label{lemma:racing-bic-many-types-1st-group}
Assume $k$ arms. Let $\delta'$ be the probability of not getting a sample of every arm $a$ in each phase. Let $\displaystyle G := \theta^2 - \theta^1$. Fix an absolute constant $\tau \in (0, 1)$ and let \[\delta_{\tau} = \frac{1}{2}\frac{\tau \Prob_{\cP_i}[G \geq \tau]}{\tau \Prob_{\cP_i}[G \geq \tau] + 1} - \delta'.\] Algorithm~\ref{alg:racing-many-types-two-phases} is BIC for all agents of types $i < \kappa$ if the parameters satisfy $\delta \leq \delta_{\tau}$ and
\[L_1 \geq \frac{2304(\log(2T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\left(\sigma_{\min}\left(\hat{\Gamma}\right)\right)^4 \tau^2 (\Prob_{\cP_i}[G \geq \tau]^2)}.\]
\end{restatable}


During the first racing stage, we collect more samples of arm 2 through agents of type 2. After getting sufficient samples of arm 2, we can also convince agents of type 1 to follow our recommendation for arm 2. The following Lemma $\ref{lemma:racing-bic-two-types-type-1}$, which follow the same structure as that of Lemma $\ref{lemma:racing-bic-two-types}$, proves the second racing stage algorithm is BIC for both agents of type 1 and type 2.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% 2nd Part %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{restatable}[Types $j > \kappa$ BIC]{lemma}{bicracingmanytypessecond}\label{lemma:racing-bic-many-types-2nd-group}
Let $\displaystyle G := \theta^2 - \theta^1$. Fix an absolute constant $\tau \in (0, 1)$ and let \[\delta_{\tau} = \frac{1}{2}\frac{\tau \Prob_{\cP_j}[G \geq \tau]}{\tau \Prob_{\cP_j}[G \geq \tau] + 1}.\] Algorithm~\ref{alg:racing-many-types-two-phases} is BIC for all agents of types $j<\kappa$ if the parameters satisfy $\delta \leq \delta_{\tau}$ and
\[L_1 \geq \frac{2304(\log(2T/\delta) + 3\log(2n(2+\Upsilon^2)))}{\left(p_2 - \sqrt{\frac{\log(1/\delta)}{2n}}\right)^4 \tau^2 (\Prob_{\cP_j}[G \geq \tau]^2)}.\]
\end{restatable}

==> files/paper/control-treatment-sampling-stage-all-params.tex <==
%\section{Setting Assumptions and Sampling Stage for Control-Treatment with Two Mixed-Preference Types}

\section{Overcoming Complete Non-Compliance}
\label{sec:two-arms-two-priors}

In this section, we provide a recommendation policy that incentivizes compliance to enable IV estimation. We focus on a setting where the agents are initially completely non-compliant: since the planner has no information about the treatment effect in the initial rounds, the recommendations have no influence on agents' action selections. For simplicity of exposition, we will present our policy in a setting where there are two types of agents who are initially ``always-takers'' and ``never-takers.'' As we show later \lsedit{in section... (general section)}, this assumption can be relaxed to have arbitrarily many types and allow all types to be ``always-takers.''

\lscomment{Maybe we should make note that we actually need always-takers and never-takers. It won't work without both.}
\swcomment{I thought it would still work with both always takers?}

\xhdr{Two private types.} We assume there are two types of agents. Let $p_i$ for $i\in\{0,1\}$ be the proportion of agents of type $i$ in the population. Let $\cP^{(0)}$ and $\cP^{(1)}$ denote the prior beliefs of the two types. Agents of type 1 initially prefer the treatment: their prior mean for $\theta$ satisfies $\mu_1 = \E_{\cP^{(1)}}[\theta] > 0$. Agents of type 0 initially prefer the control: their prior mean for $\theta$ satisfies
$\mu_0 = \E_{\cP^{(0)}}[\theta] < 0$.

\swcomment{we need to state the assumptions over priors here}

\swdelete{
\begin{itemize}
    \item agents of type 0 initially prefer the control (arm 0), i.e. $\mu^0_0 > \mu^1_0$; and
    \item agents of type 1 initially prefer the treatment (arm 1), i.e. $\mu^0_1 < \mu^1_1$.
\end{itemize}
}
\swcomment{Notations: (1) prior belief $\cP^{(1)}$ (2) we no longer needs $\mu^1_1$ type notation, right? we only have one parameter $\theta$}

\swdelete{
\swcomment{Can we say something about (1) both are always-takers and (2) handle more than two types (control-treatment with multiple types)?}
\dnedit{At the beginning, before receiving any reommendation from the social planner, both types are \textit{always-takers}, as they always choose their preferred arm. Our analysis can be extended to handle multiple types of agents with mixed preference. Such extension is deferred to the full version of our paper (or the appendix, depending on how we structure this)}

We do so by recommending control as an ``exploitation'' arm most of the time and recommending treatment as an ``exploration'' arm with a low probability. Because we recommend the exploration arm with low probability, our instrument is weak and it takes a lot of rounds to get an IV estimate with a good approximation bound. 

Once our approximation bound is good enough, we move to the second phase: the racing stage (\Cref{alg:racing-two-types-mixed-preferences}). In the racing stage, we play Active Arms Elimination \cite{active-arms-elimination-2006} and recommend arms 0 and 1 sequentially in equal proportion. In the first part of this stage, only type 0 agents are compliant, insofar as they always follow our recommendations. Up until this point, agents of type 1 will always choose arm 1, regardless of what we recommend. However, in the second part of the racing stage, our estimate $\hat{\theta}$ is good enough so that all agents become compliant and follow our recommendations. Once one arm `wins,' we end the racing stage and only recommend the winning arm for the remainder of the time horizon. At each stage, we get a confidence interval on the true treatment effect relative to our estimate $\hat{\theta}$ and approximation bound (given in \Cref{thm:treatment-approximation-bound}).

In the first phase of algorithm \ref{alg:sampling-control-treatment}, we let the agents pick their preferred arm. Hence, each agent chooses the better arm according to their prior: agents of type 0 will choose control (arm 0) while agents of type 1 will take treatment (arm 1). \lscomment{Is this true? It confers no information, but the agents don't necessarily know which stage of the algorithm they're in, so agents of type 3 might actually have a more complicated posterior based on which stage of the algorithm they believe they're in.}}

\begin{assumption} In \Cref{alg:sampling-control-treatment}, the social planner knows the following:
\begin{enumerate}
    \item The proportion $p_i$ of agents of each type $i$ in the population;
    \item The initial preference of each type: type 0 agents prefer control while type 1 agents prefer treatment;
    \item Some prior-dependent constants \dncomment{maybe move this down after defining event $\xi$}
\end{enumerate}

\end{assumption}

\lscomment{Rewrite paragraph above.}

\swcomment{check below: 1) we need to explain why only incentivize type 0; 2) removed racing stage discussion, 3) we haven't introduced the term "arm", so let's not use it to avoid confusion.}

\lscomment{Our algorithm is based on the Sampling Stage algorithm of \citet{mansour2015bic}: the difference being that our algorithm is applied in a control-treatment setting with heterogeneous types, whereas the algorithm of \citet{mansour2015bic} works for $k\geq2$ treatments with unknown effects and all agents have the same prior over the treatment effects.}

Our algorithm splits into two stages. In the first stage, we let the agents take their preferred arms according to their prior beliefs: type 0 will choose control and type 1 will choose treatment. This allows us to collect $\ell_0$ observations of rewards for $x=0$ and $\ell_1$ observations of rewards for $x=1$, for sufficiently large $\ell_0$ and $\ell_1$. Let $\bar y_0$ and $\bar y_1$ denote the empirical average rewards for the two actions, respectively. Note that since the baseline rewards $g^{(u)}$ are correlated with the selections $x$, $\bar y_1 - \bar y_0$ is a biased estimate for $\theta$. In the second stage, we will use the initial set of reward observations to construct valid instruments that incentivize agents of one of the two types to follow both control and treatment recommendations. Without loss of generality, we focus on incentivizing compliance among type 0 agents. Since they already prefer control, the primary difficulty here is to incentivize type 0 agents to be compliant with the treatment recommendation.\footnote{We could incentivize type 1 agents to take the control. However, this is an opposing goal to incentivizing type 0 agents to take the treatment, since it would require rewriting \Cref{alg:sampling-control-treatment} so that the control is recommended when exploring and rewriting event $\xi$ so that the expected reward of the treatment over $\cP^{(1)}$ is negative.} We leverage the following observation: according to the prior $\cP^{(0)}$ of type zero, there is a non-zero probability that the biased estimate $(\bar y_1 - \bar y_0)$ is so large that $\theta$ must be positive. Formally, consider the following event for the average rewards $\bar y_0$ and $\bar y_1$:
\begin{small}
\begin{equation}
\label{eq:xi}
    \xi = \bigg\{ \bar y_1 > \bar y_0 + \sigma_0\sqrt{\frac{2\log(2/\delta)}{\ell_0}} + \sigma_1\sqrt{\frac{2\log(2/\delta)}{\ell_1}} +  G^{(0)} + c_1\bigg\}
\end{equation}
\end{small}
where $0<c_1<1$ is a hyperparameter, $G^{(0)}$ is an upper bound on the expected value $\E_{\cP^{(0)}}[g^{(1)}_j-g^{(0)}_j]$, and $\sigma_0$ and $\sigma_1$ are the variance parameters for $g^{(0)}$ and $g^{(1)}$, respectively.

\swcomment{details to check above: (1) $\delta$ should be $\delta/2$ or smaller? (2) how is the constant $1/2$ chosen? should it be related to $\E[g^{(u)}]$, which was upper bounded by $\Upsilon$ (3) i also don't know why $\xi$ needs to be type-specific}

\swdelete{For a given type $i$, there is a non-zero chance that arm 0 performs so poorly that the posterior of arm 1 looks better than that of arm 0 conditioned on the observed samples. We define this event as the \textit{fighting chance} event for a particular arm $i$:
\lscomment{Should it be $\log(2/\delta)$ below?}
\lscomment{Can we change $1/2$ to just $\delta$ below?}\swcomment{yea, please update}
\begin{equation}
    \xi_i = \left\{ \frac{1}{\ell_1} \sum_{t=1}^{\ell_1} y_t^1 - \frac{1}{\ell_0} \sum_{t=1}^{\ell_0} y_t^0 > \sigma_g\left(\sqrt{\frac{2\log(1/\delta)}{\ell_0}} + \sqrt{\frac{2\log(1/\delta)}{\ell_1}}\right) + \frac{1}{2}\right\} 
\end{equation}
where $\delta>0$ is a small failure probability and at round $t$, the term $y_t^a$ denotes the observed reward of taking arm $a$ at time $t$ (or no reward if arm $a$ is not observed at time $t$), i.e. $y_t^a = y_t\1[x_t=a]$.}
 
 
\lsdelete{ 
\begin{algorithm}[tb]
   \caption{Sampling stage for control-treatment with two mixed-preference types \lscomment{revise this}}
   \label{alg:sampling-control-treatment}
\begin{algorithmic}
   \STATE {\bfseries Input:} hyperparameters $c_1,c_3>0$, exploration probability $0<\rho<1$, $\ell_1,\ell_0 \in \mathbb{N}$ and $0<\delta<\delta'$, where $c_3\delta':=\Prob_{\cP_0}[\xi]$
   \STATE In the first $\ell_0 + \ell_1$ rounds of the Sampling Stage, let the agents pick their preferred arm. The sample average of the control reward $y^0$ after $\ell_0$ agents chose control is denoted $\bar{y}^0_{\ell_0}$. Similarly, the sample average of the treatment reward $y^1$ after $\ell_1$ agents chose treatment is denoted $\bar{y}^1_{\ell_1}$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE After that, do the following:\\
    \IF{$\displaystyle \bar{y}_{\ell_0}^0 - \bar{y}_{\ell_1}^1 > \sigma_g\left(\sqrt{\frac{2\log(1/\delta)}{\ell_0}} + \sqrt{\frac{2\log(1/\delta)}{\ell_1}}\right) + G^{(0)} + c_1$}
    \STATE $a^* = 0$
    \ELSE
    \STATE $a^* = 1$
    \ENDIF
    \STATE From the set $P$ of the next $\ell_1.\rho$ agents, pick a set $Q$ of $\ell_1$ agents uniformly at random.
    \STATE Every agent $t \in P - Q$ is recommended arm $a^*$.
    Every agent $t \in Q$ is recommended arm 1.
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\SetAlgoLined
\SetKwInput{KwIn}{Input}
\KwIn{parameters $\rho, \ell_1 \in \mathbb{N}$ and $0<\delta<\delta'$, where $\delta':=\frac{\Prob_{\cP_0}[\xi]}{8}$, $c_1 > 0$}
In the first $\ell_0 + \ell_1$ rounds of the Sampling Stage, let the agents pick their preferred arm. The sample average of the control reward $y^0$ after $\ell_0$ agents chose control is denoted $\bar{y}^0_{\ell_0}$. Similarly, the sample average of the treatment reward $y^1$ after $\ell_1$ agents chose treatment is denoted $\bar{y}^1_{\ell_1}$. 


After that, do the following:\\
    \eiF{$\displaystyle \bar{y}_{\ell_0}^0 > \bar{y}_{\ell_1}^1 + C$}
    {$a^* = 0$} 
    {$a^* = 1$}
    From the set $P$ of the next $\ell_1.\rho$ agents, pick a set $Q$ of $\ell_1$ agents uniformly at random.\\
    Every agent $t \in P - Q$ is recommended arm $a^*$.\\
    Every agent $t \in Q$ is recommended arm 1.
    \caption{Sampling stage for control-treatment with two mixed-preference types}
    \label{alg:sampling-control-treatment}
\end{algorithm}

  }


\begin{algorithm}[ht!]
    \caption{Sampling stage for control-treatment with two mixed-preference types}
    \label{alg:sampling-control-treatment}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} hyperparameters $c_1,c_2>0$, exploration probability $\rho\in (0,1)$, $\ell_1,\ell_0 \in \mathbb{N}$ and $0<\delta<\delta'$, where $\delta':=\frac{\Prob_{\cP_0}[\xi]}{c_3}$
   \STATE In the first stage of $(\ell_0+\ell_1)$ rounds, no recommendation is given. Agents choose the action they prefer initially.
   \STATE Let $B:=\sigma_0\sqrt{\frac{2\log(2/\delta)}{\ell_0}} + \sigma_1\sqrt{\frac{2\log(2/\delta)}{\ell_1}} + G^{(0)} + c_1$
   \lscomment{Do we need to say what all the terms are again?}
   \IF{Event $\xi$ occurs, such that $\bar y^{(1)} > \bar y^{(0)} + B$}
   \STATE $a^*=0$
   \ELSE \STATE $a^*=1$
   \ENDIF
   \STATE From the next $\ell$ agents, pick $\rho\ell$ agents uniformly at random to be in the explore set $E$
   \FOR{The next $\ell$ rounds}
   \IF{agent $i$ is in explore set $E$} \STATE Recommend $z_i = 0$
   \ELSE
   \STATE Recommend $z_i = a^*$
   \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}

We prove that \Cref{alg:sampling-control-treatment} is compliant for agents of type 0 as long as the exploration probability $\rho$ is less than some constant that  depends on prior $\cP^{(0)}$. When an agent of type 0 is recommended treatment, they do not know whether this is due to exploration or exploitation. However, with small enough $\rho$, the expected gain from exploiting exceeds the expected loss from exploring. Hence, the agents would comply with the recommendation and take treatment.


\begin{restatable}[Type 0 compliance with \Cref{alg:sampling-control-treatment}]{lemma}{bicsamplingcontroltreatment}\label{lemma:bic-sampling-control-treatment}
    \Cref{alg:sampling-control-treatment} with parameters $(\rho, \ell_0, \ell_1)$ completes in $\ell + \ell_0 + \ell_1$ rounds. \Cref{alg:sampling-control-treatment} is compliant for all agents of type 0 if we hold the assumption above and the following parameters satisfy:
    %\vspace{-2cm}
    \begin{equation}
        \rho \leq 1 + \frac{\mu^{(0)}}{c_2\Prob_{\cP^{(0)}}[\xi]-\mu^{(0)}}
    \end{equation}
    and hyperparameters $c_1,c_2,c_3>0$ are chosen such that $(c_1-c_2)c_3>2$ and $c_3\delta'=\Prob_{\cP^{(0)}}[\xi]$.
\end{restatable}
\dndelete{For type 0, the \textit{fighting chance} event is given as
\begin{equation}
    \xi = \left\{ \frac{1}{\ell_1} \sum_{t=1}^{\ell_1} y_t^1 - \frac{1}{\ell_0} \sum_{t=1}^{\ell_0} y_t^0 > \sigma_0\sqrt{\frac{2\log(1/\delta)}{\ell_0}} + \sigma_1\sqrt{\frac{2\log(1/\delta)}{\ell_1}} + \E_{\cP^{(0)}}[g^{(1)}_i - g^{(0)}_i] + c_1 \right\} ,
\end{equation}
 and happens with probability at least $1-\delta$ for confidence $\delta \in (0,1)$.
}
where the event $\xi$ is defined above in $\Cref{eq:xi}$. 
\dndelete{
\begin{proof}
    See \Cref{sec:sampling-bic-proof} for a proof.
\end{proof}
}\\

We also provide a separate accuracy guarantee for the estimate $\hat{\theta}_S$ at the end of the $\Cref{alg:sampling-control-treatment}$.  
\begin{restatable}[Sampling Stage Treatment Effect Confidence Interval]{theorem}{samplingestimationbound}\label{thm:sampling-estimation-bound}
    With $n$ total samples collected from \Cref{alg:sampling-control-treatment} --run with exploration parameter $\rho$ large enough so that our recommendations are compliant for type 0 agents (see \Cref{lemma:bic-sampling-control-treatment}),-- we form an estimate $\hat{\theta}_n$ of the treatment effect $\theta$. For any $\delta\in(0,1)$, with probability at least $1-\delta$,
    \[\left|\hat{\theta}_n-\theta\right| \leq \frac{2\rho\sigma_g\sqrt{2n\log(4/\delta)}}{\left(np_0(1-1/\rho)-\sqrt{\frac{n(1-1/\rho)\log(4/\delta)}{2}}\right)},\]
    where $\sigma_g$ is the variance of $g^{(u_i)}$ and $p_0$ is the probability an agent is type 0 for any single round.
\end{restatable}
\dndelete{
\begin{proof}
    See \Cref{sec:sampling-estimation-bound} for a proof.
\end{proof}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Overcoming Partial Compliance and Regret Analysis}
\label{sec:racing-two-arm-regret}
We observe a set of $\ell$ samples from the sampling stage. With large enough $\ell$, we run the racing stage algorithm, which is a modification of the \textit{Active Arms Elimination}  algorithm \citep{active-arms-elimination-2006} with added compliance constraints, i.e. that agents of type 0 are compliant in the first part of the algorithm, then all agents in the second part. Finally, once an arm is found to be sub-optimal, it will be dropped from the race and the other arms ``wins''. For the remaining rounds of \Cref{alg:racing-two-types-mixed-preferences}, all agents are recommended the winning arm only.  \dndelete{We employ the doubling trick \citep{besson2018doubling} to successively increase the phase length of the racing stage.
}

\swcomment{We don't need doubling trick, which is not for accelerating also.}

\swcomment{In the algorithm, we should replace the denominator in $s_L$ by general "sufficiently small" error rate. I think should prove a theorem that shows that as long as the error bound is below some threshold, we could run such racing stage.}


% \subsection{Racing Stage for Control-Treatment with Two Mixed-Preference Types}

\begin{algorithm}[ht!]
% \SetAlgoLined
% \SetKwInput{KwIn}{Input}
\begin{algorithmic}
\STATE{\bfseries Input: } samples $S_L:=\{x_i,z_i,y_i\}_1^L$ sampling stage sans the first phase $L \in \mathbb{N}$; time horizon $T$; minimum phase length $h$; probability $\delta$
\STATE{\bfseries Input: }IV estimate of mean reward $\theta$, denoted $\hat{\theta}_L$ and approximation bound $s_L := \frac{2\sigma_g\sqrt{2L\log(4/\delta)}}{\left|\sum_{i=1}^L(x_i-\bar{x})(z_i-\bar{z})\right|}$ defined over samples $S_L$ from the sampling stage\\
    Let $\hat{\theta}_0:=\hat{\theta}_L$ and $s_0:=s_L$ and $S_0:=S_L$;\\
    Split the remainder into consecutive phases of $h2^q$ rounds each, starting $q=1$;\\
    \WHILE{$\hat{\theta}_{q-1} \leq s_{q-1}$}
    \STATE{The next $h2^q$ agents are recommended both arms sequentially;\\
    For each arm $a \in \{0,1\}$, let $y^a_t$ be one sample reward of that arm in this phase;\\
    Let the samples gathered from round $q$ be denoted $S_q:=\{x_i,z_i,y_i\}_{L+h2^{q-1}}^{L+h2^q}$\\
    Define $S_q^{\text{BEST}}$ as the samples from the phase (including the sampling stage samples $S_L$) with the best approximation bound, i.e. $S_q^{\text{BEST}}=\argmin\limits_{S_r,\,0\leq\,r\leq\,q}\frac{2\sigma_g\sqrt{2|S_r|\log(4/\delta)}}{\left|\sum_{S_r}(x_i-\bar{x})(z_i-\bar{z})\right|}$;\\
    Define $\hat{\theta}_q$ and $s_q$ as the estimate and approximation bound defined over the best samples $S_q^{\text{BEST}}$;\\
    $q = q+1$;}
    \ENDWHILE
    
    For all remaining agents recommend $a^*=\1\left[\hat{\theta}_q>0\right]$   
\end{algorithmic}

    \caption{The racing stage for control-treatment with two mixed-preference types}
    \label{alg:racing-two-types-mixed-preferences}
\end{algorithm}


\swcomment{Dropping a sequence of lemmas and theorems without text in between is terrible. general rule of thumb: try to explain, even briefly, why each lemma should be there.}

We prove that agents of type $i$ are always compliant with the recommendations of \Cref{alg:racing-two-types-mixed-preferences} 
whenever we have a small enough confidence interval of the $\hat{\theta}$ estimate. 
\begin{restatable}[Racing Stage Compliance for Type 0]{lemma}{bicracingcontroltreatmentzero}\label{lemma:bic-racing-control-treatment-0}
    Fix some constant $\tau \in (0, 1)$. Let $\Prob_{\cP^{(0)}}[\theta>\tau]$ be the prior probability that $\theta>\tau$ for agents of type 0. By \Cref{thm:treatment-approximation-bound}, the approximation bound $s_L$ after the sampling stage is given as: 
    \begin{equation}
        s_L:=\frac{2\sigma_g\sqrt{2L\log(2/\delta)}}{\left|\sum_{i=1}^L(x_i-\bar{x})(z_i-\bar{z})\right|}
        \leq\frac{\tau\Prob_{\cP_0}[\theta>\tau]}{4}.
    \end{equation} 
    Then, during the first phase of the racing stage, all agents of type 0 will be compliant with the recommendations from \Cref{alg:racing-two-types-mixed-preferences}.
\end{restatable}

Similar to the sampling stage, we also provide a standalone accuracy guarantee for the estimate $\hat{\theta}_n$ at the end of the first phase of the $\Cref{alg:racing-two-types-mixed-preferences}$. 
\begin{restatable}[First Part Racing Stage Treatment Effect Confidence Interval]{theorem}{racingestimationboundfirst}\label{thm:racing-estimation-bound-first}
    With $n$ total samples collected from the first part of \Cref{alg:racing-two-types-mixed-preferences} where the type 0 compliance criterion on the sampling stage approximation bound is met (see \Cref{lemma:bic-racing-control-treatment-0}), form an estimate $\hat{\theta}_n$ of the treatment effect $\theta$. With probability at least $1-\delta$ for any $\delta \in (0,1)$,
    \[\left|\hat{\theta}_n-\theta\right| \leq \frac{8\sigma_g\sqrt{2n\log(4/\delta)}}{np_0-\sqrt{n\log(4/\delta)}}\]
\end{restatable}
After having collected enough samples of both choices, we can guarantee that in the second part of $\Cref{alg:racing-two-types-mixed-preferences}$, both types of agents comply with the social planner's recommendations. Then, we can say that our algorithm is fully compliant for all agents in this period. 
\begin{restatable}[Racing Stage Compliance for Type 1]{lemma}{bicracingcontroltreatmentone}\label{lemma:bic-racing-control-treatment-1}
    Fix some constant $\tau \in (0, 1)$. Let $\Prob_{\cP_1}[\theta<-\tau]$ be the prior probability that $\theta<-\tau$ for agents of type 1. Let the approximation bound $s_{L_1}$ after the first racing stage be \begin{equation}
        s_{L_1}:=\frac{2\sigma_g\sqrt{2L_1\log(2/\delta)}}{\left|\sum_{i=1}^{L_1}(x_i-\bar{x})(z_i-\bar{z})\right|}
        \leq\frac{\tau\Prob_{\cP_1}[\theta < -\tau]}{4}.
    \end{equation} 
    Then, during the second part of the racing stage, the recommendations from \Cref{alg:racing-two-types-mixed-preferences} are compliant for agents of type 1 (as well as for type 0).
\end{restatable}
Finally, after $\Cref{alg:racing-two-types-mixed-preferences}$ has become compliant for both types of agents, we achieve the following accuracy guarantee for the final treatment estimate $\hat{\theta}_n$.
\begin{restatable}[Second Part Racing Stage Treatment Effect Confidence Interval]{theorem}{racingestimationboundsecond}\label{thm:racing-estimation-bound-second}
    With $n$ total samples collected from the second part of \Cref{alg:racing-two-types-mixed-preferences} where the compliance criterion for both types on the sampling stage approximation bound is met (see \Cref{lemma:bic-racing-control-treatment-0,lemma:bic-racing-control-treatment-1}), form an estimate $\hat{\theta}_n$ of the treatment effect $\theta$. With probability at least $1-\delta$ for any $\delta \in (0,1)$,
    \[\left|\hat{\theta}_n-\theta\right| \leq \frac{8\sigma_g\sqrt{2n\log(4/\delta)}}{n}\]
\end{restatable}



\lsdelete{
\subsection{Regret Analysis}
The goal of this algorithm is to maximize the cumulative reward of all agents. We measure the algorithm's performance through the definition of regret. We are interested in minimizing the ex-post regret of the algorithm, which is the regret specific to a particular treatment effect $\theta$. Since the priors are not exactly known to the social planner, this ex-post regret is correct for any realization of the priors and treatment effect $\theta$. 
Our entire algorithm (with the sampling stage and the racing stage) achieves sub-linear ex-post regret. 


\begin{restatable}[Regret]{lemma}{expostregret}\label{lemma:expost-regret}
\Cref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with sampling stage length parameters $\ell_1, \rho \in \NN$ achieves ex-post regret
\begin{equation}
R(T) \leq \ell_1 \rho + O(\sqrt{T\log T})
\end{equation}
where $\ell_1$ is the sampling stage's phase length and $1/\rho$ is the exploration probability in the sampling stage. 
\end{restatable}
% \begin{lemma} (Regret) 
% \label{lemma:expost-regret}
% Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves ex-post regret
% \begin{equation}
% R(T) \leq \ell_1 \rho + O(\sqrt{T\log T})
% \end{equation}
% where $\ell_1$ is the sampling stage's phase length and $1/\rho$ is the exploration probability in the sampling stage. 
% \end{lemma}
With similar analysis, we also achieve sub-linear expected regret over the randomness in the priors of the agents. Lemma \ref{lemma:expected-regret} provides a basic performance guarantee of our algorithm. 
\begin{restatable}[Expected Regret]{lemma}{expectedregret}\label{lemma:expected-regret}
Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves expected regret
\begin{align}
\E[R(T)] = O(\sqrt{T\log T})
\end{align}
\end{restatable}
% \begin{lemma} (Expected Regret)
% \label{lemma:expected-regret}
% Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves expected regret
% \begin{align}
% \E[R(T)] = O(\sqrt{T\log T})
% \end{align}
% \end{lemma}

These results are analyzed via standard technique and are comparable to the regret of the classic multi-armed bandit problem, with some added constants factors for the compliance constraints \cite{active-arms-elimination-2006}. Although the regret of our algorithm is the same as the fully incentive-compatible algorithm for both types, our algorithm can finish in a more timely manner and has smaller prior-dependent constants in the asymptotic bound.

From the analysis in Lemma \ref{lemma:expost-regret}, we can derive the type-specific regret for each type of agent. Since our algorithm does not guarantee that all agents follow our recommendation, this regret analysis is divided into two cases, depending on the best arm overall. With our assumption \ref{sec:assumptions-two-arms} that the proportions of each agent's type in the population are equal, Lemma \ref{lemma:type-specific-regret} below demonstrates the type-specific regret guarantee of our algorithm.
\begin{restatable}[Type-specific regret]{lemma}{typespecifictwoarms}\label{lemma:type-specific-regret}
Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves type-specific regrets in Table \ref{tab:type-specific-regret}.
\begin{table*}[ht]
    \centering
    \caption{Type-Specific Regret for Two Arms \& Two Types with partially compliant Algorithm}
    \begin{tabular}{ll}
    \toprule
    Best arm / Type     & Type-specific regret \\
    \midrule
    Arm 0 / Type 0     & $O\left(\frac{\log T }{(\tau \Prob_{\cP_0}[\theta \geq \tau] - \nu)^2} \right) + O(\sqrt{T\log T})$\\
    Arm 0 / Type 1      & $O\left(\frac{\log T}{(\tau \Prob_{\cP_0}[\theta \geq \tau] - \nu)^2} \right) + O\left(\frac{\log T}{(\tau\Prob_{\cP_1}[\theta < -\tau] - \nu)^2}\right) + O(\sqrt{T\log T})$ \\
    Arm 1 / Type 0      & $O\left(\frac{\log T}{(\tau \Prob_{\cP_0}[\theta \geq \tau] - \nu)^2}\right) +O(\sqrt{T\log T})$\\
    Arm 1 / Type 1      &  $O(\sqrt{T\log T})$ \\
    \bottomrule
    \end{tabular}
    
    \label{tab:type-specific-regret}
\end{table*}
\end{restatable}
We recall Lemma \ref{lemma:expost-regret}:
\expostregret*

\begin{proof}
From Theorem \ref{thm:treatment-approximation-bound}, the \textit{clean event} $\cC_1$ happens with probability at least $1 - \abs{\theta}$ for some $\abs{\theta} \in (0,1)$. Hence, the probability of $\neg \cC_1$ is at most $\abs{\theta}$. The probability of not getting an arm 1 sample in each phase, $\neg \cC_2$ is $\abs{\theta}'$. Hence, the expected ex-post regret conditional on $\neg \cC$ is at most $T (\abs{\theta} + \abs{\theta})'$.\\
Assume that $\cC$ holds. Observe that since $\cC$ holds, we have $\abs{\theta} \leq |\hat{\theta}_q| + s_q$ where $s_q$ is the decision threshold of phase $q$. Before the stopping criteria is invoked, we also have $|\hat{\theta}_q| \leq s_q$. Let $n$ be the number of samples used to estimate $\hat{\theta}_q$.
%This, combined with the fact that the number of recommendations $m$ equals the number of arms $k$, gives us that the empirical estimate $\hat{\Gamma}_t$ is the $m$-dimensional identity matrix at any round $t$. Thus, the minimum singular value $\sigma_{\min}(\hat{\Gamma}_t) = 1$. Then, during each iteration of the main loop, we have:
% \begin{align}
%     \abs{\theta} \leq 2 s_q &= 384\sqrt{\frac{\log(3T/\delta) + 3\log(2T(2+\Upsilon^2))}{q}}
%     \label{eq:delta-bound}
% \end{align}
Hence, we have: 
\begin{align*}
     &\quad\abs{\theta} \leq 2 s_q =  \frac{\left(16\sigma_{\eps}+16\Upsilon\right)\sqrt{2n\log(6T/\delta)}}{np_0-\sqrt{n\log(6T/\delta)}}\\
     \Rightarrow &\frac{\abs{\theta}}{16(\sigma_\epsilon + 2\Upsilon)\sqrt{2\log(6T/\delta)}} \leq \frac{1}{\sqrt{n} - \sqrt{\log(6T/\delta)}}\\
     \Rightarrow &n \leq \frac{512(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta}^2 p_0^2} + \frac{\log(6T/\delta)}{p_0^2}  + \frac{32\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{\abs{\theta} p_0^2}
\end{align*}
Therefore, the main loop must end by when the phase length is  
\begin{align*}
    n = \frac{512(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta}^2 p_0^2} + \frac{\log(6T/\delta)}{p_0^2}+ \frac{32\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{\abs{\theta} p_0^2}
\end{align*}
During the racing stage, each phase we give out $2h$ recommendations for the two arms sequentially, so each arm gets recommended $n/2$ times. If arm 0 is indeed the best arm, then on average, the regret for each phase is $0.75 n \abs{\theta}$. If arm 1 is the best arm, then on average, the regret for each phase is $0.25 n \abs{\theta}$. Conditional on event $\cC$, the arm $a^*$ at the end of the racing stage is the best arm so no more regret is collected after the racing stage is finished. Sine we are doubling the phase length after each phase, the total length of the racing stage is upper bounded by $2n$, where $n$ is the biggest phase length of the racing stage.  \\
Then, if arm 0 is the best arm, the total accumulated regret for the racing stage is 
\begin{align}
\label{eq:regret-arm-0}
    R_2(T) &\leq \frac{768(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta} p_0^2} + \frac{1.5\log(6T/\delta)\abs{\theta}}{p_0^2} + \frac{48\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{p_0^2}
\end{align}
On the other hand, if arm 1 is the best arm, the total accumulated regret for the racing stage is 
\begin{align}
\label{eq:regret-arm-1}
    R_2(T) &\leq \frac{256(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta} p_0^2} + \frac{0.5\log(6T/\delta) \abs{\theta}}{p_0^2} + \frac{16\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{p_0^2}
\end{align}
Observe that the ex-post regret for each round $t$ of the entire algorithm (both the sampling stage and the racing stage) is at most that of the racing stage plus $\abs{\theta}$ per each round of the sampling stage. Alternatively, we can also upper bound the regret by $\abs{\theta}$ per each round of the algorithm. Therefore, we can derive the ex-post regret for the entire algorithm:
If arm 0 is the best arm, then the total regret of both Algorithm
\ref{alg:sampling-control-treatment} and Algorithm \ref{alg:racing-two-types-mixed-preferences} is:
\begin{align}
    R(T) &\leq \min \Bigg \{L_1 \abs{\theta} + \frac{768(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta} p_0^2} + \frac{1.5\log(6T/\delta)\abs{\theta}}{p_0^2} \\
    &\hspace{2cm}+ \frac{48\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{p_0^2}, T\abs{\theta} \Bigg \}\\
    &\leq L_1 + O(\sqrt{T\log(T/\delta)}) 
\end{align}
If arm 1 is the best arm, then the total regret of both Algorithm 
\ref{alg:sampling-control-treatment} and Algorithm \ref{alg:racing-two-types-mixed-preferences} is:
\begin{align}
    R(T) &\leq \min \Bigg \{L_1 \rho \abs{\theta} + \frac{256(\sigma_\epsilon + 2\Upsilon)^2\log(6T/\delta)}{\abs{\theta} p_0^2} + \frac{0.5\log(6T/\delta) \abs{\theta}}{p_0^2} \\
    &\hspace{2cm}+ \frac{16\sqrt{2} (\sigma_\epsilon + 2\Upsilon)\log(6T/\delta)}{p_0^2}, T\abs{\theta} \Bigg \}\\
    &\leq L_1 \rho + O(\sqrt{T\log(T/\delta)}) 
\end{align}
\end{proof}}

\input{regret}

==> files/paper/type-specific-regret.tex <==
From the analysis in \Cref{lemma:expost-regret}, we can derive the type-specific pseudo-regret for each type of agent. Since policy $\pi_c$ does not guarantee that all agents follow our recommendation, this pseudo-regret analysis is divided into two cases, depending on the best arm overall. If we assume that proportions of each type in the population are equal, \cref{lemma:type-specific-regret} below demonstrates the type-specific pseudo-regret guarantee of our algorithm.
\begin{restatable}[Type-specific regret]{lemma}{typespecifictwoarms}\label{lemma:type-specific-regret}
\Cref{alg:sampling-control-treatment,alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ and known constant $\tau \in (0,1)$ such that $\tau \Prob_{\cP_i}[\theta \geq \tau] > 0$ achieves type-specific regrets in \cref{tab:type-specific-regret}.
\begin{table*}[ht]
    \centering
    \caption{Type-Specific pseudo-regret for Two Arms \& Two Types with partially BIC Algorithm}
    \begin{tabular}{ll}
    \toprule
    Best arm / Type     & Type-specific pseudo-regret \\
    \midrule
    Arm 0 / Type 0     & $O\left(\frac{\log T }{(\tau \Prob_{\cP_0}[\theta \geq \tau])^2} \right) + O(\sqrt{T\log T})$\\
    Arm 0 / Type 1      & $O\left(\frac{\log T}{(\tau \Prob_{\cP_0}[\theta \geq \tau])^2} \right) + O\left(\frac{\log T}{(\tau\Prob_{\cP_1}[\theta < -\tau])^2}\right) + O(\sqrt{T\log T})$ \\
    Arm 1 / Type 0      & $O\left(\frac{\log T}{(\tau \Prob_{\cP_0}[\theta \geq \tau])^2}\right) +O(\sqrt{T\log T})$\\
    Arm 1 / Type 1      &  $O(\sqrt{T\log T})$ \\
    \bottomrule
    \end{tabular}
    
    \label{tab:type-specific-regret}
\end{table*}
\end{restatable}
\dndelete{
\begin{proof}
See Appendix \ref{sec:type-specific-regret-proof} for a proof.
\end{proof}
}

\lsdelete{
\begin{definition}\label{def:fully-bic-algo}[Fully BIC Algorithm]
A \textit{fully BIC} algorithm is BIC for all agents at all rounds, similar to the detail-free algorithm in \cite{mansour2015bic}. We implement the sampling stage sub-algorithm~\eqref{alg:sampling-control-treatment} to be BIC for agents of type 0. Then, we run the racing stage sub-algorithm~\eqref{alg:racing-two-types-mixed-preferences} starting from the second racing stage, wherein recommendations are BIC for all agents.
\end{definition}

\begin{remark}[Regret Comparison Between Fully BIC and Partially BIC Algorithms]\label{remark:regret-comparison-2-arm}
The type-specific pseudo-regret for the fully BIC algorithm (\cref{def:fully-bic-algo}) is the same as the type-specific pseudo-regret for our partially BIC algorithm (see Table~\ref{tab:type-specific-regret}) wherein we replace the prior-dependent constant term $\tau^2 \Prob_{\cP_0}[G \geq \tau]$ for type 0 with the prior-dependent constant term $\tau^2 \Prob_{\cP_1}[G < -\tau]$ for type 1, which can be arbitrarily large. In the full version of our paper, we work out a case wherein the priors over the treatment reward $\theta$ for each type are Gaussian and the fully BIC algorithm (\cref{def:fully-bic-algo}) achieves linear pseudo-regret $\Omega(T)$, but our algorithm achieves sub-linear pseudo-regret $O(\sqrt{T\log T})$.
\end{remark}
}%end lsdelete

==> gaussian.tex <==
\subsection{Example: Gaussian priors}
To make the advantage of our algorithm compared to a fully incentive-compatible algorithm clear, we present an example where the prior of each type over the treatment effect of each arm is a Gaussian distribution, and the realized reward $y$ is normally distributed conditional on the treatment effect. We use $\cN(\mu, \sigma^2)$ to denote a Gaussian distribution with mean $\mu$ and variance $\sigma^2$. Through this example, we demonstrate an extreme setting where the length of the sampling stage for a fully BIC algorithm is arbitrarily large and the regret accumulated is linear, while our partially BIC algorithm still achieves sub-linear regret.\\ 
\begin{restatable}[Gaussian Regret Comparison]{example}{gaussian}\label{ex:gaussian}
Assume priors $\cP_1, \cP_2$ are independent across arms:
\begin{enumerate}
    \item $\cP_i$: $\theta \sim \cN(\mu_i, \sigma_i^2)$ with type $i\in\{0,1\}$; and
    \item $g(u_i) \sim \cN(\mu_g^i, 1)$, and $\mu_g^i \sim \cN(c, 1)$.
\end{enumerate}
Also assume that the action $X_t$ at round $t$ is chosen according to the selection function $f(z_t,t)$. Formally, the selection function is given as:
\begin{equation}
    \label{eq:gaussian-selection-function}
    X_t = f(z_t, t) := \1\left[ \E_{\mathcal{P}_t}\left[\theta \ | \ z_t, t \right] > 0 \right]
\end{equation}
Remember that the event $\xi$ is defined as 
\begin{small}
\begin{equation}
    \xi = \bigg\{ \bar y_1 > \bar y_0 + \sigma_g\bigg(\sqrt{\frac{2\log(2/\delta)}{\ell_0}} +\sqrt{\frac{2\log(2/\delta)}{\ell_1}}\bigg) +  G^{(0)} + \frac{1}{2}\bigg\}
\end{equation}
\end{small}
where $G^{(0)}$ is an upper bound on the expected value $\E_{\cP^{(0)}}[g^{(1)}-g^{(0)}]$, and $\sigma_g$ is the variance parameter for $g^{(0)}$ and $g^{(1)}$. 
Suppose the following, for some constant $\tau \in (0,1)$:
\begin{enumerate}
    \item the probability that for agents of type 2, the sample average of arm 1 in the sampling stage is sufficiently worse than the prior mean reward of arm 2, i.e. 
    \[\Prob_{\cP_2}[\xi_2] = \int_{-\infty}^{\zeta^2} \frac{1}{\sqrt{2\pi}} \exp\left(\frac{-1}{2}u^2\right) du > \frac{1}{\sqrt{\log(T)}},\] 
    and the z-score \[\zeta^2:=(\mu^2_2-\mu^1_2)\left(\sigma^2_{1,2}\frac{L_2 \sigma^2_{1,2}}{\rho^2_{1,2} + L_2 \sigma^2_{1,2}}\right)^{-1/2};\]
    
    \item the probability that for agents of type 1, arm 2 is sufficiently better than arm 1, i.e. \[\Prob_{\cP_1}[\theta^2 - \theta^1 > \tau] = \int^\infty_{\zeta_1} \frac{1}{\sqrt{2\pi}} \exp\left(\frac{-1}{2} u^2\right) du < \frac{1}{\sqrt{T}},\] 
    and the z-score 
    \[\zeta_1 = \frac{\mu^2_1 - \mu^1_1 - \tau}{\sqrt{\sigma^2_{1,1} + \sigma^2_{2,1}}}; \  \text{ and} \]
    
    \item the probability that for agents of type 2, arm 2 is sufficiently better than arm 1, i.e.
    \[\frac{1}{\sqrt{\log(T)}} > \Prob_{\cP_2}[\theta^2 - \theta^1 > \tau] = \int^\infty_{\zeta_2} \frac{1}{\sqrt{2\pi}} \exp\left(\frac{-1}{2} u^2\right) du > \frac{1}{\sqrt{T}},\] 
    and the z-score 
    \[\zeta_2 = \frac{\mu^2_2 - \mu^1_2 - \tau}{\sqrt{\sigma^2_{1,2} + \sigma^2_{1,2}}}.\]
\end{enumerate}

With these assumptions, the regret of a fully BIC algorithm is $O(T)$ and the regret of our partially BIC algorithm is $O(\sqrt{T\log(T)})$.
\end{restatable}

==> intro.tex <==
\section{Introduction}


\swcomment{

\begin{itemize}
    \item Related work.
    \item describe how this model can still be viewed as an MAB problem if we have fully BIC---that is, we average out the baseline reward across types
\end{itemize}


}




In many online recommendation systems, e.g. those used by Netflix, Amazon, Yelp, Stubhub, and Waze, users are both consumers and producers of information. Users make their selections based on recommendations from the system, and the system collects data about the users' experiences to provide better-quality recommendations for future users. To ensure the quality of its recommendations, the system typically needs to balance between \emph{exploration}---selecting potentially suboptimal options for the sake of acquiring new information---and \emph{exploitation}---selecting the best option given the available information. However, there is an inherent tension between exploration and users' incentives: since each user is primarily concerned with their short-term utility, their incentives naturally favor exploitation. 

To resolve this tension between exploration and exploitation, a long line of work started by~\cite{KremerMP13, mansour2015bic} has studied mechanisms that incentivize users to explore by leveraging the information asymmetry between the recommendation system and users \citep{MansourSSW16, ImmorlicaMSW19, SS20}. These papers consider a multi-armed bandit model where the recommendation system is a \emph{social planner} who interacts with a sequence of self-interested \emph{agents}. The agents arrive one-by-one to choose from a given set of actions (or ``arms'') and receive a reward for their choice. Upon the arrival of each agent, the social planner provides a recommendation (of one of the actions) that influences the agent's selection. The problem is to design a recommendation policy that incentivizes the agents to explore and in the long run maximize the cumulative rewards of all the agents, even when the agents want to exploit.

Prior work on \textit{incentivizing exploration} typically approaches the problem by enforcing \emph{Bayesian incentive-compatibility} (BIC) for every agent---that is, the planner recommends actions which it is in each agent's interest to follow, even if such action is be inferior according to the agent's prior belief. To achieve BIC, a recommendation mechanism typically needs to make strong assumptions that 1) all of the agents share a \emph{common prior} over the rewards of actions and 2) all agents will \emph{comply} with each recommendation. However, in reality, agents tend to be heterogeneous in terms of their beliefs and perceived rewards; as such, some may comply with a recommendation and some may not. In particular, some agents can have a stronger \emph{bias} that favors one action over others. Moreover, even if the actions have the same effect or reward for all agents, their realized or observed utilities can be different. For example, different patients taking the same drug may report levels of pain and different drivers taking the same route may have different commute time.

\begin{example}[Motivating Example: Sales Campaign] A bank wants to estimate the return on investment (ROI) of a sales intervention wherein a salesperson offers a high rate of return on a savings account if a client deposits a large sum of money into the account.

On each day $t$, a client is assigned a particular sales person, who may or may not take the intervention. If the salesperson offers the intervention ($x_t=1$ in our model) the bank incurs a cost $c_t$ to pay out on the savings account (which is given by the rate of return and the deposit amount) and generates revenue $r_t$, since the clients may be more likely to open up other accounts, e.g. credit cards or investment accounts, which generate profit over time. If the salesperson takes the control  ($x_t=0$ in our model), the cost and revenue are zero. In our model, the population return caused by the intervention is given by $\theta = \E[r_t-c_t | x_t=1]$ and the instances of $r_t-c_t$ are randomly given by $\theta x_t + \epsilon_t$.

As such, the bank could estimate the return $\theta$ caused by the intervention by simply calculating the mean return under the intervention or the control. However, the clients also generate some baseline revenue, which is independent from the sales intervention. This baseline revenue $g(u_t)$ is given by the client’s \textit{type} ($u_t$ in our model), which also determines the salesperson’s expectation of the cost and revenue of the sales intervention. For example, the client’s type could be that they're a wealthy law firm with a lot of investable assets: the client generates high baseline revenue because they have a lot of money invested in the bank, of which the bank takes a percentage fee; as well, the salesperson anticipates that the law firm will deposit a lot of money into the savings account --incurring high cost $c_t$-- without opening any additional accounts --low revenue $r_t$.

Notably, the bank only observes whether or not the salesperson takes the intervention and the net revenue $y_t$ (given in equation~\eqref{eq:reward-model}). Since the unobserved baseline revenue $g(u_t)$ is correlated with the salesperson’s choice $x_t$, this causes confounding and the bank can no longer estimate the intervention return by simply taking the mean.

As such, the bank deploys a daily recommendation platform for the sales team, so as to optimize the bank's overall net revenue. Each day, the recommendation $z_t$ is based on the history $H_t$ of the intervention, i.e. all the past recommendations $z_t$, actions taken $x_t$, and the net revenues $y_t$.

Each salesperson $t$, considers this recommendation and their prior belief about the expected net revenue caused by the sales intervention, to decide whether to take the intervention or not, as in equation~\eqref{eq:two-arm-general-selection-function}. \lscomment{The recommendation may sway some risk-averse salespeople to take the intervention and some risky salespeople to take the control, causing more variability over the types.} The bank uses the recommendation $z_t$ as an instrument to better estimate the net revenue caused by the intervention $\theta$, as we expand upon in the following section.

\lscomment{End of bank example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse

Consider a corporation that  wants to estimate the average effect of interventions that the sales team can take on their customers (e.g. outreach phone calls, offering discounts or free credits), on the revenue of their customers. The corporation wants to deploy a daily recommendation platform for the sales team, so as to optimize operations and learn best practices. We consider a simplified setting where there is only a single type of intervention and the corporation does not know its return on investment (ROI). On each day $t$, a customer is assigned a particular sales person, who may or may not take the intervention. We assume that the effect of the intervention is observed at the end of the day (e.g. whether a purchase was made; this can also be replaced by some other short-term proxy/signal of long-term revenue, if long-term revenue is the goal).\footnote{The setting can also be easily relaxed with batches of customers each day (this can be thought as a method of online experimentation and active learning from the corporation).} The corporation is trying to identify the net effect of the intervention: this corresponds to some revenue lift $\delta$ minus a (potentially known) intervention cost $c$.

We model this scenario as bandits learning of two actions, where action 1 is "not taking intervention" and action 2 is "taking intervention". Then the net effect of the intervention is $\theta^2 = \delta - c$. Moreover, when no intervention is taken, then no lift in the revenue is observed and no cost is paid, rather the customer is expected to generate an organic, baseline amount of revenue $g(u_t)$, and so $\theta^1 = 0$. Here $u_t$ is an unobserved type of the customer, that is not known to the principal, but is observed by the sales person. This signal $u_t$ essentially captures the information asymmetry of the setting: sales people know more about the customers that they are working with than the corporation (e.g. whether they are about to grow, whether they are about to sign a big contract, whether they are about to make a big purchase because of increase in demand on the customer side). So at the end of the day, the customer generates revenue:
$y_t = \theta^{a} + g(u_t) + \epsilon_t$,
where $a\in \{1, 2\}$. The information asymmetry (i.e. that the agents know $u_t$ but the principal doesn't) is exactly what causes the endogeneity problem in the choice of the agents and why an instrumental variable approach is necessary. The goal of the principal is to maximize revenue, or more concretely minimize expected regret in terms of revenue, i.e.:
\begin{equation}
    R(T) = T\theta^{a^*} - \sum_{t} \theta_t^{X_t} 
\end{equation}
where $a^*=1$ if $\delta<c$ and $a^*=2$ if $\delta\geq c$.

The principal does not know the ROI $\theta^2$, and as is typical in corporate settings, will compensate the salesperson as a fraction of the observed revenue $y_t$, whenever an intervention is made.\footnote{Potentially this compensation structure could change once the ROI is estimated by the principal, which would then remove the endogeneity problem, but until the ROI is pin-pointed, this is a typical compensation schemes in corporate settings.} Thus, the salesperson receives reward:
\begin{equation}
    r_t = \beta\, y_t
\end{equation}
for some $\beta\in (0, 1]$. We also assume that each sales person has some outside option of collecting a reward $\pi$ (e.g. by doing what they would normally be doing and not following the principals recommendation). Thus the salesperson will take the action $a=1$ only if they expect a positive net benefit:
\begin{equation}
    X_t = 1 + \1\left\{\E_{\theta\sim \cP}[\theta^2] + g(u_t) \geq \pi/\beta\right\} = 1 + \1\left\{\E_{\delta\sim \cP}[\delta] - c + g(u_t) \geq \pi/\beta \right\} 
\end{equation}

In the case of two types $u_t\in \{1, 2\}$, We will also assume for simplicity that a priori both types will prefer to take the intervention. However, we assume that there is a probability under their prior beliefs that $\theta^2+g(u_t) \leq \pi/\beta$ for both types. At the end of the day the principal and the salesperson observe $y_t=\theta^a + g(u_t) + \epsilon_t$. This example is a special case of our framework, where $\theta^2=\delta - c$ and all agents have a uniform prior $\cP$ on $\delta$, with $c$ known. Moreover, $\phi(u_t)=\pi/\beta + c - g(u_t)$, for a known $\pi$, but a type $u_t$ unobserved by the principal and only observed by the agent.\fi

\end{example}


To explicitly capture the underlying heterogeneity across agents, we study a new model in which each agent has unobserved private type that determines both their prior preferences across the actions and their action-independent confounding shift in the rewards. Since the heterogeneity of the agents confounds the observed rewards, we draw techniques from instrumental variable regression to estimate the reward effects across the actions.
In particular, we take a novel view that  the planner’s recommendations can serve as a form of instrumental variables (IV) that only affect agents’ arm selection but not the observed rewards. We construct such IVs by carefully mapping the history–the interactions between the planner and the previous agents to a random recommendation. By running IV regression, our mechanism obtains a reliable estimate of reward effect of each action and in turn incentivize the agents' selections to converge on the optimal action.

A major advantage of our IV-based mechanism is that we no longer need to enforce BIC for all agents. Our algorithm can estimate the action effects accurately, as long as the recommendations induce variability in the agents' selections. An important special case is when a fraction of the types are more willing to explore an action that a priori inferior. Furthermore, as soon as the mechanism obtains a sufficiently accurate estimate on the action effects, the policy can then be BIC for the remaining types. We demonstrate such partially BIC policy can significantly improve the regret bounds of a fully BIC policy obtained by extending the algorithm of \cite{mansour2015bic} to our setting. Moreover, our IV-based mechanism also mitigates the negative externality that their fully BIC policy imposes on a subgroup of agents. The reason is that their fully BIC policy will necessarily impose a longer exploration phase on agents of all types, which incurs unnecessary additional regret on agents who are more willing to follow the planner's recommendations. Since our IV-based mechanism does not require fully BIC to obtain accurate estimates, it also mitigates such unfair externality.

\paragraph{Additional motivating examples}
The trade-off between exploration and exploitation in the bandit setting could be observed in various scenarios that highlights the need for a natural instrument to help estimate the reward of each arm.\\
One such scenario concerns the lending discriminatory of a bank to different businesses, big and small. A bank is trying a sales campaign where a loan officer can offers a business client a low interest loan as an intervention. If they offer the loan, the bank incurs cost based on how much money the business takes out and if they default. Businesses generate baseline revenue that depends on its type and is independent of the intervention, i.e. big businesses already have more investment with the bank. so they generate more revenue regardless of the loan offer. Whether the loan officer offers the loan depends on the business type: they are biased against small businesses since they are more likely to default. The intervention choice is correlated with the baseline revenue and causes confounding effect. This calls for an instrument, which in this case is the bank's recommendation, to accurately estimate the effectiveness of the loan. By giving recommendation to induces variability, the bank can incentivizes loan officers to lend to small businesses. Thus, we can also prevent the discrimination against one type of business in this setting. 

\subsection{Related Work}




\textbf{Organization.} In this workshop version, we will present our formal model (Sec.\ref{sec:model}) and illustrate key ideas of our mechanism in a simple setting of two private types and two arms (Sec. \ref{sec:two-arms-two-priors}). We defer the fully general results and details to the full version.


\swdelete{Our work applies instrument variable (IV) regression \citep{angrist2001iv, angrist1995tsls,angrist1996iv} in a multi-armed bandits setting \citep{auer2002mab,katehakis1987mab,slivkins2019bandits}. We use IV regression because it yields consistent causal effect estimates in the presence of confounding, unlike OLS or ANOVA. We consider a more general setting than the model considered in \citep{mansour2015bic}, because we consider these confounding effects. Particularly, our model and algorithm accommodates for heterogeneous priors, noncompliance, and binary treatment effect estimation; those in \citep{mansour2015bic} do not. Both \citep{Kallus2018InstrumentArmedB} and \citep{bareinboim2015causal} consider confounding in multi-armed bandits settings. However, \citep{bareinboim2015causal} does not consider incentive-compatibility nor do they employ IV regression. 
\dndelete{\cite{Kallus2018InstrumentArmedB} uses IV regression in a Bayesian bandits setting, but they consider an entirely different ``instrument-armed bandit'' problem that does not consider incentivizing agents.}

The compliance mapping is fixed: it doesn't change as the learner collects more information.
The reward model doesn't capture the confounding effect: for Kallus states that ``When the treatment applied is x, the reward observed is Y (x)''.

\lscomment{Kallus only considers regret for compliant type. In comparison, since all agents may become compliant in our setting, we can achieve sublinear regret in comparison to the best arm for all types of agents.}

\citet{Kallus2018InstrumentArmedB} also studies how to leverage instrumental variables in a multi-armed bandits setting, where social planner provides arm recommendations to agents who may choose an arm different from the recommendation. However, there are many differences. First, our model allows the agents' compliance to change over time according to the agents' reward motives and signals about the history of the performance of each arm, \citet{Kallus2018InstrumentArmedB} only considers the case where agent compliance is stationary over time even when the social planner has an accurate estimate of the rewards. In our setting, the social planner can leverage the collected data to  convince any agent (who may be initially noncompliant) to follow our recommendations. 
As a result, the regret notion in our setting is also different from that of 
\citet{Kallus2018InstrumentArmedB}. \swcomment{explain the different notion of regret? } We also consider this kind of noncompliance, as well as some additional confounding effects. 


Because noncompliance allows for agents to choose different arms than the social planner recommends, \citet{Kallus2018InstrumentArmedB} considers four alternative notions of regret:
\begin{enumerate}
    \item \emph{Static Treatment Regret} considers only the difference between the chosen actions and the best action in hindsight, disregarding the recommendations. \lscomment{This just sounds like regular regret??}
    \item \emph{Intent-to-Treat (ITT) Regret} considers the difference between the recommendations and the single best recommendation in hindsight (i.e. the recommendation for the arm with the highest expected reward), disregarding the arms that the agent actually chooses.
    \item \emph{Latent-Class Treatment Regret} considers the difference between the chosen actions and the best action in hindsight for a given type of agent. \lscomment{I don't really get this one. But, it seems like this accommodates for heterogeneous treatment effects? Though, Kallus just considers types to be fully compliant, never compliant, and partially compliant?} 
    \item \emph{Compliers' Regret} considers the regret only for agents who comply with the recommended action.
\end{enumerate}

Under ITT regret, ``one does not seek to select or identify the best treatment'' because minimizing ITT regret does not entail minimizing the regret given by finding the best treatment \cite{Kallus2018InstrumentArmedB}. 

\citet{Kallus2018InstrumentArmedB} prefers Compliers' Regret.

In our setting, Latent-Class Treatment Regret does not apply, because we consider only homogeneous treatment effects. Minimizing ITT Regret ``does not seek to select or identify the best treatment''. Compliers' Regret is strictly weaker than our notion of regret which considers all agents, regardless of compliance. Primarily, we consider the standard notion of regret ---the difference between the rewards from the chosen actions over rounds and the single best reward in hindsight. \lscomment{(I think Kallus calls this the Static Treatment Regret.)}

 \dndelete{This allows us to achieve better type-specific regret.} \lscomment{should we say ``type-specific'' here... seems too jargony to bring up now...} Furthermore, accounting for this change in compliance is more realistic, because agents can reason about the recommendation systems' effectiveness and update their beliefs accordingly.

\lsdelete{
who investigates different notions of regret in a setting where the action choice and reward observed do not capture the confounding effect. We formally define both the reward and the agents' action choice formulations and show the need for an instrument because of the confounding effect. Kallus only consider the case where the compliance types are fixed and stationary, while we allow the agents' compliance to change throughout our algorithm. After collecting sufficient data, we can convince agents who are initially noncompliant to follow our recommendation, which allows us to achieve better type-specific regrets. Furthermore, accounting for this change of compliance is more realistic because agents can reason about the recommendation systems' effectiveness and update their beliefs accordingly. 

In this work, they study a . However, their model and algorithm cannot accommodate for non-compliance and confounding in a Bayesian bandits setting nor treatment effect estimation with a control variable. By contrast, we explicitly model confounding in a control-treatment setting, which allows us to model non-compliance in our specific setting. Additionally, our model and algorithm may be generalized to the fully-compliant bandits setting that \cite{mansour2015bic} consider. Thus, our work covers a more general setting.

Bayesian Incentive Compatible (BIC) Bandit problems are a variant of the incentivized bandit exploration problem with an additional constraint on the prior of agents \cite{mansour2015bic}. In the BIC bandit problem, a social planner gives out recommendations to incentivize the agents to either explore or exploit to maximize the total rewards \cite{mansour2015bic}. The agents are assumed to be self-interested individuals who want to maximize their reward from each round. It is up to the social planner's recommendation policy to ensure that the agents are still choosing the arm that maximizes their benefits while exploring different arms to find the highest reward. This problem can be reduced to the traditional MAB problem with stochastic rewards without the incentive-compatible constraint. The Bayesian part of this problem comes from the agents' Bayesian priors, onto which we perform updates using the history of observed rewards.

Bayesian Incentive Compatible Bandit provides a realistic setting for medical trials. While it might be tempting to offer external incentives (such as monetary payment) to ensure compliance with the recommendation, such practice could result in selection bias. For example, more indigent patients would be more willing to explore different arms if given monetary payment. The data set would then represent the actions and reward for these people, instead of the general population. Hence, it is worthwhile to investigate an incentive-compatible algorithm that is less prone to such error and mitigates negative externality caused by one type of agent on another.}

Prior work on \textit{incentivizing exploration} typically approaches the problem by enforcing \emph{compliance} (or \emph{Bayesian incentive-compatibility}) for every agent ---that is, the planner recommends actions which it is in each agent's interest to follow, even if such action is inferior according to the agent's prior belief. To achieve full compliance, a recommendation mechanism typically needs to make strong assumptions that 1) all of the agents share \lsdelete{a \emph{common prior} over the rewards of actions}\lsedit{the same \emph{prior preferences} over the rewards of all actions} and 2) all agents will \emph{comply} with every recommendation. However, in reality, agents tend to be heterogeneous in terms of their beliefs and perceived rewards; as such, some may comply with a recommendation and some may not. In particular, some agents can have a stronger \emph{bias} that favors one action over others. Moreover, even if the actions have the same effect or reward for all agents, their realized or observed utilities can be different. For example, different patients taking the same drug may report different levels of pain and different drivers taking the same route may have different commute times.}


==> multi-arm-case.tex <==
\newpage
\section{Multi-arm case - Heterogeneous beliefs}
Assumption: 
\begin{itemize}
    \item The social planner knows about a bound on each agent's confounder $u_t$: $\abs{g(u_t)} \leq \Upsilon$. 
    \item The entire population of agents has two types, each with its own common prior, namely $\cP_1$ and $\cP_2$, on the distribution of the mean reward vector $\theta$.
    \item The prior mean reward of arms $1$ through $m$ are $\theta_0^1,\ \theta_0^2,\ \dots,\ \theta_0^m$, respectively and $\theta^1_0 \geq \theta^2_0 \geq \dots \geq \theta^m_0$ for all agents.
    \item The social planner knows the ordering of the arms according to their prior mean rewards.
    \item The prior is independent across arms.
\end{itemize}
Denote $C = \Upsilon + \sigma_{\epsilon}\sqrt{\frac{2\ln(1/\delta)}{L_1}}$.\\ 
  
\begin{algorithm}[H] 
\SetAlgoLined 
\SetKwInput{KwIn}{Input}
\KwIn{parameters $L_1, \rho \in \mathbb{N}$}
\KwIn{Sample average of reward $y^1$ after $L_1$ pulls of arm $1$, denoted $\bar{y}^1_{L_1}$}
    \For{each arm $i > 1$ in increasing lexicographic order}{
    \eIf{$\displaystyle \theta_0^i > \bar{y}^1_{L_1} + C$ and $\bar{y}^1_{L_1} + C < \bar{y}^j_{L_1}$ and $ \bar{y}^j_{L_1} + C < \theta^i_0$ for all arms $1 < j <i$} 
    {$a^*_i = i$} 
    {$a^*_i = 1$}
    From the set $P$ of the next $L_1.\rho$ agents, pick a set $Q$ of $L_1$ agents uniformly at random.\\
    Every agent $p \in P - Q$ is recommended arm $a_i^*$.\\
    Every agent $p \in Q$ is recommended arm $i$.\\
    Let $\bar{y}^i_{L_1}$ be the average reward among the agents in $Q$.
    }
    \caption{The sampling stage for multiple arms}
    \label{alg:multi-arm-sampling} 
\end{algorithm}

\begin{lemma}
Consider BIC bandit exploration with $m$ arms. The algorithm above with parameters $(\rho, L_1)$ completes in $L_1\rho(m - 1) + L_1$ rounds. Consider the event 
\begin{equation}
    \hat{\xi}_i = \left\{ \bar{y}^1_{L_1} + C < \min_{1 < j < i} \bar{y}^j_{L_1} - C \text{and } \max_{1 \leq j < i} \bar{y}^j_{L_1} + C < \theta^i_0 \right \}
\end{equation}
and let event $\hat{\xi}$ be such that $\Prob[\hat{\xi}] = \min_i \Prob[\hat{\xi}_i]$. \\
The algorithm is BIC if we have the assumptions above and $\theta_0^i > 0$ for all $1<i\leq m$, and the parameters satisfy: 
\begin{equation}
    \rho \geq 1 + \frac{\theta^1_0 - \theta^m_0}{(\Upsilon + 2\sigma_{\epsilon})\sqrt{\frac{2\ln(3/\delta)}{L_1}} \Prob[\hat{\xi}]}
\end{equation}
where $g(u_i) \in [-\Upsilon, \Upsilon]$.
\end{lemma}
\begin{proof}
Observe that agent $p$ in phase $i$ of the algorithm is recommended either arm 1 or arm $i$. We need to prove incentive-compatibility for the two cases separately.\\
Let $\hat{\xi}_{i}$ be the event that the exploit arm $a^*_i$ in phase $i$ is $i$. Formally, we define:
\begin{equation} 
    \hat{\xi}_i = \left\{ \bar{y}^1_{L_1} + C < \min_{1 < j < i} \bar{y}^j_{L_1} - C \text{and } \max_{1 \leq j < i} \bar{y}^j_{L_1} + C < \theta^i_0 \right \}
\end{equation}
\begin{enumerate}[label = Part \Roman*:]
    \item \textbf{Recommendation for arm $i$}: We want to first argue that an agent $p$ who is recommended arm $i$ will not want to switch to any other arm $j$. For arms $j > i$, there is no information about arms $i$ or $j$ collected by the algorithm and by assumption, we have $\theta_0^i \geq \theta_0^j$. Hence, it suffices to consider when $j < i$. We want to show 
    \begin{align*}
        \E[\theta_0^i - \theta^j | z_t = e_i] \Prob[z_t = e_i] \geq 0 
    \end{align*}
    Agent $p$ is in the explore group $Q$ with probability $\frac{1}{\rho}$ and in the exploit group $P - Q$ with probability $1 - \frac{1}{\rho}$. Since being in the explore group does not confer any information about the mean rewards of any arm, the expected gain from choosing arm $i$ over arm $j$ conditional on the agent $p$ being in the explore group is $\theta^i_0 - \theta^j_0$. (Note that $\theta^i_0 - \theta^j_0 \leq 0$, since by definition $\theta^i_0 < \theta^j_0$ for all $j < i$.) If the agent is in the exploit group, then recommendation for arm $i$ implies that the event $\hat{\xi}_i$ has happened. Hence, we have:
    \begin{align*}
        \E[\theta_0^i - \theta^j | z_t = e_i]\Prob[z_t = e_i] = \E[\theta^i_0 - \theta^j |\hat{\xi}_i ]\Prob[\hat{\xi}_i] \left(1 - \frac{1}{\rho}\right) + \frac{\theta^i_0 - \theta^j_0}{\rho}
    \end{align*}
    For the algorithm to be incentive-compatible, we need to pick $\rho$ large enough such that:
    \begin{align}
        \E[\theta_0^i - \theta^j | \hat{\xi}_i]\Prob[\hat{\xi}_i]\left(1 - \frac{1}{\rho} \right) + \frac{1}{\rho}(\theta_0^i - \theta_0^j) &\geq 0 \nonumber\\
    	\E[\theta_0^i - \theta^j | \hat{\xi}_i]\Prob[\hat{\xi}_i] - \frac{1}{\rho}\E[\theta_0^i - \theta^j|\hat{\xi}_i] \Prob[\hat{\xi}_i] + \frac{1}{\rho}(\theta_0^i - \theta_0^j) &\geq 0 \nonumber\\
    	\rho\E[\hat{\xi}_i|\hat{\xi}_i]\Prob[\hat{\xi}_i] &\geq \E[\theta_0^i - \theta^j | \hat{\xi}_i]\Prob[\hat{\xi}_i] - (\theta_0^i - \theta_0^j) \nonumber\\
    	\rho &\geq 1 + \frac{\theta_0^j - \theta_0^i}{\E[\theta_0^i - \theta^j | \hat{\xi}_i]\Prob[\hat{\xi}_i]} \label{eq:multi-arm-L-condition}
    \end{align}
    This comes down to finding a lower bound on the denominator of the expression above. 
    Assuming that we know the prior and can calculate the probability of event $\hat{\xi}_i$, we can pick an appropriate $\rho$ to satisfy the BIC condition.
If the event $\hat{\xi}_i$ happens, we have 
\begin{align*}
    \theta^i_0 - \bar{y}^j_{L_1} &> \Upsilon +\sigma_{\epsilon}\sqrt{\frac{2\ln(1/\delta)}{L_1}}\\
    \theta^i_0 - \E[y^j] &> \Upsilon +\sigma_{\epsilon}\sqrt{\frac{2\ln(1/\delta)}{L_1}} + \frac{1}{L_1} \sum_{i=1}^{L_1} \left( \theta^j + g(u_i) + \epsilon_i \right) - \E[\theta^j] - \E[g(u)]\\
    \theta^i_0 - \E[\theta^j] - \E[g(u)] &> \Upsilon +\sigma_{\epsilon}\sqrt{\frac{2\ln(1/\delta)}{L_1}} + \left( \Upsilon\sqrt{\frac{2\ln(1/\delta_2)}{L_1}} + \sigma_{\epsilon}\sqrt{\frac{2\ln(1/\delta_3)}{L_1}} \right) \\
    \theta^i_0 - \theta^j &> \Upsilon + \sigma_{\epsilon}\sqrt{\frac{2\ln(1/\delta)}{L_1}} +  (\Upsilon+\sigma_{\epsilon})\sqrt{\frac{2\ln(2/\delta_y)}{L_1}} - \Upsilon\\
    \theta^i_0 - \theta^j &> (\Upsilon + 2\sigma_{\epsilon})\sqrt{\frac{2\ln(3/\delta)}{L_1}}
\end{align*} 
Hence, for the algorithm to be BIC, it is sufficient to pick:
\begin{equation}
    \rho \geq 1 + \frac{\theta^j_0 - \theta^i_0}{(\Upsilon + 2\sigma_{\epsilon})\sqrt{\frac{2\ln(3/\delta)}{L_1}} \Prob[\hat{\xi}_i]}
\end{equation}
Since we have $\theta^j_0 \leq \theta^1_0, \forall j$, it is sufficient to pick $j = 1$ in the inequality above.
\item \textbf{Recommendation for arm 1}: When agent $p$ is recommended arm 1, the agent knows that he is not in the explore group. Hence, the recommendation implies that the event $\neg\hat{\xi}_i$ happens. We want to show that for any arm $j > 1$:
\begin{equation}
    \E[\theta^1 - \theta^j | \neg\hat{\xi}_i] \Prob[\neg\hat{\xi}_i] \geq 0
\end{equation}
If an agent does not want to change to arm $j = i$, then he also does not want to change to any other arm $j > i$ due to lacks of information. Hence, it suffices to consider only arms $j \leq i$.\\
Observe that:
\begin{align*}
    \E[\theta^1 - \theta^j | \neg\hat{\xi}_i] \Prob[\neg\hat{\xi}_i] &= \E_{\theta \sim \cP}[\theta^1 - \theta^j] - \E[\theta^1 - \theta^j | \hat{\xi}_i]\Prob[\hat{\xi}_i]\\
    &= \theta^1_0 - \theta^j_0 + \E[\theta^j - \theta^1|\hat{\xi}_i]\Prob[\hat{\xi}_i]
\end{align*}
Since we have $\theta^1_0 \geq \theta^j_0$, it would suffice to show that:
\begin{equation}
    \E[\theta^j - \theta^1 | \hat{\xi}_i] \Prob[\hat{\xi}_i] \geq 0
\end{equation}
When the event $\hat{\xi}_i$ happens, we have:
\begin{align*}
    \hat{y}^j_{L_1} - \hat{y}^1_{L_1} &> \Upsilon + \sigma_{\epsilon}\sqrt{\frac{\ln(1/\delta)}{L_1}}\\
    \E[y^j] - \hat{y}^1_{L_1} &> \Upsilon + \sigma_{\epsilon}\sqrt{\frac{\ln(1/\delta)}{L_1}} - \left(\frac{1}{L_1}\sum_{i = 1}^{L_1} (\theta^j + g(u_i) + \epsilon_i) - \E[\theta^j] - \E[g(u_i)] \right)\\
    \E[y^j] - \E[y^1] &> \Upsilon + \sigma_{\epsilon}\sqrt{\frac{\ln(1/\delta)}{L_1}}\\
    \theta^j + \E[g(u)] - \theta^1 - \E[g(u)] &> \Upsilon + \sigma_{\epsilon}\sqrt{\frac{\ln(1/\delta)}{L_1}}\\
    \theta^j - \theta^1 &> \Upsilon + \sigma_{\epsilon}\sqrt{\frac{\ln(1/\delta)}{L_1}} > 0
\end{align*}
\end{enumerate}
We have proved that all recommendations in phase $i$ are BIC if we take
\begin{equation}
    \rho \geq 1 + \frac{\theta^1_0 - \theta^m_0}{(\Upsilon + 2\sigma_{\epsilon})\sqrt{\frac{2\ln(3/\delta)}{L_1}} \Prob[\hat{\xi}]}
\end{equation}
where $\Prob[\hat{\xi}] = \min_i \Prob[\hat{\xi}_i]$.
\end{proof}

%---------------------------------------%

%---------------------------------------%

\begin{algorithm}[H]
\SetAlgoLined
\SetKwInput{KwIn}{Input}
\KwIn{parameters $L_1 \in \mathbb{N}$; time horizon $T$; IV estimates of the mean rewards for each arm, denoted $\hat{\theta}^1_{L_1}, \dots,  \hat{\theta}^k_{L_1}$}
    Initialize set of active arms: B = \{ all arms \}.\\ 
    Split remainder into consecutive phases, starting from phase $q = L_1$;\\
    \While{$|B| > 1$}
    {
    Let $\hat{\theta}^i_{q}$ is the IV estimate of the reward of each arm $i \in B$ up to and including phase $q$;\\
    Let $\hat{\theta}^*_q = \max_{i \in B} \hat{\theta}_q^i$ be the largest average reward so far;\\
    Recompute $B = \left \{ \text{arms } i: \hat{\theta}_q^* - \hat{\theta}_q^i \leq 2m^{\frac{3}{2}}c_0 \sqrt{\frac{\ln(mT/\delta)}{q}} \right \}$;\\
    The next $|B|$ agents are recommended each arm $i \in B$ sequentially in lexicographic order;\\
    Let $y^i_q$ be the reward of each arm $i \in B$ in this phase;\\
    $q = q+1$;
    }
    For all remaining agents recommend $a^*$ that remains in $B$.
    \caption{The racing stage for multiple arms}
    \label{alg:multi-arm-racing}
\end{algorithm}
\begin{lemma} (Stopping Criteria)
\label{lemma:stopping criteria-multi-arm}
Given samples of the instrumental variable $z_t$ and response variable $y_t$ from $t$ rounds of the racing stage, we can derive the stopping criteria of the algorithm~\eqref{alg:multi-arm-racing} at round $t$:
\begin{align*} 
    |\hat{\theta}^*_q - \hat{\theta}^1_q| \leq 2m^{\frac{3}{2}}c_0 \sqrt{\frac{\ln(mT/\delta)}{q}}
\end{align*}
where 
     \begin{itemize}
         \item $c_0 \in \mathbbm{R}$ is some constant depending on $|g(u_i)|\leq \Upsilon$, $\sigma_{\epsilon}$, and $\max_i \theta^i \leq R$,
     \end{itemize}
\end{lemma}
\begin{proof}
For the algorithm~\eqref{alg:multi-arm-racing} to successfully find the better arm, we need the deviation bound of the two arms to not overlap. Let $\hat{\theta}^*_q = \max_{i \in B} \hat{\theta}_q^i$ be the largest average reward so far. Let the last phase that we did not invoke the stopping criteria for a particular arm $i$ be $q$, we have
\begin{align}
    \abs{\hat{\theta}^*_q - \hat{\theta}^i_q} \leq r_q^* + r_q^i
\end{align}
where $r_t^i$ is the deviation radius of arm $i$ at round $q$.
We also have:
\begin{align*}
    r_q^* + r_q^i &= |\hat{\theta}^*_q - \theta^*| + |\hat{\theta}^i_q - \theta^i|
\end{align*}
We have 
\begin{align*}
    2\norm{\hat{\theta}_q - \theta}_2 &\geq 2\norm{\hat{\theta}_q - \theta}_\infty\\
    &\geq |\hat{\theta}^*_q - \theta^*| + |\hat{\theta}^i_q - \theta^i|\\
    &\geq |\hat{\theta}^*_q - \hat{\theta}^i_q|
\end{align*} 
From Theorem ~\eqref{thm:finite-sample}, we have:
\begin{align*}
    \norm{\hat{\theta}_q - \theta}_2 &\leq  \frac{c_0}{\sigma_{\min}(\hat{\Gamma}_t)z_{\min}} \sqrt{\frac{m\ln(Tm/\delta)}{L_{\min}}}\\
    \Rightarrow |\hat{\theta}^1_q - \hat{\theta}^2_q| &\leq \frac{2c_0}{\sigma_{\min}(\hat{\Gamma}_t)z_{\min}} \sqrt{\frac{m\ln(Tm/\delta)}{L_{\min}}}\\
    &= \frac{2c_0}{\sigma_{\min}(\hat{\Gamma}_t)z_{\min}} \sqrt{\frac{m\ln(Tm/\delta)}{q}} \ \text{(since $L_{\min} = q$ in the racing stage)}\\
    &= \frac{2mc_0}{\sigma_{\min}(\hat{\Gamma}_t)} \sqrt{\frac{m\ln(Tm/\delta)}{q}} \ \text{(since $z_{\min} = 1/m$ in the racing stage)}
\end{align*}
where $c_0 \in \mathbbm{R}$ is some constant depending on $|g(u)| \leq \Upsilon$, $\sigma_{\epsilon}$, and $\max_i \theta^i \leq R$. In our setting, the number of recommendation is equal to the number of treatments so $m = k$. Also, we are guaranteeing agents' compliance through our recommendation policy, so $\sigma_{\min}(\hat{\Gamma}_t) = 1$. Hence, the stopping criteria can be written as: 
\begin{equation}
    |\hat{\theta}^*_q - \hat{\theta}^i_q| \leq 2m^{\frac{3}{2}}c_0 \sqrt{\frac{\ln(mT/\delta)}{q}}
\end{equation}
\end{proof}


\begin{lemma} (BIC) 
Fix an absolute constant $\tau \in (0, 1)$ and let $\delta_{\tau} = \frac{\frac{1}{2} \tau \Prob[G \geq \tau]}{\tau \Prob[G \geq \tau] + 1}$. Algorithm~\eqref{alg:multi-arm-racing} is BIC if the parameters satisfy $\delta \leq \delta_{\tau}$ and $L_1 \geq \frac{64m^3c_0^2\ln(mT/\delta)}{\tau^2\Prob[G \geq \tau]^2}$.
\end{lemma}
\begin{proof}
We want to show that for any agent $p$ in the racing stage and for any two arms $i, j \in B:$
\begin{align*}
    \E[\theta^i - \theta^j | z_p = e_i]\Prob[z_p = e_i] \geq 0
\end{align*}
We will prove a stronger statement:
\begin{align*}
    \E[\theta^i - \max_{j \neq i} \theta^j | z_p = e_i] \Prob[z_p = e_i] \geq 0
\end{align*}
For each pair of arms $i, j \in B$, denote $G_{ij} = \theta^i - \theta^j$ and 
\begin{align*}
    G_i = \theta^i - \max_{j \neq i} \theta^j = \min_{j \neq i} G_{ij}
\end{align*}
For each phase, let $\hat{G}^{ij}_q = \hat{\theta}^i_t - \hat{\theta}^j_t$ and $s_q := 2m^{\frac{3}{2}}c_0 \sqrt{\frac{\ln(mT/\delta)}{q}}$ be the decision threshold for each phase $q \geq L_1$ in Algorithm 2.\\
From the Theorem~\eqref{thm:finite-sample}, with probability at least $1 - \delta$. we have:
\begin{equation}
\label{eq:event-C-multi-arm}
    \cC = \{\forall q \geq L_1: |G_{ij} - \hat{G}^{ij}_q| < s_q\}
\end{equation}
where $L_1$ is the number of samples after running the sampling stage. 

Let $\tau \in (0, 1)$. Fix phase $t \geq L_1$, and some agent $p$ in this phase. We want to show that $\E[G_i\vert z_p = e_i]\Prob[z_p = e_i] \geq 0$.\\
From theorem ~\eqref{thm:finite-sample}, we have for any $G$:
\begin{equation*}
    \Prob[\neg \cC \vert G] \leq \delta
\end{equation*} 
Therefore, since $G\geq -1$, we have: 
\begin{align*}
\label{eq:racing-bic-multi-arm}
    \E[G_i|z_p = e_i]\Prob[z_p = e_i] &= \E[G_i|z_p = e_i, \cC]\Prob[z_p = i, \cC] + \E[G_i|z_p = e_i, \neg C]\Prob[z_p = e_i, \neg C]\\
    &\geq \E[G|z_p = e_i, \cC]\Prob[z_p = e_i, \cC] - \delta
\end{align*}
We want to upper bound the first term. This can be done by splitting it into four cases based on the value of $G_i$. We have:

\begin{equation} 
    \begin{split}
    \E[G_i | z_p = e_i, \cC]\Prob[z_p = e_i, \cC] = 
    &\E[G_i | z_p = e_i, \cC, G_i \geq \tau]\Prob[z_p= e_i, \cC, G_i \geq \tau] \\
    &\ + \E[G_i | z_p = e_i, \cC, 0 \leq G_i < \tau]\Prob[z_p = e_i, \cC, 0 \leq G_i < \tau] \\
    &\ + \E[G_i | z_p = e_i, \cC, -2s_q < G_i < 0]\Prob[z_p = e_i, \cC, -2s_q < G_i < 0]\\
    &\ + \E[G_i | z_p = e_i, \cC, G_i \leq -2s_q]\Prob[z_p = e_i, \cC, G_i \leq -2s_q]  \label{eq:multi-arm-racing-bic-cases}
    \end{split}
\end{equation}

Observe that by definition of $s_q$, we have 
\begin{align*}
    2s_q &\leq 4m^{\frac{3}{2}}c_0 \sqrt{\frac{\ln(mT/\delta)\tau^2(\Prob[G_i \geq \tau])^2}{64m^3 c_0^2 \ln(mT/\delta)}}\\
    &= \frac{\tau \Prob[G_i \geq \tau]}{2}\\
    &\leq \tau
\end{align*}
Hence, when we have $G_i \geq \tau \geq 2s_q$, then all other arms except arm $i$ must have already been eliminated at phase $q \geq L_1$ since conditional on $\cC$, $\hat{G}_q^{ij} > G_{ij} - s_q \geq G_i - s_q  \geq  s_q$. Similarly, when we have $G_i \leq -2s_t$, then arm $i$ must have already been eliminated at phase $q \geq L_1$ since
\begin{align*}
    \theta_q^i - \theta_q^* = \min_{j \neq i} G_n^{ij} < \min_{j \neq i} G_{ij} + s_q = G_i + s_q \leq -s_q
\end{align*}
Hence, arm $i$ could not be recommended in that case. We can then rewrite~\eqref{eq:multi-arm-racing-bic-cases} as
\begin{align*}
    \E[G_i | z_p - e_i, \cC]\Prob[z_p = e_i ,\cC] \geq &\E[G_i | z_p = e_i, \cC, G_i \geq \tau]\Prob[z_p= e_i, \cC, G_i \geq \tau] +\\
    &\E[G_i | z_p = e_i, \cC, 0 \leq G_i < \tau]\Prob[z_p = e_i, \cC, 0 \leq G_i < \tau] +\\
    &\E[G_i | z_p = e_i, \cC, -2s_q < G_i < 0]\Prob[z_p = e_i, \cC, -2s_q < G_i < 0]\\
    \geq &\tau \Prob[\cC, G_i \geq \tau] + 0 \Prob[\cC, 0 \leq G_i < \tau] -2s_q \Prob[\cC, G_i \leq -2s_q]\\
    = &\tau \Prob[\cC, G_i \geq \tau] - 2s_q\Prob[\cC, G_i \geq -2s_q]\\
    \geq &\tau \Prob[\cC, G_i \geq \tau] - 2s_q\\
    \geq &\tau \Prob[\cC, G_i \geq \tau] - \frac{\tau \Prob[G_i \geq \tau]}{2}\\
    \geq &\tau \Prob[\cC | G_i \geq \tau] \Prob[G_i \geq \tau] - \frac{\tau \Prob[G_i \geq \tau]}{2}\\
    \geq &\tau (1 - \delta) \Prob[G_i \geq \tau] - \frac{\tau \Prob[G_i \geq \tau]}{2}\\
    = & \left(\frac{1}{2} - \delta \right) \tau \Prob[G_i \geq \tau]\\
    \geq & \left(\frac{1}{2} - \delta_\tau \right) \tau \Prob[G_i \geq \tau]\\
    = & \left(\frac{1}{2} - \frac{\frac{1}{2} \tau \Prob[G_i \geq \tau]}{\tau \Prob[G_i \geq \tau] + 1} \right) \tau \Prob[G_i \geq \tau]\\
    = & \frac{\frac{1}{2} \tau^2 (\Prob[G_i \geq \tau])^2 + \frac{1}{2} \tau \Prob[G_i \geq \tau] - \frac{1}{2} \tau^2 (\Prob[G_i \geq \tau])^2}{\tau \Prob[G_i \geq \tau] + 1}\\
    = & \frac{\frac{1}{2} \tau \Prob[G_i \geq \tau]}{\tau \Prob[G_i \geq \tau] + 1}\\
    = &  \delta_\tau\\
    \geq & \delta
\end{align*}
Hence, we have 
\begin{align*}
    \E[G_i|z_p = e_i]\Prob[z_p = e_i] &\geq \E[G_i|z_p = e_i, \cC]\Prob[z_p = e_i, \cC] - \delta\\
    &\geq \delta - \delta\\
    &= 0
\end{align*}
Therefore, the algorithm is BIC.
\end{proof}

\begin{lemma}(Regret) With probability at least $1 - \delta$, the algorithm with any parameters $L_1, \rho \in \mathbb{N}$ and $\delta \in (0,1)$ achieves ex-post regret:
\begin{equation}
    R(T) \leq (L_1 + L_1 \rho (m-1)) + O(m^2\sqrt{mT\ln(mT/\delta)})
\end{equation}
where $\Delta = \min_{i \in A} |\theta^* - \theta^i|$, $A$ is the set of non-optimal arms, $L_1$ is the duration of one phase in the initial sampling stage and $\frac{1}{\rho}$ is the exploration probability in the sampling stage.
\end{lemma}
\begin{proof}
Assume that $\cC$ holds. Let $\theta^* = \max_{i} \theta^i$. Let $G_{*i} = \theta^* - \theta^i$ and $\Delta_i = |G_{*i}|$. Observe that since $\cC$ holds, we have $\Delta_i = |G_{i*}| \leq |\hat{G}^{*i}_q| + s_q$ where $s_q$ is the decision threshold of phase $q$. Before the stopping criteria is invoked and arm $i$ is removed from the pool of active arms, we also have $|\hat{G}^{*i}_q| \leq s_q$. Since our algorithm is BIC, every agent will comply with our recommendations. This, combined with the fact that the number of recommendations $m$ equals the number of arms $k$, gives us that the empirical estimate $\hat{\Gamma}_t$ is the $m$-dimensional identity matrix at any round $t$. Thus, the minimum singular value $\sigma_{\min}(\hat{\Gamma}_t) = 1$. Then, for each arm $i \in B$, we have:
\begin{align}
    \Delta_i \leq 2 s_q &= 4m^{\frac{3}{2}} c_0 \sqrt{\frac{\ln(mT/\delta)}{q}}
    \label{eq:delta-bound-multi-arm}
\end{align}
Hence, we have:
\begin{align*}
     \Delta_i \leq 2 s_q &= 4m^{\frac{3}{2}} c_0 \sqrt{\frac{\ln(mT/\delta)}{q}}\\
     \Rightarrow \frac{\Delta_i}{4 m^{\frac{3}{2}} c_0 \sqrt{\ln(mT/\delta)}} &\leq \frac{1}{\sqrt{q}}\\
     \Rightarrow \sqrt{q} &\leq \frac{4 m^{\frac{3}{2}} c_0 \sqrt{\ln(mT/\delta)}}{\Delta_i}\\
     \Rightarrow q &\leq \frac{16 m^3 c_0^2 \ln(mT/\delta)}{\Delta_i^2}
\end{align*}
Therefore, we must have eliminated arm $i$ by phase $q = \frac{16 m^3 c_0^2 \ln(mT/\delta)}{\Delta_i^2}$.\\
During the racing stage, each phase we give out $|B|$ recommendations for each arm $i \in B$ sequentially. Hence, the regret contribution of each arm $i$ for each phase is $\Delta_i$. Conditional on event $\cC$, the arm $a^*$ at the end of the racing stage is the best arm so no more regret is collected after the racing stage is finished. Then, the total regret accumulated for each arm $i$ is 
\begin{equation}
    R_i(T) \leq \frac{16 m^3 c_0^2 \ln(mT/\delta)}{\Delta_i}. 
\end{equation}
Hence, the total regret accumulated in the racing stage is:
\begin{align}
    R(T) &= \sum_{\text{arm } i \in A} \frac{16m^3 c_0^2 \ln(mT/\delta)}{\Delta_i} &\text{(where $A =$ \{all non-optimal arms\})}
\end{align}
Let $\Delta = \min_{i \in A} \theta^* - \theta^i$. We can upper-bound the regret of the racing stage as:
\begin{align}
    R(T) \leq \frac{16m^4 c_0^2 \ln(mT/\delta)}{\Delta}
\end{align}
Observe that the ex-post regret of the entire algorithm (both the sampling stage and the racing stage) is at most that of the racing stage plus $\Delta$ per each round of the sampling stage. Alternatively, we can also upper bound the regret by $\Delta$ per each round of the algorithm. Therefore, we can derive the ex-post regret of the entire algorithm:
\begin{equation}
    R(T) \leq \min \left \{(L_1 + L_1\rho (m-1)) \Delta + \frac{16m^4 c_0^2 \ln(mT/\delta)}{\Delta}, T\Delta \right \} \leq (L_1 + L_1 \rho (m-1)) + O(m^2\sqrt{mT\ln(mT/\delta)})
\end{equation}
\end{proof}


\begin{lemma}(Expected Regret) Algorithm with any parameters $L_1. \rho \in \mathbb{N}$ and $\delta \in (0,1)$ achieves expected ex-post regret:
\begin{equation}
    \E[R(T)] = O\left( m^2\sqrt{mT\log(mT)} \right)
\end{equation}
where $T$ is the time horizon and $m$ is the number of arms.
\end{lemma}

\begin{proof}
From Theorem~\eqref{thm:finite-sample}, we have the probability that the \textit{clean event} $\cC$ happens is at least $1 - \delta$ for some $\delta \in (0,1)$. Hence, the probability of $\neg \cC$ is at most $\delta$. The expected ex-post regret conditional on $\neg \cC$ is at most $T \delta$.\\
Now, we can set parameters $\delta,\ L_1,$ and  $\rho$ in terms of the time horizon $T$, in order to obtain an expected regret bound strictly relative to $T$. First, we set $\delta = 1/T^2$. Thus, for arbitrary constants $\tau$ and $\Prob[G \geq \tau]$, we may set $T$ sufficiently large such that 
\[\delta \leq \delta_{\tau} = \frac{\tau \Prob[G \geq \tau]}{2\left( \tau \Prob[G \geq \tau] + 1 \right)}.\] 

Next, recall that $L_1$, the length of each phase in Stage 1, is lower-bounded by
\begin{align*}
    L_1 \geq \frac{64m^3 c_0^2 \log(mT/\delta)}{\tau^2 \Prob[G \geq \tau]^2} = \frac{64m^3 c_0^2 \log(mT^3)}{\tau^2 \Prob[G \geq \tau]^2} 
    = \frac{64m^3 c_0^2 \log(m)}{\tau^2 \Prob[G \geq \tau]^2} + \frac{192 m^3 c_0^2 \log(T)}{\tau^2 \Prob[G \geq \tau]^2} 
    = c_1 m^3 \log(mT)
\end{align*}
where $c_1 = \frac{192 c_o^2}{\tau^2 \Prob[G \geq \tau]^2}$ and $m$ are constants. We can set $L_1 = \sqrt{T}$. Thus, for arbitrary constants $m$ and $c_1$, we can always find $T$ sufficiently large such that $L_1 \geq c_1 m^3 \log(mT)$.

Lastly, we set $\rho = m\sqrt{m\log(mT)}$. Thus, for arbitrary constants $\theta^1_0, \theta^m_0, \Upsilon, \sigma_{\epsilon}$ and $\Prob[\xi]$, we may set $T$ and $m$ sufficiently large such that 
\[ \rho \geq 1 + \frac{\theta^1_0 - \theta^m_0}{(\Upsilon + 2\sigma_{\epsilon})\sqrt{\frac{2\ln(3/\delta)}{L_1}} \Prob[\hat{\xi}]}\]

Therefore, the expected regret of our entire algorithm is:
\begin{align*}
    \E[R(T)] &= \E[R(T)|\neg \cC]\Prob[\neg \cC] + \E[R(T)|\cC]\Prob[\cC] \\
    &\leq T\delta + \left((L_1 + L_1\rho(m-1)) + O(m^2\sqrt{mT\log(mT/\delta)} \right)\\
    &= \frac{1}{T} + \left(\sqrt{T} + (m-1)m\sqrt{m\log(mT)}\sqrt{T} \right) + O\left( m^2\sqrt{mT\log(mT)} \right)\\
    &= \frac{1}{T} + O\left( m^2\sqrt{mT\log(mT)} \right) + O\left( m^2\sqrt{mT\log(mT)} \right)\\
    &= O\left( m^2\sqrt{mT\log(mT)} \right)
\end{align*}

\end{proof}



==> new-estimator.tex <==
\subsubsection{With Centering}
Let the operator $\bar{\cdot}$ denote the mean, such that $\bar{y}:=\frac{1}{n}\sum_{i=1}^n y_i$ and $\bar{g}:=\frac{1}{n}\sum_{i=1}^n g(u_i)$, etc. Then,

\lscomment{Should it be like $\bar{\cdot}_n,$ i.e.  the mean for all rounds until $n$?}

\begin{align*}
    \bar{y} &= \langle\beta,\bar{z}\rangle + \langle\theta,\bar{\eta}\rangle + \bar{g} + \bar{\epsilon}
\end{align*}
Thus, the centered reward and treatment choice at round $i$ are given as:
\begin{equation}
    \begin{cases}
    \label{eq:general-centered-reward-treatment-choice}
    y_i - \bar{y} = \langle\beta,z_i-\bar{z}\rangle + \langle\theta,\eta_i-\bar{\eta}\rangle + g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\\
    x_i - \bar{x} = \langle\Gamma,z_i-\bar{z}\rangle + \eta_i-\bar{\eta}
    \end{cases}
\end{equation}
This formulation of the centered reward $y_i-\bar{y}$ allows us to express and bound the error between the treatment effect $\theta$ and its instrumental variable estimate $\hat{\theta}_n$, which we show in the following section.

\begin{restatable}[Treatment effect approximation bound for General Model]{theorem}{generaltreatmentapproximationbound}\label{thm:general-treatment-approximation-bound}
        Given a sample set $(z_i, x_i, y_i)_n$, which contains $n$ samples of instrument $z\in\RR^k$, treatment $x\in\RR^k$, and reward $y\in\RR$, we bound the difference between the true treatment effect $\theta\in\RR^k$ and the predicted treatment effect $\hat{\theta}_n$ derived via IV regression over $(z_i, x_i, y_i)_n$. Let $\Upsilon$ be a upper bound on the confounding term $g(u_i)$. For some confidence $\delta>0$, with probability at least $1 - \delta$:
\[\norm{\hat{\theta}_n-\theta}_2 \leq \frac{\left(2\sigma_{\eps}+2\Upsilon\right)\sqrt{2n\log(4/\delta)}}{\sigma_\text{r}\left\{\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\right\}},\]
where $\sigma_\text{r}\{\cdot\}$ denotes the smallest non-zero singular value.
\end{restatable}

\begin{proof}
    See \cref{sec:general-approximation-bound-proof} for a proof.
\end{proof}



\subsubsection{Finite Sample Analysis}
\label{sec:general-approximation-bound-proof}
Given $n \in \RR$ samples $(z_i, x_i, y_i)_i=1^n$, we would like to bound the difference between the predicted exogenous treatment effect, denoted $\hat{\theta}_n$, and the true exogenous treatment effect $\theta$. 

We can estimate $\hat{\theta}_n$ via Two-Stage Least Squares (2SLS) regression. In the first stage, we estimate $\hat{\beta}_n$ by regressing $y_i-\bar{y}$ onto $z_i-\bar{z}$ and $\hat{\Gamma}_n$ by regressing $x_i-\bar{x}$ onto $z_i-\bar{z}$:
\begin{equation}
    \hat{\beta}_n = \bigg(\sum_{i=1}^n(z_i-\bar{z})(z_i-\bar{z})^\intercal\bigg)^\dagger\sum_{i=1}^n(y_i-\bar{y})(z_i-\bar{z})
    \hspace{.25cm}
    \text{ and }
    \hspace{.25cm}
    \hat{\Gamma}_n = \bigg(\sum_{i=1}^n(z_i-\bar{z})(z_i-\bar{z})^\intercal\bigg)^\dagger\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal
\end{equation}

Second, we take the inverse of $\Gamma$ times $\beta$ as the predicted causal effect vector $\hat{\theta}_n$, i.e. 
\begin{align*}
    \hat{\theta}_n 
    &= \hat{\Gamma}_n^\dagger\hat{\beta}_n\\
    &= \bigg(\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\bigg)^\dagger\bigg(\sum_{i=1}^n(z_i-\bar{z})(z_i-\bar{z})^\intercal\bigg)\bigg(\sum_{i=1}^n(z_i-\bar{z})(z_i-\bar{z})^\intercal\bigg)^\dagger\sum_{i=1}^n(y_i-\bar{y})(z_i-\bar{z})\\
    &= \bigg(\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\bigg)^\dagger\sum_{i=1}^n(y_i-\bar{y})(z_i-\bar{z})
\end{align*}

Hence, the L2-norm of the difference between $\theta$ and $\hat{\theta}_n$ is given as:
\begin{align*}
    \norm{\hat{\theta}_n - \theta}_2
    &= \norm{\bigg(\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\bigg)^\dagger\bigg(\sum_{i=1}^n(z_i-\bar{z})\left(\langle\theta,x_i-\bar{x}\rangle + g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)^\intercal\bigg) - \theta}_2\\
    &= \norm{\bigg(\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\bigg)^\dagger\bigg(\sum_{i=1}^n(z_i-\bar{z})\left((x_i-\bar{x})^\intercal\theta + g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)\bigg) - \theta}_2\\
    &= \norm{\theta + \bigg(\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\bigg)^\dagger\bigg(\sum_{i=1}^n(z_i-\bar{z})\left(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)\bigg) - \theta}_2\\
    &= \norm{\bigg(\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\bigg)^\dagger\sum_{i=1}^n(z_i-\bar{z})(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon})}_2\\
\end{align*}

Next, note that
\begin{align*}
    \norm{\hat{\theta}_n - \theta}_2
    &= \norm{\bigg(\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\bigg)^\dagger\sum_{i=1}^n(z_i-\bar{z})(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon})}_2\\
    &\leq \norm{\bigg(\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\bigg)^\dagger}_2\norm{\sum_{i=1}^n(z_i-\bar{z})(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon})}_2\\
    &= \frac{\norm{\sum_{i=1}^n(z_i-\bar{z})(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon})}_2}{\sigma_\text{r}\left\{\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\right\}},\\
\end{align*}
where $\text{r}$ is the rank of $\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal$ and the singular values are sorted in decreasing order, i.e. $\sigma_1 \geq \dots \geq \sigma_\text{r}$. Thus, $\sigma_\text{r}\{\cdot\}$ denotes the smallest non-zero singular value of a matrix.

\lscomment{Do we need to show that the spectral norm of the pseudoinverse equals $\sigma_\text{r}\left\{\sum_{i=1}^n(z_i-\bar{z})(x_i-\bar{x})^\intercal\right\}$?}


Finally, we may bound $\norm{\hat{\theta}_n-\theta}_2$ by upper bounding $\norm{\sum_{i=1}^n(z_i-\bar{z})(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon})}_2$. We do so in \cref{eq:general-approximation-bound-numerator}.
\begin{lemma}\label{eq:general-approximation-bound-numerator}
For some $\delta \in (0,1)$, with probability at least $1-\delta$, we have
\begin{equation}
    \norm{\sum_{i=1}^n(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon})(z_i-\bar{z})}_2 \leq \left(2\sigma_{\eps}+2\Upsilon\right)(n/n_{\min})\sqrt{2n_{\min}\log(4/\delta)}
\end{equation}
\begin{proof}
    \begin{align*}
        &\norm{\sum_{i=1}^n \left(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)(z_i - \bar{z})}_2\\
        &= \norm{\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \E[g(u)]-\bar{g} + \epsilon_i-\bar{\epsilon}\right)(z_i - \bar{z})}_2\\
        &= \norm{\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)z_i - \sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)\bar{z} + \sum_{i=1}^n \left(\E[g(u)]-\bar{g}-\bar{\epsilon}\right)(z_i - \bar{z})}_2\\
        &= \norm{\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)z_i - \sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)\bar{z}}_2 \tag{since $\sum_{i=1}^n(z_i - \bar{z})=0$}\\
        &\leq \norm{\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)z_i}_2 + \left|\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)\right|\norm{\bar{z}}_2 \tag{by triangle inequality and Cauchy-Schwarz}\\
        &\leq \norm{\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)z_i}_2 + \left|\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)\right|\tag{since $\norm{\bar{z}}_2\leq1$}\\
        &\leq \left|n\sigma_{\eps}\sqrt{\frac{2\log(1/\delta_1)}{n_{\min}}} + 2n\Upsilon\sqrt{\frac{\log(1/\delta_2)}{2n_{\min}}}\right| + \left|\sigma_{\eps}\sqrt{2n\log(1/\delta_3)} + 2\Upsilon\sqrt{\frac{n\log(1/\delta_4)}{2}}\right|\tag{by Chernoff Bound, where $n_{\min}=\min_i\sum_{i=1}^n\1[z_i=1]$}\\
        &\leq \left(2\sigma_{\eps}+2\Upsilon\right)(n/n_{\min})\sqrt{2n_{\min}\log(4/\delta)} \tag{since $n\leq\,n\sqrt{n_{\min}}/n_{\min}$ and by Union Bound, where $\delta:=\delta_1+\delta_2+\delta_3+\delta_4$}
    \end{align*}
\end{proof}
\end{lemma}

\subsubsection{Without Centering}
This formulation of the centered reward $y_i$ allows us to express and bound the error between the treatment effect $\theta$ and its instrumental variable estimate $\hat{\theta}_n$, which we show in the following section.

\begin{restatable}[Treatment effect approximation bound for General Model]{theorem}{generaltreatmentapproximationbound}\label{thm:general-treatment-approximation-bound}
        Given a sample set $(z_i, x_i, y_i)_n$, which contains $n$ samples of instrument $z\in\RR^k$, treatment $x\in\RR^k$, and reward $y\in\RR$, we bound the difference between the true treatment effect $\theta\in\RR^k$ and the predicted treatment effect $\hat{\theta}_n$ derived via IV regression over $(z_i, x_i, y_i)_n$. Let $\Upsilon$ be a upper bound on the confounding term $g(u_i)$. For some confidence $\delta>0$, with probability at least $1 - \delta$:
%\[\norm{\hat{\theta}_n-\theta}_2 \leq \frac{\left(\sigma_{\eps}+2\Upsilon\right)\sqrt{2n_\log(4/\delta)}}{\sigma_\text{r}\left\{\sum_{i=1}^nz_ix_i^\intercal\right\}},\]
where $\sigma_\text{r}\{\cdot\}$ denotes the smallest non-zero singular value.
\end{restatable}

\begin{proof}
    See \cref{sec:general-approximation-bound-proof} for a proof.
\end{proof}

\subsubsection{Finite Sample Analysis}
\label{sec:general-approximation-bound-proof}
Given $n \in \RR$ samples $(z_i, x_i, y_i)_i=1^n$, we would like to bound the difference between the predicted exogenous treatment effect, denoted $\hat{\theta}_n$, and the true exogenous treatment effect $\theta$. 

We can estimate $\hat{\theta}_n$ via Two-Stage Least Squares (2SLS) regression. In the first stage, we estimate $\hat{\beta}_n$ by regressing $y_i$ onto $z_i$ and $\hat{\Gamma}_n$ by regressing $x_i$ onto $z_i$:
\begin{equation}
    \hat{\beta}_n = \bigg(\sum_{i=1}^nz_iz_i^\intercal\bigg)^{-1}\sum_{i=1}^ny_iz_i
    \hspace{.4cm}
    \text{ and }
    \hspace{.4cm}
    \hat{\Gamma}_n = \bigg(\sum_{i=1}^nz_iz_i^\intercal\bigg)^{-1}\sum_{i=1}^nz_ix_i^\intercal
\end{equation}

Second, we take the inverse of $\Gamma$ times $\beta$ as the predicted causal effect vector $\hat{\theta}_n$, i.e. 
\begin{align*}
    \hat{\theta}_n 
    &= \hat{\Gamma}_n^{-1}\hat{\beta}_n\\
    &= \bigg(\sum_{i=1}^nz_ix_i^\intercal\bigg)^{-1}\bigg(\sum_{i=1}^nz_iz_i^\intercal\bigg)\bigg(\sum_{i=1}^nz_iz_i^\intercal\bigg)^{-1}\sum_{i=1}^nz_iy_i\\
    &= \bigg(\sum_{i=1}^nz_ix_i^\intercal\bigg)^{-1}\sum_{i=1}^nz_iy_i
\end{align*}

Hence, the L2-norm of the difference between $\theta$ and $\hat{\theta}_n$ is given as:
\begin{align*}
    \norm{\hat{\theta}_n - \theta}_2
    &= \norm{\bigg(\sum_{i=1}^nz_ix_i^\intercal\bigg)^{-1}\sum_{i=1}^nz_iy_i}_2\\
    &= \norm{\bigg(\sum_{i=1}^nz_ix_i^\intercal\bigg)^{-1}\sum_{i=1}^nz_i\left(\langle\theta,x_i\rangle + g(u_i) + \epsilon_i\right)^\intercal\bigg) - \theta}_2\\
    &= \norm{\bigg(\sum_{i=1}^nz_ix_i^\intercal\bigg)^{-1}\sum_{i=1}^nz_i\left(x_i^\intercal\theta + g(u_i) + \epsilon_i\right)\bigg) - \theta}_2\\
    &= \norm{\theta + \bigg(\sum_{i=1}^nz_ix_i^\intercal\bigg)^{-1}\sum_{i=1}^nz_i\left(g(u_i) + \epsilon_i\right) - \theta}_2\\
    &= \norm{\bigg(\sum_{i=1}^nz_ix_i^\intercal\bigg)^{-1}\sum_{i=1}^nz_i\left(g(u_i) + \epsilon_i\right)}_2\\
    &\leq \norm{\bigg(\sum_{i=1}^nz_ix_i^\intercal\bigg)^{-1}}_2\norm{\sum_{i=1}^nz_i(g(u_i)+\epsilon_i)}_2\tag{by Cauchy-Schwarz}\\
    &= \frac{\norm{\sum_{i=1}^nz_i(g(u_i)+\epsilon_i)}_2}{\sigma_{\min}\left\{\sum_{i=1}^nz_ix_i^\intercal\right\}},
\end{align*}
where $\sigma_{\min}\{\cdot\}$ denotes the minimum singular value.


Finally, we may bound $\norm{\hat{\theta}_n-\theta}_2$ by upper bounding $\norm{\sum_{i=1}^nz_i(g(u_i)+\epsilon_i)}_2$. We do so in \cref{eq:general-approximation-bound-numerator}.
\begin{lemma}\label{eq:general-approximation-bound-numerator}
For some $\delta \in (0,1)$, with probability at least $1-\delta$, we have
\begin{equation}
    \norm{\sum_{i=1}^nz_i(g(u_i)+\epsilon_i)}_2 \leq nk\Upsilon+(k\sigma_{\eps}+2k\Upsilon)\sqrt{2n\log(2/\delta)}
\end{equation}
\begin{proof}
\lscomment{Double-check the move from the first to the second line below...}
    \begin{align*}
        &\norm{\sum_{i=1}^n (g(u_i)+\epsilon_i)z_i}_2\\
        &=\norm{\sum_{j=1}^k\sum_{i=1}^n (g(u_i)+\epsilon_i)\1[z_i=\e_j]}_2\\
        &\leq\norm{\sum_{j=1}^k\sum_{i=1}^n (g(u_i)+\epsilon_i)}_2\\
        &\leq \sum_{j=1}^k\left|n\E[g(u)] + 2\Upsilon\sqrt{\frac{n\log(1/\delta_1)}{2}} + \sigma_{\eps}\sqrt{2n\log(1/\delta_2)}\right| \tag{by Chernoff Bound}\\
        &\leq nk\Upsilon + (k\sigma_{\eps}+2k\Upsilon)\sqrt{2n\log(2/\delta)}\tag{by Union Bound, where $\delta:=\delta_1+\delta_2$}
    \end{align*}
    
    
    \medskip
    
    
    \begin{align*}
        \norm{\sum_{i=1}^n (g(u_i)+\epsilon_i)z_i}_2
        &=\sqrt{\sum_{j=1}^k\left(\sum_{i=1}^n (g(u_i)+\epsilon_i)\1[z_i=\e_j]\right)^2}\\
        &=\sqrt{\sum_{j=1}^k\left(\sum_{i=1}^{n_j} (g(u_i)+\epsilon_i)\right)^2}\tag{where $n_j=\sum_{i=1}^n\1[z_i=\e_j]$}\\
        &\leq \sqrt{\sum_{j=1}^k\left(2\Upsilon\sqrt{\frac{n_j\log(1/\delta_j)}{2}} + \sigma_{\eps}\sqrt{2n_j\log(1/\delta_j')}\right)^2} \tag{by Chernoff Bound and since $\E[g(u)]=0$ \lscomment{refer to theorems}}\\
        &\leq \sqrt{\sum_{j=1}^k\left(2\Upsilon\sqrt{\frac{n_j\log(2k/\delta)}{2}} + \sigma_{\eps}\sqrt{2n_j\log(2k/\delta)}\right)^2} \tag{by Union Bound with $\delta=\sum_{j=1}^k\delta_j+\delta_j'$}\\
        &\leq\sqrt{k\left(2\Upsilon\sqrt{\frac{n\log(2k/\delta)}{2}} + \sigma_{\eps}\sqrt{2n\log(2k/\delta)}\right)^2} \tag{since $n_j\leq n$ for all $j$}\\
        &=\sqrt{k}\left(2\Upsilon\sqrt{\frac{n\log(2k/\delta)}{2}} + \sigma_{\eps}\sqrt{2n\log(2k/\delta)}\right)\\
        &\leq \sqrt{k}\left(2\Upsilon+\sigma_{\eps}\right)\sqrt{2n\log(2k/\delta)} \tag{since $\sqrt{\frac{n\log(2k/\delta)}{2}}\leq\sqrt{2n\log(2k/\delta)}$}
    \end{align*}
\end{proof}
\end{lemma}

Next, we bound the denominator.

==> one-dimension-bound.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\section{IV Estimator Proof for control-treatment setting}
\label{sec:iv-estimator}
\subsection{Model}
We present our model as a system of linear equations expressed as such
\begin{equation}
    \begin{cases}
    y_i = \theta x_i + g(u_i) + \epsilon_i\\
    x_i = f(u_i, z_i)
    \end{cases}
\end{equation}
The recommendation $z_i$ and the action choice $x_i$ to be binary, i.e, either $0$ or $1$. This correspond to our control-treatment setting where the control action correspond to $0$, and the treatment correspond to $1$. The reward $y_i$ is given by the action $x_i$, treatment effect $\theta$, zero-mean noise $\epsilon$ and the unobserved confounding shift $g(u_i)$. Our goal is to consistently estimate the treatment effect $\theta$. This is complicated by the unobserved confounding shift $g(u_i)$ and its correlation with the action choice $x_i$.\\
We model a linear relationship between the action $x_i$ and the recommendation $z_i$ by introducing two population probability that an agent choose the treatment given a recommendation $\gamma_0$ and $\gamma_1$, formally defined as
\begin{align*}
    \gamma_0 &= \Prob[x_i = 1| z_i = 0] \hspace{1cm}\text{and}\\
    \gamma_1 &= \Prob[x_i = 1| z_i = 1]
\end{align*}
Then, we can rewrite our equation modelling $x_i$ as such:
\begin{align*}
    x_i &= \gamma_1 z_i + \gamma_0 (1 - z_i) + (f(u_i, z_i) - \gamma_1 z_i - \gamma_0 (1 - z_i))\\
    &= \gamma_1 z_i + \gamma_0 (1 - z_i) + \eta_i\\
    &= \gamma z_i + \gamma_0 + \eta_i
\end{align*}
where $\eta_i = f(u_i, z_i) - \gamma_1 z_i - \gamma_0 (1 - z_i)$ is a mean-zero random variable and $\gamma = \gamma_1 - \gamma_0$ is the population \textit{compliance coefficient}. Now, we can rewrite the reward $y_i$ as 
\begin{align*}
    y_i &= \theta\left(\gamma z_i + \gamma_0 + \eta_i\right) + g(u_i) + \epsilon_i\\
    &= \underbrace{\theta\,\gamma}_{\beta} z_i + \theta \gamma_0 + \theta \eta_t + g(u_i) + \epsilon_i
\end{align*}
Let the operator $\bar{\cdot}$ denote the mean, such that $\bar{y}:=\frac{1}{n}\sum_{i=1}^n y_i$ and $\bar{g}:=\frac{1}{n}\sum_{i=1}^n g(u_i)$, etc. Then,
\begin{align*}
    \bar{y} &= \beta\bar{z} + \theta\gamma_0 + \theta\bar{\eta} + \bar{g} + \bar{\epsilon}
\end{align*}
Thus, the centered reward and treatment choice at round $i$ are given as:
\begin{equation}
    \begin{cases}
    \label{eq:centered-reward-treatment-choice}
    y_i - \bar{y}_i = \beta(z_i-\bar{z}) + \theta(\eta_i-\bar{\eta}) + g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\\
    x_i - \bar{x}_i = \gamma(z_i-\bar{z}) + \eta_i-\bar{\eta}
    \end{cases}
\end{equation}
This formulation of the centered reward $y_i-\bar{y}$ allows us to express and bound the error between the treatment effect $\theta$ and its instrumental variable estimate $\hat{\theta}_n$, which we show in the following section.
\subsection{Finite Sample Analysis}
Given $n \in \RR$ samples $(z, x, y)_n$, we would like to bound the difference between the predicted exogenous treatment effect, denoted $\hat{\theta}_n$, and the true exogenous treatment effect $\theta$. 
\treatmentapproximationbound*

\lscomment{Placeholder. Add a corollary for the approximation bound necessary \lscomment{want a lower bound for $\displaystyle\left|\sum_{i=1}^n \gamma(z_i-\bar{z})^2 + \sum_{i=1}^n(\eta_i-\bar{\eta})(z_i-\bar{z})\right|$ in the approximation bound proof }}
\begin{corollary}
Given a sample set $(z_i, x_i, y_i)_n$, which contains $n$ samples of instrument $z$, treatment $x$, and reward $y$, we bound the difference between the true treatment effect $\theta$ and the predicted treatment effect $\hat{\theta}_n$ derived via IV regression over $(z_i, x_i, y_i)_n$. Let $\Upsilon$ be a upper bound on the confounding term $g(u_i)$. During the racing stage, for some confidence $\delta>0$, with probability at least $1 - \delta$:
    \begin{align*}
    \abs{\hat{\theta}_n - \theta} 
    &\leq \frac{4(2 + 2\Upsilon + 2\sigma_\epsilon + (\sqrt{n/n_1} + \sqrt{n/n_0}))\sqrt{2\log(8/\delta)}}{\hat{\gamma}\sqrt{n}}\\
    &= O\left(\frac{1}{\hat{\gamma}\,n_{\min}}\right),
    \end{align*}
    where $n_{\min} := \min_{a\in\{0,1\}}n_a$
\end{corollary}
We can estimate $\hat{\theta}_n$ via a Two-Stage Least Squares (2SLS). In the first stage, we regress $y_i-\bar{y}$ onto $z_i-\bar{z}$ to get the empirical estimate $\hat{\beta}_n$ and $x_i-\bar{x}$ onto $z_i-\bar{z}$ to get $\hat{\gamma}_n$ as such:
\begin{equation}
    \hat{\beta}_n := \frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (z_i -\bar{z})^2} \hspace{1cm}\text{and}\hspace{1cm} \hat{\gamma}_n := \frac{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})}{\sum_{i=1}^n (z_i -\bar{z})^2}
    \label{eq:beta-gamma-hat}
\end{equation}
Second, we take their quotient as the predicted treatment effect $\hat{\theta}_n$, i.e. 
\begin{align}
    \hat{\theta}_n &= \frac{\hat{\beta}_n}{\hat{\gamma}_n}\\
    &= \frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (z_i -\bar{z})^2} \frac{\sum_{i=1}^n (z_i -\bar{z})^2}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})} \nonumber\\
    &= \frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})}
\end{align}

Hence, the absolute value of the difference
\begin{align*}
    \left| \hat{\theta}_n - \theta \right|
    &= \left| \frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})} - \theta \right|\\
    &= \left| \frac{\sum_{i=1}^n \left(\theta\gamma(z_i-\bar{z}) + \theta(\eta_i-\bar{\eta}) + g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)(z_i - \bar{z})}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})} - \theta \right| \tag{by \cref{eq:centered-reward-treatment-choice}}\\
    &= \left| \theta + \frac{\sum_{i=1}^n \left(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)(z_i - \bar{z})}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})} - \theta \right|\\
    &= \frac{\left|\sum_{i=1}^n \left(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)(z_i - \bar{z})\right|}{\left|\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})\right|}\\
    &= \frac{\left|\sum_{i=1}^n \left(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)(z_i - \bar{z})\right|}{\left|\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})\right|}
\end{align*}
In order to upper bound $\left|\hat{\theta}_n - \theta\right|$ in terms of the number of samples $n$, we need to find an upper bound for $\displaystyle\left|\sum_{i=1}^n \left(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)(z_i - \bar{z})\right|$ (see \cref{eq:approximation-bound-numerator})

In the following lemma, we demonstrate the bound on the numerator:
\begin{lemma}
\label{eq:approximation-bound-numerator}
For some $\delta \in (0,1)$, with probability at least $1-\delta$, we have
\begin{equation}
    \left|\sum_{i=1}^n \left(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)(z_i - \bar{z})\right| \leq \left(2\sigma_{\eps}+2\Upsilon\right)\sqrt{2n\log(5/\delta)}
\end{equation}
\end{lemma}
\begin{proof}
    \begin{align*}
        &\left|\sum_{i=1}^n \left(g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\right)(z_i - \bar{z})\right|\\
        &= \left|\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \E[g(u)]-\bar{g} + \epsilon_i-\bar{\epsilon}\right)(z_i - \bar{z})\right|\\
        &= \left|\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)z_i - \sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)\bar{z} + \sum_{i=1}^n \left(\E[g(u)]-\bar{g}-\bar{\epsilon}\right)(z_i - \bar{z})\right|\\
        &= \left|\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)z_i - \sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)\bar{z}\right| \tag{since $\sum_{i=1}^n(z_i - \bar{z})=0$}\\
        &\leq \left|\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)z_i\right| + \left|\sum_{i=1}^n \left(g(u_i)-\E[g(u)] + \epsilon_i\right)\right| \tag{$|\bar{z}|<1$ and Cauchy-Schwartz}\\
        &\leq \left|\sigma_{\eps}\sqrt{2n_1\log(1/\delta_1)} + \Upsilon\sqrt{\frac{n_1\log(1/\delta_2)}{2}}\right| + \left|\sigma_{\eps}\sqrt{2n\log(1/\delta_3)} + \Upsilon\sqrt{\frac{n\log(1/\delta_4)}{2}}\right| \tag{by Chernoff Bound, where $n_1=\sum_{i=1}^n\1[z_i=1]$}\\
        &\leq \left(2\sigma_{\eps}+2\Upsilon\right)\sqrt{2n\log(4/\delta_5)} \tag{since $n_1\leq n$ and Union Bound}\\
    \end{align*}
\end{proof}

\begin{lemma}
    Lower bound on $\displaystyle\left|\sum_{i=1}^n \left(\gamma(z_i-\bar{z}) + \eta_i-\bar{\eta}\right)(z_i - \bar{z})\right|$:
\end{lemma}
\begin{proof}
    \begin{align*}
        \left|\sum_{i=1}^n \left(\gamma(z_i-\bar{z}) + \eta_i-\bar{\eta}\right)(z_i - \bar{z})\right|
        &= \left|\gamma\sum_{i=1}^n(z_i-\bar{z})^2 + \sum_{i=1}^n(\eta_i-\bar{\eta})(z_i - \bar{z})\right|\\
        &= \left|\gamma\sum_{i=1}^n(z_i-\bar{z})^2 + \sum_{i=1}^n\eta_i(z_i - \bar{z}) - \sum_{i=1}^n\bar{\eta}(z_i - \bar{z})\right|\\
        &= \left|\gamma\sum_{i=1}^n(z_i-\bar{z})^2 + \sum_{i=1}^n\eta_i(z_i - \bar{z})\right|\\
        &\geq \left|\max\left\{0,\gamma\sum_{i=1}^n(z_i-\bar{z})^2 - \sqrt{\frac{n\log(1/\delta_6)}{2}}\right\}\right| \tag{by Chernoff Bound}\\
    \end{align*}
    
    Now, the bound on the term $\gamma\sum_{i=1}^n(z_i-\bar{z})^2$ depends on which stage of the algorithm the samples are from: the term $\gamma$ is given by how compliant the agents are with the algorithm's recommendations and the term $\sum_{i=1}^n(z_i-\bar{z})^2$ is given by the ratio of control versus treatment recommendations.
    
    With solely data from the sampling stage or the first phase of the racing stage, the term \[\gamma_{\text{sampling stage}} = \Prob_{\cU}[x_i=1|z_i=1]-\Prob_{\cU}[x_i=1|z_i=0]=1-p_1,\]
    where $p_1$ is the proportion of agents that prefer the treatment $x_i=1$. This is because in the sampling stage, we make sure that agents of type 1 are BIC and agents of type 1 prefer arm 1 anyways. With solely data from the second phase of the racing stage, the term $\gamma_{\text{racing stage}}=1$ since every agent complies with all our recommendations.
    
    Finally, we need to find a lower bound on the term $\sum_{i=1}^n (z_i - \bar{z})^2$. In the sampling stage, we recommend the treatment with frequency $1/\rho$. Thus,
    \[
        \sum_{i=1}^n(z_i-\bar{z})^2 \geq \sum_{i=1}^n\frac{1}{\rho^2} = \frac{n}{\rho^2}
    \]
    
    In the racing stage, we recommend the control and the treatment with the same frequency. Hence, during the racing stage, we have $\bar{z}=1/2$ and
    \[
        \sum_{i=1}^n (z_i - \bar{z})^2 \geq \frac{n}{4}
    \]
\end{proof}


\newpage
\textbf{New Material:}
Lower bound on $\left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|$

In either stage, let $c$ be the probability of recommending arm 1. Then, $\bar{z}=c$. Also let $n_0$ and $n_1$ be the number of samples with agents of type 0 and type 1, respectively. Let $n_{0,0}$ be the number of samples with agents of type 0 with recommendations of arm 0.

\begin{align*}
    \left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|
    &= \left|\sum_{i=1}^n(x_i-\bar{x})(z_i-c)\right|\\
    &= \left|\sum_{i=1}^n(x_i-\bar{x})z_i-c\sum_{i=1}^n(x_i-\bar{x})\right|\\
    &= \left|\sum_{i=1}^{cn}(1-\bar{x})-c\sum_{i=1}^n(x_i-\bar{x})\right|\tag{$z_i=1\Rightarrow\,x_i=1$; otherwise, $z_i=0$}\\
    &= \left|cn(1-\bar{x})-c\sum_{i=1}^nx_i+c\sum_{i=1}^n\bar{x}\right|\\
    &= \left|cn-cn\bar{x}+cn\bar{x}-c\sum_{i=1}^nx_i\right|\\
    &= c\left|n-\sum_{i=1}^nx_i\right|\\
    &= cn_{0,0}\\
\end{align*}

Now, we need to lower bound $n_{0,0}$. For any round $i$, since $z_i\perp\,x_i$, given that the recommendation $z_i=0$, the probability that an agent of type 0 shows up is $p_0$. Thus, the expected value 
\[\E[n_{0,0}]=np_0(1-c),\]
where $p_0$ is the proportion of agents of type 0 in the population and by Chernoff bound, with probability at least $1-\delta$,
\[n_{0,0} \geq np_0(1-c)-\sqrt{\frac{n(1-c)\log(1/\delta)}{2}}.\]

Therefore, with probability at least $1-\delta$,
\[\left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|\geq c\left(np_0(1-c)-\sqrt{\frac{n(1-c)\log(1/\delta)}{2}}\right)\].

In the sampling stage, when $c=1/\rho$, with probability at least $1-\delta$,
\[\left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|\geq (1/\rho)\left(np_0(1-1/\rho)-\sqrt{\frac{n(1-1/\rho)\log(1/\delta)}{2}}\right)\].

In the racing stage, when $c=1/2$, with probability at least $1-\delta$,
\[\left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|\geq \frac{np_0-\sqrt{n\log(1/\delta)}}{4}\].

Supposing this bound holds for the sampling stage and each phase in the racing stage, then 
$s_q \leq s_L$, since (assuming that $\rho\geq2$),
\[\frac{np_0-\sqrt{n\log(1/\delta)}}{4}\geq(1/\rho)\left(np_0(1-1/\rho)-\sqrt{\frac{n(1-1/\rho)\log(1/\delta)}{2}}\right)\]

\[s_L:= \frac{\left(2\rho\sigma_{\eps}+2\Upsilon\right)\sqrt{2L\log(6/\delta)}}{Lp_0(1-1/\rho)-\sqrt{L(1-1/\rho)\log(6/\delta)/2}}\]

\[s_q:= \frac{\left(8\sigma_{\eps}+8\Upsilon\right)\sqrt{2^qL\log(6/\delta)}}{2^qLp_0-\sqrt{2^qL\log(6/\delta)}}\]

Assuming that the BIC condition has been met at every phase before phase $q$, the algorithm should be BIC for agents of type 0 in phase $q$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{algorithm}[ht!]
% \SetAlgoLined
% \SetKwInput{KwIn}{Input}
% \KwIn{number of rounds in sampling stage sans the first phase $L \in \mathbb{N}$; time horizon $T$; minimum phase length parameter $h$; probability $\delta$; and upper bound $\nu$ on cost function $\phi(u_t)$}
% \KwIn{IV estimate of mean reward $\theta$, denoted $\hat{\theta}_{L}$, given $L$ samples from the sampling stage}
%     Let $\hat{\theta}_0=\hat{\theta}_{L}$;\\
%     Split the remainder into consecutive phases of $2^{q-1}\cdot\max\{L,h\}$ rounds each, starting $q=1$;\\
%     \If{$\hat{\theta}_L\leq\frac{\left(2\rho\sigma_{\eps}+2\Upsilon\right)\sqrt{2L\log(6/\delta)}}{Lp_0(1-1/\rho)-\sqrt{L(1-1/\rho)\log(6/\delta)/2}}$}{}
%     \Else{
%     \While{$\hat{\theta}_q \leq \frac{\left(8\sigma_{\eps}+8\Upsilon\right)\sqrt{2^qL\log(6/\delta)}}{2^qLp_0-\sqrt{2^qL\log(6/\delta)}}$}
%     {The next $L2^{q-1}$ agents are recommended both arms sequentially;\\
%     For each arm $a \in \{0,1\}$, let $y^a_t$ be one sample reward of that arm in this phase;\\
%     Let the estimate $\hat{\theta}_q^{racing}$ be the IV estimate of the mean reward $\theta$ using only the $L2^{q-1}$ samples from the $q$th phase\\
%     Update $\hat{\theta}_q$ to the  whichever estimate, either $\hat{\theta}_L$ or $\hat{\theta}_q^{racing}$, is associated with the smaller approximation bound, i.e. $\hat{\theta}_q = \argmin\limits_{\hat{\theta}_n\in\left\{\hat{\theta}_L,\,\hat{\theta}_q^{racing}\right\}} \frac{\left(2\sigma_{\eps}+2\Upsilon\right)\sqrt{2n\log(5/\delta)}}{\left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|}$\\ \dncomment{I think doing $S^{BEST}_q$ is better here}
%     $q = q+1$;}} 
%     For all remaining agents recommend $a^*=\1\left[\hat{\theta}_q>0\right]$
%     \caption{The racing stage for control-treatment with two mixed-preference types}
%     \label{alg:racing-two-types-mixed-preferences}
% \end{algorithm}

% \begin{theorem}
%     Fix some constant $\tau \in (0, 1)$. Remember that $\phi(u_t)\in[-\nu,\nu]$ for all $u_t$ and $\Prob_{\cP_0}[\theta>\tau]$ be the prior probability that $\theta>\tau$ for agents of type 1. Let the approximation bound $s_L$ after the sampling stage be \begin{equation}
%         s_L:=\frac{2\left(\sigma_{\eps}+\Upsilon\right)\sqrt{2L\log(5/\delta)}}{\left|\sum_{i=1}^L(x_i-\bar{x})(z_i-\bar{z})\right|}
%         \leq\frac{\tau\Prob_{\cP_0}[\theta>\tau]}{4}-\frac{\nu}{2}.
%     \end{equation} 
%     Then, during the first phase of the racing stage, the recommendations from \cref{alg:racing-two-types-mixed-preferences} are BIC for agents of type 1.
% \end{theorem}

% \begin{proof} 
% \lscomment{Define $s_q$ such that $s_L=\tau\Prob_{\cP_0}[\theta\geq\tau]\delta'-\nu$, for any $\delta'\in(0,1)$}
% For brevity, denote the number of rounds in a phase $q$ in \cref{alg:racing-two-types-mixed-preferences} as $L_q:=2^{q-1}\max\{L,h\}\geq L$ and $L_0:=L$. Let the decision threshold for a phase $q$ be
% \[s_q := \frac{2(\sigma_{\eps}+\Upsilon)\sqrt{2^q\max\{L,h\}\log(5/\delta)}}{\left|\sum_{i=L_{q-1}}^{L_q}(x_i-\bar{x})(z_i-\bar{z})\right|}.\] Assume that after the elimination, at every iteration a sample of the eliminated arm is also drawn, but not revealed to the agent.\\
% We define the event $\cC_1$ as the accuracy guarantee of $\hat{\theta}$ such that:
% \begin{equation}
% \label{eq:event-C-1}
%     \cC_1 := \left\{ \forall q \geq L: |\theta - \hat{\theta}_q| < s_q \right\}
% \end{equation}
% where $L$ is the number of samples after running the sampling stage.\\
% Let $X^a_q$ be the number of arm $a\in\{0,1\}$ samples in phase $q$. The decision threshold $s_q$ in phase $q$ is unbounded if $X^a_q=0$ for either arm $a$. We also define event $\cC_2$ where there is at least one sample of each arm in each phase:
% \begin{equation}
% \label{eq:event-C-2}
%     \cC_2 := \left\{\forall q\geq L,a: X^a_q \geq 1 \right\}
% \end{equation}
% Recall that $p_i$ of the population is type $i$. Then, if \cref{alg:racing-two-types-mixed-preferences} is BIC for all agents of type 1 and we recommend each arm at least $h2^{q-2}$ times in phase $q$, we have $X^0_q>h2^{q-2}$ and $X^1_q \sim B(h2^{q-2},p_1)$. Hence, we have
% \begin{equation}
%     \Prob[X^1_q \geq 1] = 1 - p_1^{h2^{q-2}} = \delta'.
% \end{equation}

% Let $\tau\in(0,1)$. Fix phase $q\geq L$, and some agent $t$ in this phase. In order to prove that \cref{alg:racing-two-types-mixed-preferences} is BIC for all agents of type 0, we want to show that 
% \begin{equation}
%     \label{eq:racing-bic-type0}
%     \E_{\cP_0}[\theta\vert z_t=1]\Prob_{\cP_0}[z_t=1] \geq 0.
% \end{equation}


% \lscomment{Start: Need to edit this part}
% Note that, by assumption, the parameter
% \begin{align*}
%     h &\geq \frac{\log\left(\frac{3\tau\Prob_{\cP_0}[\theta\geq\tau]+4}{4\tau\Prob_{\cP_0}[\theta\geq\tau]+4}\right)}{\log(1-p_2)}\\
%     \Rightarrow \left(\frac{1}{2}
%     \right)^h 
%     &\geq \frac{3\tau\Prob_{\cP_0}[\theta\geq\tau]+4}{4\tau\Prob_{\cP_0}[\theta\geq\tau]+4}\\
%     \Rightarrow \delta' = 1 - \left(\frac{1}{2}\right)^h 
%     &\leq \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{4\tau\Prob_{\cP_0}[\theta\geq\tau]+4}.
% \end{align*}
% \lscomment{End: Need to edit this part}

% From Theorem ~\eqref{thm:approximation-bound}, with probability $\delta>0$ we have that
% \begin{equation*}
%     \Prob[\neg \cC_1 \vert G] \leq \delta
% \end{equation*} 
% \dncomment{Is it G or $\theta$ here?}
% Define event $\cC$ such that both events $\cC_1$ and $\cC_2$ hold simultaneously in a round: 
% \begin{equation}
% \label{eq:event-C}
%     \cC := \left\{ \forall q \geq L_1: \cC_1 \  \& \ \cC_2 \right\}
% \end{equation}

% Using union bound, we have
% \begin{align}
%     \Prob[\neg \cC \vert G] &\leq \Prob[\neg \cC_1 \vert G] + \Prob[\neg \cC_2 \vert G]\\
%     &\leq \delta + \delta' \nonumber\\
%     &\leq \delta_{\tau} + \delta' \nonumber \\
%     &\leq \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{4\tau\Prob_{\cP_0}[\theta\geq\tau]+4} + \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{4\tau\Prob_{\cP_0}[\theta\geq\tau]+4} \nonumber \\
%     &= \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2\tau\Prob_{\cP_0}[\theta\geq\tau]+2} \label{eq:delta'}
% \end{align}
% Therefore, since $\theta\geq -1$, we have: 
% \begin{align*}
% \label{eq:racing-bic}
%     \E_{\cP_0}[\theta|z_t=1]\Prob_{\cP_0}[z_t=1] &= \E_{\cP_0}[\theta|z_t=1, \cC]\Prob_{\cP_0}[z_p = 2, \cC] + \E_{\cP_0}[\theta|z_t=1, \neg C]\Prob_{\cP_0}[z_t=1, \neg C]\\
%     &\geq \E_{\cP_0}[\theta|z_t=1, \cC]\Prob_{\cP_0}[z_t=1, \cC] - \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2\tau\Prob_{\cP_0}[\theta\geq\tau]+2} 
% \end{align*}
% We want to upper bound the first term. This can be done by splitting it into four cases based on the value of $\theta$. We have:

% \begin{equation} 
%     \begin{split}
%     \E_{\cP_0}[\theta|z_t=1,\cC]\Prob_{\cP_0}[z_t=1, \cC] = 
%     &\E_{\cP_0}[\theta|z_t=1, \cC, \dnedit{\theta} \geq \tau]\Prob_{\cP_0}[z_p= \e_2, \cC, \dnedit{\theta}\geq \tau] \\
%     &\ + \E_{\cP_0}[\theta|z_t=1, \cC, 0 \leq \dnedit{\theta} < \tau]\Prob_{\cP_0}[z_t=1, \cC, 0 \leq \dnedit{\theta} < \tau] \\
%     &\ + \E_{\cP_0}[\theta|z_t=1, \cC, -2s_q < \dnedit{\theta} < 0]\Prob_{\cP_0}[z_t=1, \cC, -2s_q < \dnedit{\theta} < 0] \\
%     &\ + \E_{\cP_0}[\theta|z_t=1, \cC, \dnedit{\theta} \leq -2s_q]\Prob_{\cP_0}[z_t=1, \cC, \dnedit{\theta}\leq -2s_q] \label{eq:racing-bic-cases}
%     \end{split}
% \end{equation}

% \lscomment{Start: Need to edit this part to prove that $s_q\leq s_L$ for all $q>L$} We want to prove that the approximation bound $s_q$ defined over the samples $\{x_i,z_i,y_i\}_{i=L_{q-1}}^{L_q}$ is less than that of the sampling stage, i.e. $s_q\leq s_L,\,\forall\,q\geq1$. 

% \begin{align*}
%     \frac{s_q}{s_L}
%     &=\frac{2(\sigma_{\eps}+\Upsilon)\sqrt{2^q\max\{L,h\}\log(5/\delta)}}{\left|\sum_{i=L_{q-1}}^{L_q}(x_i-\bar{x})(z_i-\bar{z})\right|} \frac{\left|\sum_{i=1}^L(x_i-\bar{x})(z_i-\bar{z})\right|}{2\left(\sigma_{\eps}+\Upsilon\right)\sqrt{2L\log(5/\delta)}}\\
%     &\leq \sqrt{\frac{2^{q-1}\max\{L,h\}}{L}}\frac{\left|\sum_{i=1}^L(x_i-\bar{x})(z_i-\bar{z})\right|}{\left|\sum_{i=L_{q-1}}^{L_q}(x_i-\bar{x})(z_i-\bar{z})\right|}\\
%     &= \sqrt{\frac{2^{q-1}\max\{L,h\}}{L}}\frac{\left|\sum_{i=1}^L(x_i-\bar{x})(z_i-1/\rho)\right|}{\left|\sum_{i=L_{q-1}}^{L_q}(x_i-\bar{x})(z_i-1/2)\right|}\\
%     &\leq\frac{\tau\Prob_{\cP_0}[\theta>\tau]}{4}-\frac{\nu}{2}
% \end{align*}

% Clearly, the numerator of $s_q$ is greater than or equal to the numerator of $s_L$ for $q\geq1$:
% \[2(\sigma_{\eps}+\Upsilon)\sqrt{2^q\max\{L,h\}\log(5/\delta)}\geq2(\sigma_{\eps}+\Upsilon)\sqrt{2L\log(5/\delta)}\]

% Observe that $s_q$, we have:
% \begin{align*}
%     2s_q &\leq 2s_{L}\\
%     &\leq \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2}-\nu\\
%     &\leq \tau
% \end{align*}

% \lscomment{End: Need to edit this part to prove that $s_q\leq s_L$ for all $q>L$}

% Conditional on $\cC$, the empirical estimate $\dnedit{\hat{\theta}_q} > \dnedit{\theta} - s_q \geq 2s_q$. Hence, when we have $\dnedit{\theta} \geq \tau \geq 2s_q$, then $\dnedit{\hat{\theta}}\geq s_q$ and arm 0 must have already been eliminated at phase $q \geq L_1$. This implies that the probability $\Prob_{\cP_0}[z_t=1, \cC, \dnedit{\theta}\geq \tau] = \Prob_{\cP_0}[\cC, \dnedit{\theta}\geq \tau]$. Similarly, when we have $\dnedit{\theta} \leq -2s_q$, then $\dnedit{\hat{\theta}} \leq -s_q$ and arm 1 must have already been eliminated at phase $q \geq L_1$. Hence, arm 1 could not be recommended in that case and the probability $\Prob_{\cP_0}[z_t=1, \cC, G\leq-2s_q] = 0$.\\
% We can then rewrite equation~\eqref{eq:racing-bic-cases} as
% \begin{align*} 
%     \E_{\cP_0}[\theta|z_t=1, \cC]\Prob_{\cP_0}[z_t=1 ,\cC] \geq &\E_{\cP_0}[\theta|z_t=1, \cC, \dnedit{\theta} \geq \tau]\Prob_{\cP_0}[z_p= \e_2, \cC, \dnedit{\theta} \geq \tau]\\
%     &+ \E_{\cP_0}[\theta|z_t=1, \cC, 0 \leq \dnedit{\theta} < \tau]\Prob_{\cP_0}[z_t=1, \cC, 0 \leq \dnedit{\theta} < \tau]\\
%     &+ \E_{\cP_0}[\theta|z_t=1, \cC, -2s_q < \dnedit{\theta} < 0]\Prob_{\cP_0}[z_t=1, \cC, -2s_q < \dnedit{\theta} < 0]\\
%     \geq &\tau \Prob_{\cP_0}[\cC, \dnedit{\theta} \geq \tau] + 0\cdot \Prob_{\cP_0}[\cC, 0 \leq \dnedit{\theta} < \tau] -2s_q \Prob_{\cP_0}[z_t=1, \cC, -2s_q<\dnedit{\theta}<0]\\
%     \geq &\tau \Prob_{\cP_0}[\cC, \dnedit{\theta} \geq \tau] - 2s_q\\
%     \geq &\tau \Prob_{\cP_0}[\cC, \dnedit{\theta} \geq \tau] - \frac{\tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau]}{2}\\
%     \geq &\tau \Prob_{\cP_0}[\cC | \dnedit{\theta} \geq \tau] \Prob_{\cP_0}[\dnedit{\theta} \geq \tau] - \frac{\tau \Prob_{\cP_0}[G \geq \tau]}{2}\\
%     \geq &\tau (1 - (\delta + \delta')) \Prob_{\cP_0}[\dnedit{\theta} \geq \tau] - \frac{\tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau]}{2}\\
%     = & \left(\frac{1}{2} - (\delta + \delta') \right) \tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau]\\
%     \geq & \left(\frac{1}{2} - \frac{\frac{1}{2} \tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau]}{\tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau] + 1} \right) \tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau] \tag{by Equation~\ref{eq:delta'}}\\
%     = & \frac{1}{2} \left(\frac{\tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau] + 1 - \tau \Prob_{\cP_0}[\dnedit{\theta}\geq \tau]}{\tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau] + 1} \right)\tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau]\\
%     = & \frac{1}{2} \left(\frac{\tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau]}{\tau \Prob_{\cP_0}[\dnedit{\theta} \geq \tau] + 1} \right)
% \end{align*}
% Hence, we have 
% \begin{align*}
%     \E_{\cP_0}[\theta|z_t=1]\Prob_{\cP_0}[z_t=1] &\geq \E[\theta|z_t=1, \cC]\Prob_{\cP_0}[z_t=1, \cC] - \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2\tau\Prob_{\cP_0}[\theta\geq\tau]+2} \\
%     &\geq \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2\tau\Prob_{\cP_0}[\theta\geq\tau]+2}  -  \frac{\tau\Prob_{\cP_0}[\theta\geq\tau]}{2\tau\Prob_{\cP_0}[\theta\geq\tau]+2} \\
%     &= 0
% \end{align*}
% Therefore, Algorithm~\ref{alg:racing-two-types-mixed-preferences} fulfills equation~\ref{eq:racing-bic-type0} and is BIC for all agents of type \dnedit{0}.
% \end{proof}
\newpage

==> regret.tex <==
\subsection{Regret Analysis}\label{sec:regret}
The goal of this algorithm is to maximize the cumulative reward of all agents. We measure the algorithm's performance through the definition of regret. We are interested in minimizing the ex-post regret of the algorithm, which is the regret specific to the treatment effect $\theta$. Since the priors are not exactly known to the social planner, this ex-post regret is correct for any realization of the priors and treatment effect $\theta$. 
\begin{definition} [Ex-post Regret] The ex-post regret of the algorithm is
	\begin{equation}
	R_\theta(T) = T \theta{a^*} - \sum_{t=1}^T \theta x_t
	\end{equation}
	The Bayesian expected regret of the algorithm is:
	\begin{equation}
	R_{\cP}(T) = \E\left[T \theta{a^*} - \sum_{t=1}^T \theta x_t \right] = \E[R_\theta(T)]
	\end{equation}
	where if $\theta > 0$, then $\theta^{a^*}=\theta$; and otherwise if $\theta\leq0,$ then $\theta^{a^*}=0$.
\end{definition}

Using these definitions, our entire algorithm (with the sampling stage and the racing stage) achieves sub-linear ex-post regret. 
\begin{restatable}[Regret]{lemma}{expostregret}\label{lemma:expost-regret}
\Cref{alg:sampling-control-treatment,alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves ex-post regret
\begin{equation}
R(T) \leq \ell_1 \rho + O(\sqrt{T\log T})
\end{equation}
where $\ell_1$ is the sampling stage's phase length and $1/\rho$ is the exploration probability in the sampling stage. 
\end{restatable}
\dndelete{
\begin{proof}
See Appendix \ref{sec:expost-proof} for a proof.
\end{proof}
}
% \begin{lemma} (Regret) 
% \label{lemma:expost-regret}
% Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves ex-post regret
% \begin{equation}
% R(T) \leq \ell_1 \rho + O(\sqrt{T\log T})
% \end{equation}
% where $\ell_1$ is the sampling stage's phase length and $1/\rho$ is the exploration probability in the sampling stage. 
% \end{lemma}
With similar analysis, we also achieve sub-linear expected regret over the randomness in the priors of the agents. \Cref{lemma:expected-regret} provides a basic performance guarantee of our algorithm. 
\begin{restatable}[Expected Regret]{lemma}{expectedregret}\label{lemma:expected-regret}
\Cref{alg:sampling-control-treatment,alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves expected regret
\begin{align}
\E[R(T)] = O(\sqrt{T\log T})
\end{align}
\end{restatable}
\dndelete{
\begin{proof}
See Appendix \ref{sec:expected-regret-proof} for a proof.
\end{proof}
}
% \begin{lemma} (Expected Regret)
% \label{lemma:expected-regret}
% Algorithm \ref{alg:sampling-control-treatment} and \ref{alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ achieves expected regret
% \begin{align}
% \E[R(T)] = O(\sqrt{T\log T})
% \end{align}
% \end{lemma}

These results are analyzed via standard technique and are comparable to the regret of the classic multi-armed bandit problem, with some added constants factors for the BIC constraints \cite{active-arms-elimination-2006}. Although the regret of our algorithm is the same as the fully incentive-compatible algorithm for both types, our algorithm can finish in a more timely manner and has smaller prior-dependent constants in the asymptotic bound.

From the analysis in \cref{lemma:expost-regret}, we can derive the type-specific regret for each type of agent. Since our algorithm does not guarantee that all agents follow our recommendation, this regret analysis is divided into two cases, depending on the best arm overall. If we assume that proportions of each type in the population are equal, \cref{lemma:type-specific-regret} below demonstrates the type-specific regret guarantee of our algorithm.
\begin{restatable}[Type-specific regret]{lemma}{typespecifictwoarms}\label{lemma:type-specific-regret}
\Cref{alg:sampling-control-treatment,alg:racing-two-types-mixed-preferences} with parameters $\ell_1, \rho \in \NN$ and known constant $\tau \in (0,1)$ such that $\tau \Prob_{\cP_i}[\theta \geq \tau] > 0$ achieves type-specific regrets in \cref{tab:type-specific-regret}.
\begin{table*}[ht]
    \centering
    \caption{Type-Specific Regret for Two Arms \& Two Types with partially BIC Algorithm}
    \begin{tabular}{ll}
    \toprule
    Best arm / Type     & Type-specific regret \\
    \midrule
    Arm 0 / Type 0     & $O\left(\frac{\log T }{(\tau \Prob_{\cP_0}[\theta \geq \tau])^2} \right) + O(\sqrt{T\log T})$\\
    Arm 0 / Type 1      & $O\left(\frac{\log T}{(\tau \Prob_{\cP_0}[\theta \geq \tau])^2} \right) + O\left(\frac{\log T}{(\tau\Prob_{\cP_1}[\theta < -\tau])^2}\right) + O(\sqrt{T\log T})$ \\
    Arm 1 / Type 0      & $O\left(\frac{\log T}{(\tau \Prob_{\cP_0}[\theta \geq \tau])^2}\right) +O(\sqrt{T\log T})$\\
    Arm 1 / Type 1      &  $O(\sqrt{T\log T})$ \\
    \bottomrule
    \end{tabular}
    
    \label{tab:type-specific-regret}
\end{table*}
\end{restatable}
\dndelete{
\begin{proof}
See Appendix \ref{sec:type-specific-regret-proof} for a proof.
\end{proof}
}
\lscomment{I don't think the notion of ``fully BIC'' makes sense in the mixed preference setting.}

\lsdelete{
\begin{definition}\label{def:fully-bic-algo}[Fully BIC Algorithm]
A \textit{fully BIC} algorithm is BIC for all agents at all rounds, similar to the detail-free algorithm in \cite{mansour2015bic}. We implement the sampling stage sub-algorithm~\eqref{alg:sampling-control-treatment} to be BIC for agents of type 0. Then, we run the racing stage sub-algorithm~\eqref{alg:racing-two-types-mixed-preferences} starting from the second racing stage, wherein recommendations are BIC for all agents.
\end{definition}

\begin{remark}[Regret Comparison Between Fully BIC and Partially BIC Algorithms]\label{remark:regret-comparison-2-arm}
The type-specific regret for the fully BIC algorithm (\cref{def:fully-bic-algo}) is the same as the type-specific regret for our partially BIC algorithm (see Table~\ref{tab:type-specific-regret}) wherein we replace the prior-dependent constant term $\tau^2 \Prob_{\cP_0}[G \geq \tau]$ for type 0 with the prior-dependent constant term $\tau^2 \Prob_{\cP_1}[G < -\tau]$ for type 1, which can be arbitrarily large. In the full version of our paper, we work out a case wherein the priors over the treatment reward $\theta$ for each type are Gaussian and the fully BIC algorithm (\cref{def:fully-bic-algo}) achieves linear regret $\Omega(T)$, but our algorithm achieves sub-linear regret $O(\sqrt{T\log T})$.
\end{remark}
}%end lsdelete

==> two-arm-generalization.tex <==
\section{Warmup: two arms and two types}\label{sec:two-arms-two-priors}

In this section, we provide a concrete example to demonstrate how our algorithm works. We consider a simple setting which entails only two arms (either control or treatment) and two types of agents. Each type has a different Bayesian prior over the rewards of these two arms: one type prefers the control and one prefers the treatment.

At a high level, our algorithm follows the structure of the  BIC mechanism of \cite{mansour2015bic} with two key modifications. In particular, our algorithm is no longer required to be BIC for all agents. As a result, it can obtain a better regret bound whenever one of the types is more compliant. Also, our mechanism estimates the action effects $\theta$ with IV regression. Our algorithm runs in two stages: first, the \textit{sampling stage} and then the \textit{racing stage}. The sampling stage sub-algorithm collects $L_2$ samples of each arm. These $L_2$ samples are then input as a parameter into the racing stage algorithm, which recommends each arm one-by-one until one arm ``wins.'' We design the algorithm to incentivize one type to be compliant throughout. We are able to do so because we employ an instrumental variable (IV) regression in order to estimate the true treatment effect of each arm. Because we require only partial incentive-compatibility, our algorithm achieves better regret than a fully BIC algorithm similar to that of the detail-free algorithm in \cite{mansour2015bic} would.
%  \lscomment{Cite a spot where the fully BIC algorithm is explicitly demonstrated?}

This section is organized as follows:
Section~\ref{sec:assumptions-two-arms} lays out the background assumptions for this two-arm two-type setting. Section~\ref{sec:sampling-two-arms-two-types} outlines assumptions needed for the sampling stage algorithm, demonstrates said algorithm in \cref{alg:sampling-two-types-general}, and proves that it is BIC for one type in \cref{lemma:bic-sampling-two-arms-general}. Section~\ref{sec:racing-two-arms-two-types} also notes assumptions needed for the racing stage, demonstrates the racing stage algorithm (\cref{alg:racing-two-types-general}), and proves incentive-compatibility first for one type, then later for both. Finally, Section~\ref{sec:regret-two-arms-two-types} states the overall expected regret and the type-specific regrets for our algorithm in lemma~\ref{lemma:ex-post-2-arm}, \ref{lemma:expected-regret-two-arms}, and \ref{lemma:type-specific-two-arm}. In \cref{remark:regret-comparison-2-arm}, we demonstrate the advantage of our algorithm by comparing the type-specific regret of our algorithm to that of a fully BIC algorithm.

\subsection{Setting Assumptions}\label{sec:assumptions-two-arms} Before we present the algorithm, we present our background assumptions. 
\begin{assumption} \label{assumption:two-arms}
    The entire population of agents has two types, i.e. type 1 and type 2. The proportions of agents of either type in the population are equal. Each type $i$ has a Bayesian prior, namely $\cP_i$, over the distribution of the mean reward vector $\theta$. For each type $i$, the prior mean reward of arm $a$ is given by $\mu^a_i := \E_{\cP_i}[\theta^a]$. \swedit{We assume that 
    $\mu^a_i\in [-1, 1]$ for all actions $a$ and types $i$,} and the arms are ordered according to their prior mean rewards and that this ordering is shared across types, i.e. $\mu^1_{i} > \mu^2_{i}$ for either type $i\in\{1,2\}$.
\end{assumption}

If agents were left to their own devices, we would only see samples of arm 1, since all agents prefer arm 1 to arm 2. Thus, we need to incentivize agents to choose arm 2 via our recommendations. 

%However, because we use IV regression to estimate the treatment effect, we do not need to enforce full compliance from every agent. Thus, our algorithm primarily incentivizes type 2 agents to comply with our recommendations.

\subsection{Sampling Stage Algorithm for Two Arms and Two Types}\label{sec:sampling-two-arms-two-types}
Following the two-arm fully BIC sampling stage algorithm in \cite{mansour2015bic}, \cref{alg:sampling-two-types-general} capitalizes on an information asymmetry between the agents and the social planner in order to incentivize the agents to comply to the its recommendations. 
However, while the fully BIC sampling stage is BIC for all agents at all rounds, \cref{alg:sampling-two-types-general} is designed to be BIC for agents of a given type $i$.\footnote{\cite{mansour2015bic} does not explicitly consider agents of heterogeneous types. However, we consider an extension of their algorithm in our setting as an algorithm that is BIC for agents of all types at all rounds.} In our \textit{partially BIC} algorithm, we implement \cref{alg:sampling-two-types-general} to be BIC for agents of type 2, because these agents are easier to convince to be BIC under our recommendation policy than are agents of type 1. In Section~\ref{sec:regret-two-arms-two-types}, we demonstrate how implementing a partially BIC algorithm which is BIC for only agents of a single type allows for improvements in regret over a fully-BIC algorithm which is BIC for agents of all types.

In the first phase of \cref{alg:sampling-two-types-general}, we recommend only arm 1: this recommendation confers no information about the history and each agent chooses the better arm according to their prior, i.e. arm 1. Thus, we observe the rewards from $L_2$ samples of arm 1. For a given type $i$, there is a non-zero chance that arm 1 performs so poorly that the prior of arm 2 looks better than the posterior of arm 1 conditioned on these $L_2$ samples. For type $i$, define this event as
\begin{equation}
    \xi_i = \left\{ \frac{1}{L_2}\sum_{t = 1}^{L_2} y^1_t + \frac{1}{2} + \nu + \Upsilon + \sigma_\epsilon \sqrt{\frac{2\log(1/\delta)}{L_2}} < \mu^2_i \right\},
\end{equation}
where $\delta$ is a sampling failure probability to be determined.

Starting in the second phase of the sampling stage, we recommend either an arm to exploit or an arm to explore. If event $\xi_i$ occurs, the algorithm always recommends arm 2 to \textit{exploit}. The algorithm also \textit{explores} by recommending arm 2 to $L_2$ agents (out of $\rho L_2$ in total, where $1/\rho$ represents the exploration probability). Thus, when any agent receives a recommendation for arm 2, there is a chance that it is because $\xi_i$ occurred and there is a chance that it is because the algorithm chose them to explore on. If the exploration probability is small enough (i.e. $\rho$ is large enough), then agents of type $i$ are always inclined to follow a recommendation for arm 2.

We order the two types such that agents of type 1 require a smaller exploration probability than agents of type 2. As such, we implement \cref{alg:sampling-two-types-general} to be BIC for only agents of type 2.

We use a set of assumptions to limit the prior to ensure that our algorithm has a chance to recommend the weaker arm and that our estimates are close to the true treatment effects. Hence, we restrict the priors to be independent across arms, with bounded treatment effects and confounder.

\begin{algorithm}[H]
\SetAlgoLined
\SetKwInput{KwIn}{Input}
\KwIn{parameters $\rho, L_2 \in \mathbb{N}$ and $0<\delta<\delta'$, where $\delta':=\frac{\Prob_{\cP_i}[\xi_i]}{8}$}
In the first $L_2$ rounds, let the agents pick their preferred arm (arm 1). The sample average of reward $y^1$ after $L_2$ pulls of arm $1$ is denoted $\bar{y}^1_{L_2}$. After that, do the following:\\
    \eIf{$\displaystyle \mu^2_2 > \bar{y}^1_{L_2}+ \frac{1}{2} + \nu + \Upsilon + \sigma_{\epsilon}\sqrt{\frac{2\log(1/\delta)}{L_2}}$}
    {$a^* = 2$} 
    {$a^* = 1$}
    From the set $P$ of the next $L_2.\rho$ agents, pick a set $Q$ of $L_2$ agents uniformly at random.\\
    Every agent $t \in P - Q$ is recommended arm $a^*$.\\
    Every agent $t \in Q$ is recommended arm 2.
        \caption{The general sampling stage for two arms with two heterogeneous types}
    \label{alg:sampling-two-types-general}
\end{algorithm}

We prove that the algorithm $\ref{alg:sampling-two-types-general}$ is BIC for agents of type $i$ as long as the number of phases $\rho$ is larger than some prior-dependent constant. The intuition is when an agent of type $i$ is recommended arm 2, they do not know whether this is due to exploration or exploitation. However, with large enough number of phases $\rho$, the exploration probability $1/\rho$ is low enough that the expected gain from exploiting exceed the expected loss from exploring and the agent would take arm 2. 

\begin{restatable}[Two Arm Sampling Stage BIC for Type $i$]{lemma}{bicsamplingtwoarmsgeneral}\label{lemma:bic-sampling-two-arms-general}
    \Cref{alg:sampling-two-types-general} with parameters $(\rho, L_2)$ completes in $L_2\rho + L_2$ rounds. \Cref{alg:sampling-two-types-general} is BIC for all agents of type $i$ if we hold Assumption~\ref{assumption:two-arms} above and the parameters satisfy:
    %\vspace{-2cm}
    \begin{equation}
        \rho \geq 1 + \frac{4(\mu_i^1 - \mu_i^2 + \nu\Prob_{\cP_i}[\xi_i])}{\Prob_{\cP_i}[\xi_i]}.
    \end{equation}
\end{restatable}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Racing Stage %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Racing Stage Algorithm for Two Arms and Two Types}\label{sec:racing-two-arms-two-types} 
From the sampling stage, we get a set of observations for $L_2\rho + L_2$ rounds. Because, as shown in \cref{lemma:bic-sampling-two-arms-general}, agents of type 2 will always follow our recommendation, this allows us to induce variability among the action choices of type 2 agents and get samples of arm 2. This allows the empirical compliance matrix $\hat{\Gamma}$ to have all positive singular values. Thus, we can use our recommendations as instruments and regress over them (using IV regression) to estimate the exogenous mean rewards $\hat{\theta}^1$ and $\hat{\theta}^2$. 

In the racing stage (\cref{alg:racing-two-types-general}), each arm will be recommended one-by-one until one of them can be determined to be optimal with high confidence. After that, the racing stage has ended the ``winner'' arm is recommended for the rest of the time horizon. Thus, when an agent gets a recommendation for arm 2, they are not sure whether they are receiving that recommendation because they are still in the racing stage or because it has ended and arm 2 has won. We will leverage this uncertainty to incentivize them to follow the recommendations.

By collecting more samples, we are able to form good enough estimates $\hat{\theta}^1$ and $\hat{\theta}^2$ and increase the likelihood that the racing stage has ended when an agent receives a recommendation for arm 2. Thus, we collect a sufficient number of samples in the sampling stage in order to make the racing stage algorithm BIC for agents of type 2. By similar reasoning as the recommendation in the sampling stage, we can treat the recommendation in the racing stage as an instrument because agents of type 2. We use all $L_2$ samples from the sampling stage and any additional samples in the racing stage in order to estimate the mean rewards $\hat{\theta}^1$ and $\hat{\theta}^2$.

Similar to the sampling stage, we also rely on agents of type 2 to take our arm 2 recommendation in the beginning of the racing stage. Hence, to account for the probability of agent of type 2 getting an arm 2 recommendation, we divide the racing stage into phases of $2h$ rounds each, where each arm is recommended $h$ times in a phase. 

After each phase, we check if the empirical gap $|\hat{\theta}^1 - \hat{\theta}^2|$ is larger than some threshold. If that happens, the arm with the higher estimate is determined with high probability to be the best arm, and all agents are only recommended this arm from now on. To ensure that the winner of the racing stage is indeed the best arm with high probability, we need to pick a threshold large enough, similar to the termination condition in the Active Arm Elimination algorithm from \cite{active-arms-elimination-2006}.

We also divide the racing stage into two smaller sub-algorithms. The first part of the racing stage is partially BIC, where we guarantee that only agents of type 2 will comply with our recommendations. After collecting sufficient samples of arm 2, if the algorithm has not found the ``winner'' yet, we can proceed to the second part of the racing stage. At this point, we have collected enough samples to also convince agents of type 1 to follow our recommendations. By having two consecutive racing stages, we can potentially reduce the regret of our algorithm and achieve a fully BIC algorithm, where every agent follows our recommendations.
\begin{algorithm}[ht!]
\SetAlgoLined
\SetKwInput{KwIn}{Input}
\KwIn{parameters $L_2 \in \mathbb{N}$; time horizon $T$; probability $\delta$, number of recommendations $h$ for a single arm in a single phase, and upper bound $\nu$ on bias function $\phi(u_t)$}
\KwIn{IV estimates of mean reward $\theta^1$ and $\theta^2$, denoted $\hat{\theta}^1_{L_2}$ and $\hat{\theta}^2_{L_2}$}
    Let $\hat{\theta}^1_{L_2}$ and $\hat{\theta}^2_{L_2}$ be the IV estimate of the mean reward $\theta^1$ and $\theta^2$ after $L_2\rho$ rounds of Algorithm 1;\\
    Split remainder into consecutive phases of $2h$ rounds each, starting from phase $q = L_2$;\\
    \While{$q < \frac{147456(\log(3T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\left(\frac{\tau\Prob_{\cP_1}[G \geq \tau]}{2} - \nu \right)^2}$}
    {\While{$|\hat{\theta}^1_q - \hat{\theta}^2_q| \leq 192\sqrt{\frac{\log(3T/\delta) + 3\log(2T(2+\Upsilon^2))}{q}}$}
    {
    The next $2h$ agents are recommended both arms sequentially;\\
    For each arm $a \in \{1, 2\}$, let $y^a_t$ be one sample reward of that arm in this phase;\\
    Let $\hat{\theta}^a_{q}$ is the IV estimate of the reward of each arm $a \in \{1, 2\}$ for the racing stage up to and including phase $q$;\\
    $q = q+1$;
    }
    For all remaining agents recommend $a^* = \argmax_{a \in {\{1, 2\}}} \hat{\theta}^a_q$ and end the algorithm.} 
    \While{$|\hat{\theta}^1_q - \hat{\theta}^2_q| \leq 192\sqrt{\frac{\log(3T/\delta) + 3\log(2T(2+\Upsilon^2))}{q}}$}
    {
    The next $2h$ agents are recommended both arms sequentially;\\
    For each arm $a \in \{1, 2\}$, let $y^a_q$ be one sample reward of that arm in this phase;\\
    Let $\hat{\theta}^a_{q}$ is the IV estimate of the reward of each arm $a \in \{1, 2\}$ for the racing stage up to and including phase $q$;\\
    $q = q+1$;
    }
    For all remaining agents recommend $a^* = \argmax_{a \in {\{1, 2\}}} \hat{\theta}^a_q$
    \caption{The racing stage for two arms with two heterogeneous types}
    \label{alg:racing-two-types-general}
\end{algorithm}

We prove that \cref{alg:racing-two-types-general} is BIC for all agents of type 2 as long as we have collected sufficient samples of arm 2 in the sampling stage and our estimate of $\theta$ is close to the true treatment effect. Due to information asymmetry, when an agent is recommended arm 2, they do not know whether the two arms are still racing each other or if the best arm has been found. However, with a small enough threshold, the expected gain from exploiting the best arm exceeds the expected loss from exploring a random arm and the agents of type 2 would follow our recommendation. 


\begin{restatable}[Type 2 BIC]{lemma}{racingbictwotypesgeneral}\label{lemma:racing-bic-two-types-general}
    Let $\displaystyle G := \theta^2 - \theta^1$. Assume that there exists a fixed constant $\tau \in (0,1)$ such that $\tau \Prob_{\cP_1}[G \geq \tau] > 2\nu$ and $\tau \Prob_{\cP_2}[G \geq \tau] \geq 2\nu$. Let \[\delta_{\tau} = \frac{1}{4}\frac{\tau \Prob_{\cP_2}[G \geq \tau]}{\tau \Prob_{\cP_2}[G \geq \tau] + 1}.\] Algorithm~\ref{alg:racing-two-types-general} is BIC for all agents of type 2 if the parameters satisfy $\delta \leq \delta_{\tau}$ and
    \[h \geq -\frac{\log\left(\frac{3\tau \Prob_{\cP_2}[G \geq \tau]+4}{4\tau \Prob_{\cP_2}[G \geq \tau] + 4}\right)}{\log(2)}\] and
    \[L_2 \geq \frac{147456(\log(3T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\left(\frac{\tau (\Prob_{\cP_2}[G \geq \tau]}{2} - \nu \right)^2}.\]
\end{restatable}

During the first racing stage, we collect more samples of arm 2 through agents of type 2. After getting sufficient samples of arm 2, we can also convince agents of type 1 to follow our recommendations for arm 2. The following Lemma $\ref{lemma:racing-bic-two-types-type-1-general}$, which follows the same structure as that of Lemma $\ref{lemma:racing-bic-two-types-general}$, proves that the second racing stage algorithm is BIC for both agents of type 1 and type 2.  


\begin{restatable}[Type 1 BIC]{lemma}{racingbictwotypestypeonegeneral}\label{lemma:racing-bic-two-types-type-1-general}
    Let $\displaystyle G := \theta^2 - \theta^1$. Fix an absolute constant $\tau \in (0, 1)$ and let \[\delta_{\tau} = \frac{1}{2}\frac{\tau \Prob_{\cP_1}[G \geq \tau]}{\tau \Prob_{\cP_1}[G \geq \tau] + 1}.\] Algorithm~\ref{alg:racing-two-types-general} is BIC for all agents of type 1 if the parameters satisfy $\delta \leq \delta_{\tau}$ and
    \[L_1 \geq \frac{147456(\log(3T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\left(\frac{\tau (\Prob_{\cP_1}[G \geq \tau]}{2} - \nu \right)^2}.\]
\end{restatable}


%\section{Regret}
\subsection{Regret Analysis}\label{sec:regret-two-arms-two-types}
With the number of samples of each arm collected in the sampling stage $L_2$, the number of sampling stage phases $\rho$ and the accuracy guarantee of our estimate $\delta$, our sampling stage and racing stage algorithms achieve sub-linear regret for a particular instance of the treatment effect vector $\theta$. Since the priors are not exactly known to the social planner, this ex-post regret is correct for any realization of the priors and treatment effect vector $\theta$.  

\begin{restatable}[Regret]{lemma}{regrettwoarms}\label{lemma:ex-post-2-arm}
    Algorithm 1 and 2 with parameters $L_2, \rho \in \mathbb{N}$ and $\delta \in (0,1)$ achieves ex-post regret:
    \begin{equation}
        R(T) \leq L_2\rho + O(\sqrt{T\log(T/\delta)}) 
    \end{equation}
    where $\Delta = |\theta^1 - \theta^2|$,  $L_2$ is the duration of one phase in the initial sampling stage and $\frac{1}{\rho}$ is the exploration probability in the sampling stage.
\end{restatable}

With the number of samples of each arm collected in the sampling stage $L_2$, the number of sampling stage phases $\rho$, and the accuracy guarantee of our estimate $\delta$, our sampling stage and racing stage algorithms achieve sub-linear Bayesian regret over the randomness in the priors of the agents. Lemma $\ref{lemma:expected-regret-two-arms}$ provides a basic performance guarantee of our algorithm. 
\begin{restatable}[Expected Regret]{lemma}{expectedregrettwoarms}\label{lemma:expected-regret-two-arms}  
    Algorithm with parameters $L_2. \rho \in \mathbb{N}$ and $\delta = 1/{T^2}$ achieves expected ex-post regret.
    \begin{equation}
        \E[R(T)] = O\left( \sqrt{T\log T} \right)
    \end{equation}
    where $T$ is the time horizon.
\end{restatable}

From the regret analyzed in \cref{lemma:ex-post-2-arm}, we can derive the type-specific regret of each type of agent. Since our algorithm does not guarantee that all agents follow our recommendations in the sampling stage and the first racing stage, the type-specific regret is divided into two cases, depending on the best arm overall. In addition to the regret in \cref{lemma:ex-post-2-arm}, this regret also depends on the proportion of each type of agents in the population, which consider to be equal between the two types. Lemma~\ref{lemma:type-specific-two-arm} below demonstrates our type-specific regrets guarantee.
\begin{restatable}[Type-specific regret of a partially BIC algorithm]{lemma}{typespecifictwoarmsgeneral}\label{lemma:type-specific-two-arm} 
   The following type-specific expected regret bounds in \cref{tab:type-specific-regret-heterogeneous} hold.
    
   % We observe the following type-specific regret bounds (for confidence $\delta>0$):
    \begin{table}[H]
    \centering
    \begin{tabular}{|l|l|}
    \hline
    Best arm\ /\ Type & Type-specific Regret \\ \hline
    Arm 1: Type 1 & $O(\log T)$                     \\ \hline
    Arm 1: Type 2 & $O\left(\frac{\log T}{(\tau \Prob_{\cP_2}[G \geq \tau] - \nu)^2}\right) +O(\log T)$                     \\ \hline
    Arm 2: Type 1 & $O\left(\frac{\log T}{(\tau \Prob_{\cP_2}[G \geq \tau] - \nu)^2} \right) + O\left(\frac{\log T}{(\tau\Prob_{\cP_1}[G \geq \tau] - \nu)^2}\right) + O(\sqrt{T\log T})$                     \\ \hline
    Arm 2: Type 2 & $O\left(\frac{\log T }{(\tau \Prob_{\cP_2}[G \geq \tau] - \nu)^2} \right) + O(\sqrt{T\log T})$                     \\ \hline
    \end{tabular}
    \caption{Type-Specific Regret for Two Arms \& Two Types with partially BIC Algorithm}
    \label{tab:type-specific-regret-heterogeneous}
    \end{table}
\end{restatable}

\begin{definition}\label{def:fully-bic-algo}[Fully BIC Algorithm]
A \textit{fully BIC} algorithm is BIC for all agents at all rounds, similar to the detail-free algorithm in \cite{mansour2015bic}. We implement \cref{alg:sampling-two-types-general} to be BIC for agents of type 1 (which will also be BIC for agents of type 2). Then, we run \cref{alg:racing-two-types-general} starting from the second racing stage, wherein recommendations are BIC for all agents.
\end{definition}

\begin{remark}[Regret Comparison Between Fully BIC and Partially BIC Algorithms]\label{remark:regret-comparison-2-arm}
The type-specific regret for the fully BIC algorithm (\cref{def:fully-bic-algo}) is the same as the type-specific regret for our partially BIC algorithm (see \cref{tab:type-specific-regret-heterogeneous}) wherein we replace the prior-dependent constant term $\tau \Prob_{\cP_2}[G \geq \tau]$ for type 2 with the prior-dependent constant term $\tau \Prob_{\cP_1}[G \geq \tau]$ for type 1, which can be arbitrarily large. In the full version of our paper, we work out a case wherein the priors over the treatment reward vector $\theta$ for each type are Gaussian and the fully BIC algorithm (\cref{def:fully-bic-algo}) achieves linear regret $\Omega(T)$, but our algorithm achieves sub-linear regret $O(\sqrt{T\log T})$.
\end{remark}


==> two-arms-two-types.tex <==
\section{Warmup: two arms and two types}\label{sec:two-arms-two-priors}

In this section, we provide a concrete example to demonstrate how our algorithm works. We consider a simple setting which entails only two arms and two types. Each type has a different Bayesian prior over the rewards of these two arms, but both types agree on which arm is better than the other.

At a high level, our algorithm follows the structure of the  BIC mechanism of \cite{mansour2015bic} with two key modifications. In particular, our algorithm is no longer required to be BIC for all agents. As a result, it can obtain a better regret bound whenever one of the types is more compliant. Also, our mechanism estimates the action effects $\theta$ with IV regression. Our algorithm runs in two stages: first, the \textit{sampling stage} and then the \textit{racing stage}. The sampling stage sub-algorithm collects $L_2$ samples of each arm. These $L_2$ samples are then input as a parameter into the racing stage algorithm, which recommends each arm one-by-one until one arm ``wins.'' We design the algorithm to incentivize one type to be compliant throughout. We are able to do so because we employ an instrumental variable (IV) regression in order to estimate the true treatment effect of each arm. Because we require only partial incentive-compatibility, our algorithm achieves better regret than a fully BIC algorithm similar to that of the detail-free algorithm in \cite{mansour2015bic} would.
%  \lscomment{Cite a spot where the fully BIC algorithm is explicitly demonstrated?}

This section is organized as follows:
Section~\ref{sec:assumptions-two-arms} lays out the background assumptions for this two-arm two-type setting. Section~\ref{sec:sampling-two-arms-two-types} outlines assumptions needed for the sampling stage algorithm, demonstrates said algorithm in Algorithm~\ref{alg:sampling-two-types}, and proves that it is BIC for one type in Lemma~\ref{lemma:bic-sampling-two-arms}. Section~\ref{sec:racing-two-arms-two-types} also notes assumptions needed for the racing stage, demonstrates the racing stage algorithm (Algorithm~\ref{alg:racing-two-types}), and proves incentive-compatibility first for one type, then later for both. Finally, Section~\ref{sec:regret-two-arms-two-types} states the overall expected regret and the type-specific regrets for our algorithm in Lemmas~\ref{lemma:ex-post-2-arm}, \ref{lemma:expected-regret-two-arms}, and \ref{lemma:type-specific-two-arm}. In Remark~\ref{remark:regret-comparison-2-arm}, we demonstrate the advantage of our algorithm by comparing the type-specific regret of our algorithm to that of a fully BIC algorithm.

\subsection{Setting Assumptions}\label{sec:assumptions-two-arms} Before we present the algorithm, we present our background assumptions. 
\begin{assumption} \label{assumption:two-arms}
    The entire population of agents has two types, i.e. type 1 and type 2. The proportions of agents of either type in the population are equal. Each type $i$ has a Bayesian prior, namely $\cP_i$, over the distribution of the mean reward vector $\theta$. For each type $i$, the prior mean reward of arm $a$ is given by $\mu^a_i := \E_{\cP_i}[\theta^a]$. We assume that the arms are ordered according to their prior mean rewards and that this ordering is shared across types, i.e. $\mu^1_{i} > \mu^2_{i}$ for either type $i\in\{1,2\}$.
\end{assumption}

If agents were left to their own devices, we would only see samples of arm 1, since all agents prefer arm 1 to arm 2. Thus, we need to incentivize agents to choose arm 2 via our recommendations. 

%However, because we use IV regression to estimate the treatment effect, we do not need to enforce full compliance from every agent. Thus, our algorithm primarily incentivizes type 2 agents to comply with our recommendations.

\subsection{Sampling Stage Algorithm for Two Arms and Two Types}\label{sec:sampling-two-arms-two-types}
Following the two-arm fully BIC sampling stage algorithm in \cite{mansour2015bic}, Algorithm~\ref{alg:sampling-two-types} capitalizes on an information asymmetry between the agents and the social planner in order to incentivize the agents to comply to the its recommendations. 
However, while the fully BIC sampling stage is BIC for all agents at all rounds, Algorithm~\ref{alg:sampling-two-types} is designed to be BIC for agents of a given type $i$.\footnote{\cite{mansour2015bic} does not explicitly consider agents of heterogeneous types. However, we consider an extension of their algorithm in our setting as an algorithm that is BIC for agents of all types at all rounds.} In our \textit{partially BIC} algorithm, we implement Algorithm~\ref{alg:sampling-two-types} to be BIC for agents of type 2, because these agents are easier to convince to be BIC under our recommendation policy than are agents of type 1. In Section~\ref{sec:regret-two-arms-two-types}, we demonstrate how implementing a partially BIC algorithm which is BIC for only agents of a single type allows for improvements in regret over a fully-BIC algorithm which is BIC for agents of all types.

In the first phase of Algorithm~\ref{alg:sampling-two-types}, we recommend only arm 1: this recommendation confers no information about the history and each agent chooses the better arm according to their prior, i.e. arm 1. Thus, we observe the rewards from $L_2$ samples of arm 1. For a given type $i$, there is a non-zero chance that arm 1 performs so poorly that the prior of arm 2 looks better than the posterior of arm 1 conditioned on these $L_2$ samples. For type $i$, define this event as
\begin{equation}
    \xi_i = \left\{ \frac{1}{L_2}\sum_{t = 1}^{L_2} y^1_t + \frac{1}{2} + \Upsilon + \sigma_\epsilon \sqrt{\frac{2\log(1/\delta)}{L_2}} < \mu^2_i \right\},
\end{equation}
where $\delta$ is a sampling failure probability to be determined.

Starting in the second phase of the sampling stage, we recommend either an arm to exploit or an arm to explore. If event $\xi_i$ occurs, the algorithm always recommends arm 2 to \textit{exploit}. The algorithm also \textit{explores} by recommending arm 2 to $L_2$ agents (out of $\rho L_2$ in total, where $1/\rho$ represents the exploration probability). Thus, when any agent receives a recommendation for arm 2, there is a chance that it is because $\xi_i$ occurred and there is a chance that it is because the algorithm chose them to explore on. If the exploration probability is small enough (i.e. $\rho$ is large enough), then agents of type $i$ are always inclined to follow a recommendation for arm 2.

We order the two types such that agents of type 1 require a smaller exploration probability than agents of type 2. As such, we implement Algorithm~\ref{alg:sampling-two-types} to be BIC for only agents of type 2.

We use a set of assumptions to limit the prior to ensure that our algorithm has a chance to recommend the weaker arm and that our estimates are close to the true treatment effects. Hence, we restrict the priors to be independent across arms, with bounded treatment effects and confounder.\\ 
% Since it is harder to convince agents of type 1 to follow our recommendation, we relies on agents of type 2 to collect $L_2$ samples of each arm during the sampling stage. Hence, we based the parameters of this algorithm around the prior of type 2, $\cP_2$.\\ 
% In the samplings stage, we define the exploit arm by comparing the sample average reward of arm 1 with the prior mean reward $\mu^2_2$ of arm 2. To account for the inaccuracy of the average $\bar{y}^1$ in face of the confounder $g(u_t)$, we only choose arm 2 as the exploit arm $a*$ if the prior mean reward $\mu^2_2$ is larger than $\bar{y}^1$ by a sufficient margin. Denote $C = \Upsilon + \sigma_{\epsilon}\sqrt{\frac{2\log(1/\delta)}{L_2}}$ as the margin of the average reward estimate for a particular arm. Once the arm $a*$ is selected, it will be recommended to all agents in the remaining rounds of the sampling stage, except for some agents chosen uniformly at random which are recommended arm 2.\\
% Define the event that the sample average of arm 1 is sufficiently worse than the prior mean reward of arm 2 as $\xi_1$ and $\xi_2$ for type 1 and type 2, respectively where $\xi_1 = \{ \bar{y}^1 + C < \mu^2_1\}$ and $\xi_2 = \{ \bar{y}^1 + C < \mu^2_2\}$. To ensure that arm 2 has a chance to be recommended as the exploit arm , assume that $\Prob[\xi_2] > 0$.\\
\begin{algorithm}[H]
\SetAlgoLined
\SetKwInput{KwIn}{Input}
\KwIn{parameters $\rho, L_2 \in \mathbb{N}$}
In the first $L_2$ rounds, let the agents pick their preferred arm (arm 1). The sample average of reward $y^1$ after pulling arm $1$ $L_2$ times is $\bar{y}^1_{L_2}$.\\
    \eIf{$\displaystyle \mu^2_2 > \bar{y}^1_{L_2}+ \frac{1}{2} + \Upsilon + \sigma_{\epsilon}\sqrt{\frac{2\log(1/\delta)}{L_2}}$}
    {$a^* = 2$} 
    {$a^* = 1$}
    From the set $P$ of the next $L_2.\rho$ agents, pick a set $Q$ of $L_2$ agents uniformly at random.\\
    Every agent $t \in P - Q$ is recommended arm $a^*$.\\
    Every agent $t \in Q$ is recommended arm 2.
        \caption{The sampling stage for two arms with two heterogeneous types}
    \label{alg:sampling-two-types}
\end{algorithm}
We prove that the algorithm $\ref{alg:sampling-two-types}$ is BIC for agents of type $i$ as long as the number of phases $\rho$ is larger than some prior-dependent constant. The intuition is when an agent of type $i$ is recommended arm 2, they do not know whether this is due to exploration or exploitation. However, with large enough number of phases $\rho$, the exploration probability $1/\rho$ is low enough that the expected gain from exploiting exceed the expected loss from exploring and the agent would take arm 2. 

\begin{restatable}[Two Arm Sampling Stage BIC for Type $i$]{lemma}{bicsamplingtwoarms}\label{lemma:bic-sampling-two-arms}
    Algorithm~\ref{alg:sampling-two-types} with parameters $(\rho, L_2)$ completes in $L_2\rho + L_2$ rounds. Algorithm~\ref{alg:sampling-two-types} is BIC for all agents of type $i$ if we hold Assumption~\ref{assumption:two-arms} above and the parameters satisfy:
    %\vspace{-2cm}
    \begin{equation}
        \rho \geq 1 + \frac{4(\mu_2^1 - \mu_2^2)}{\Prob_{\cP_i}[\xi_i]}.
    \end{equation}
\end{restatable}

%\vspace{-5cm}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% Racing Stage %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\subsection{Racing Stage Algorithm for Two Arms and Two Types}\label{sec:racing-two-arms-two-types} 

From the sampling stage, we get a set of observations for $L_2\rho + L_2$ rounds. Because, as shown in Lemma~\ref{lemma:bic-sampling-two-arms}, agents of type 2 will always follow our recommendation, this allows us to induce variability among the action choices of type 2 agents and get samples of arm 2. This allows the empirical compliance matrix $\hat{\Gamma}$ to have all positive singular values. Thus, we can use our recommendations as instruments and regress over them (using IV regression) to estimate the exogenous mean rewards $\hat{\theta}^1$ and $\hat{\theta}^2$. 

In the racing stage (Algorithm~\ref{alg:racing-two-types}), each arm will be recommended one-by-one until one of them can be determined to be optimal with high confidence. After that, the racing stage has ended the ``winner'' arm is recommended for the rest of the time horizon. Thus, when an agent gets a recommendation for arm 2, they are not sure whether they are receiving that recommendation because they are still in the racing stage or because it has ended and arm 2 has won. We will leverage this uncertainty to incentivize them to follow the recommendations.

By collecting more samples, we are able to form good enough estimates $\hat{\theta}^1$ and $\hat{\theta}^2$ and increase the likelihood that the racing stage has ended when an agent receives a recommendation for arm 2. Thus, we collect a sufficient number of samples in the sampling stage in order to make the racing stage algorithm BIC for agents of type 2. By similar reasoning as the recommendation in the sampling stage, we can treat the recommendation in the racing stage as an instrument because agents of type 2. We use all $L_2$ samples from the sampling stage and any additional samples in the racing stage in order to estimate the mean rewards $\hat{\theta}^1$ and $\hat{\theta}^2$.

Similar to the sampling stage, we also rely on agents of type 2 to take our arm 2 recommendation in the beginning of the racing stage. Hence, to account for the probability of agent of type 2 getting an arm 2 recommendation, we divide the racing stage into phases of $2h$ rounds each, where each arm is recommended $h$ times in a phase. 

After each phase, we check if the empirical gap $|\hat{\theta}^1 - \hat{\theta}^2|$ is larger than some threshold. If that happens, the arm with the higher estimate is determined with high probability to be the best arm, and all agents are only recommended this arm from now on. To ensure that the winner of the racing stage is indeed the best arm with high probability, we need to pick a threshold large enough, similar to the termination condition in the Active Arm Elimination algorithm from \cite{active-arms-elimination-2006}.

We also divide the racing stage into two smaller sub-algorithms. The first part of the racing stage is partially BIC, where we guarantee that only agents of type 2 will comply with our recommendations. After collecting sufficient samples of arm 2, if the algorithm has not found the ``winner'' yet, we can proceed to the second part of the racing stage. At this point, we have collected enough samples to also convince agents of type 1 to follow our recommendations. By having two consecutive racing stages, we can potentially reduce the regret of our algorithm and achieve a fully BIC algorithm, where every agent follows our recommendations.

\begin{algorithm}[ht!]
\SetAlgoLined
\SetKwInput{KwIn}{Input}
\KwIn{parameters $L_2 \in \mathbb{N}$; time horizon $T$; probability $\delta$, number of recommendations $h$ for a single arm in a single phase}
\KwIn{IV estimates of mean reward $\theta^1$ and $\theta^2$, denoted $\hat{\theta}^1_{L_2}$ and $\hat{\theta}^2_{L_2}$}
    Let $\hat{\theta}^1_{L_2}$ and $\hat{\theta}^2_{L_2}$ be the IV estimate of the mean reward $\theta^1$ and $\theta^2$ after $L_2\rho$ rounds of Algorithm 1;\\
    Split remainder into consecutive phases of $2h$ rounds each, starting from phase $q = L_2$;\\
    \While{$q < \frac{589824(\log(3T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\tau^2 (\Prob_{\cP_1}[G \geq \tau]^2)}$}
    {\While{$|\hat{\theta}^1_q - \hat{\theta}^2_q| \leq 192\sqrt{\frac{\log(3T/\delta) + 3\log(2T(2+\Upsilon^2))}{q}}$}
    {
    The next $2h$ agents are recommended both arms sequentially;\\
    For each arm $a \in \{1, 2\}$, let $y^a_t$ be one sample reward of that arm in this phase;\\
    Let $\hat{\theta}^a_{q}$ is the IV estimate of the reward of each arm $a \in \{1, 2\}$ for the racing stage up to and including phase $q$;\\
    $q = q+1$;
    }
    For all remaining agents recommend $a^* = \argmax_{a \in {\{1, 2\}}} \hat{\theta}^a_q$ and end the algorithm.} 
    \While{$|\hat{\theta}^1_q - \hat{\theta}^2_q| \leq 192\sqrt{\frac{\log(3T/\delta) + 3\log(2T(2+\Upsilon^2))}{q}}$}
    {
    The next $2h$ agents are recommended both arms sequentially;\\
    For each arm $a \in \{1, 2\}$, let $y^a_q$ be one sample reward of that arm in this phase;\\
    Let $\hat{\theta}^a_{q}$ is the IV estimate of the reward of each arm $a \in \{1, 2\}$ for the racing stage up to and including phase $q$;\\
    $q = q+1$;
    }
    For all remaining agents recommend $a^* = \argmax_{a \in {\{1, 2\}}} \hat{\theta}^a_q$
    \caption{The racing stage for two arms with two heterogeneous types}
    \label{alg:racing-two-types}
\end{algorithm}

% First, we want to determine the threshold needed to declare the winner of the racing stage the best arm overall with high confidence. Similar to the technique used in \cite{active-arms-elimination-2006}, this threshold is determined through the accuracy guarantee of our treatment effect estimate in Theorem \ref{thm:finite-sample}. Once the confidence interval of the estimates $\hat{\theta}^1$ and $\hat{\theta}^2$ stop overlapping, we can declare the arm with higher estimate as the winner of the racing stage. The detail of this analysis is in Lemma $\ref{lemma:stopping criteria}$ below. 
% \begin{lemma} (Stopping Criteria)
% \label{lemma:stopping criteria}
% Given samples of the instrumental variable $z_t$ and response variable $y_t$ from $t$ rounds of the racing stage, we can derive the stopping criteria of the algorithm~\eqref{alg:racing-two-types} at phase $q$:
% \begin{align} 
%     |\hat{\theta}^1_q - \hat{\theta}^2_q| \leq \frac{12\sqrt{\log(2T/\delta) + 3\log(2n(2+\Upsilon^2))}}{\left(p_2 - \sqrt{\frac{\log(1/\delta)}{2n}}\right)^2 \sqrt{q}}.
% \end{align}
% \end{lemma}
% \begin{proof}
% For the algorithm~\eqref{alg:racing-two-types} to successfully find the better arm, we need the deviation bound of the two arms to not overlap. Let the last round that we did not invoke the stopping criteria be $q$, we have
% \begin{align}
%     \abs{\hat{\theta}^1_q - \hat{\theta}^2_q} \leq r_q^1 + r_q^2
% \end{align}
% where $r_q^a$ is the deviation radius of arm $a$ for $a \in \{1, 2\}$ at round $q$.
% We also have:
% \begin{align*}
%     r_q^1 + r_q^2 &= |\hat{\theta}^1_q - \theta^1| + |\hat{\theta}^2_q - \theta^2|\\
%     &\leq 2\norm{\hat{\theta}_q - \theta}_2
% \end{align*}
% From Corollary ~\eqref{cor:finite-sample}, we have:
% \begin{align*}
%     \norm{\hat{\theta}_q - \theta}_2 &\leq  \frac{6\sqrt{\log(2T/\delta) + 3\log(2n(m+\Upsilon^2))}}{\left(p_2 - \sqrt{\frac{\log(1/\delta)}{2n}}\right)^2 \sqrt{n_{\min}}}\\
%     \Rightarrow |\hat{\theta}^1_q - \hat{\theta}^2_q| &\leq \frac{12\sqrt{\log(2T/\delta) + 3\log(2n(m+\Upsilon^2))}}{\left(p_2 - \sqrt{\frac{\log(1/\delta)}{2n}}\right)^2 \sqrt{q}} \ \text{(since $n_{\min} >= q$)}\\
%     &= \frac{12\sqrt{\log(2T/\delta) + 3\log(2n(2+\Upsilon^2))}}{\left(p_2 - \sqrt{\frac{\log(1/\delta)}{2n}}\right)^2 \sqrt{q}} \ \text{(since $m=2$)}
% \end{align*}
% Therefore, the stopping criteria can be rewritten as:
%     \begin{equation}
%         |\hat{\theta}^1_q - \hat{\theta}^2_q| \leq \frac{12\sqrt{\log(2T/\delta) + 3\log(2n(2+\Upsilon^2))}}{\left(p_2 - \sqrt{\frac{\log(1/\delta)}{2n}}\right)^2 \sqrt{q}}
%     \end{equation} 
% \end{proof}
We prove that the Algorithm \ref{alg:racing-two-types} is BIC for all agents of type 2 as long as we have collected sufficient samples of arm 2 in the sampling stage and our estimate of $\theta$ is close to the true treatment effect. Due to information asymmetry, when an agent is recommended arm 2, they do not know whether the two arms are still racing each other or if the best arm has been found. However, with a small enough threshold, the expected gain from exploiting the best arm exceeds the expected loss from exploring a random arm and the agents of type 2 would follow our recommendation. 
\newpage
\begin{restatable}[Type 2 BIC]{lemma}{racingbictwotypes}\label{lemma:racing-bic-two-types}
    Let $\displaystyle G := \theta^2 - \theta^1$. Fix an absolute constant $\tau \in (0, 1)$ and let \[\delta_{\tau} = \frac{1}{4}\frac{\tau \Prob_{\cP_2}[G \geq \tau]}{\tau \Prob_{\cP_2}[G \geq \tau] + 1}.\] Algorithm~\ref{alg:racing-two-types} is BIC for all agents of type 2 if the parameters satisfy $\delta \leq \delta_{\tau}$ and
    \[h \geq -\frac{\log\left(\frac{3\tau \Prob_{\cP_2}[G \geq \tau]+4}{4\tau \Prob_{\cP_2}[G \geq \tau] + 4}\right)}{\log(2)}\] and
    \[L_2 \geq \frac{589824(\log(3T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\tau^2 (\Prob_{\cP_2}[G \geq \tau]^2)}.\]
\end{restatable}

During the first racing stage, we collect more samples of arm 2 through agents of type 2. After getting sufficient samples of arm 2, we can also convince agents of type 1 to follow our recommendations for arm 2. The following Lemma $\ref{lemma:racing-bic-two-types-type-1}$, which follows the same structure as that of Lemma $\ref{lemma:racing-bic-two-types}$, proves that the second racing stage algorithm is BIC for both agents of type 1 and type 2.  

\begin{restatable}[Type 1 BIC]{lemma}{racingbictwotypestypeone}
\label{lemma:racing-bic-two-types-type-1}
Assume two arms. Let $\displaystyle G := \theta^2 - \theta^1$. Fix an absolute constant $\tau \in (0, 1)$ and let \[\delta_{\tau} = \frac{1}{2}\frac{\tau \Prob_{\cP_1}[G \geq \tau]}{\tau \Prob_{\cP_1}[G \geq \tau] + 1}.\] Algorithm~\ref{alg:racing-two-types} is BIC for type 1 in the second part of the racing stage if the parameters satisfy $\delta \leq \delta_{\tau}$ and
\[L_1 := q \geq \frac{589824(\log(3T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\tau^2 (\Prob_{\cP_1}[G \geq \tau]^2)}.\]
\end{restatable}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% REGRET ANALYSIS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Regret Analysis}\label{sec:regret-two-arms-two-types}
With the number of samples of each arm collected in the sampling stage $L_2$, the number of sampling stage phases $\rho$ and the accuracy guarantee of our estimate $\delta$, our sampling stage and racing stage algorithms achieve sub-linear regret for a particular instance of the treatment effect vector $\theta$. Since the priors are not exactly known to the social planner, this ex-post regret is correct for any realization of the priors and treatment effect vector $\theta$.  

\begin{restatable}[Regret]{lemma}{regrettwoarms}\label{lemma:ex-post-2-arm}
    Algorithm 1 and 2 with parameters $L_2, \rho \in \mathbb{N}$ and $\delta \in (0,1)$ achieves ex-post regret:
    \begin{equation}
        R(T) \leq L_2 (\rho + 1) + O(\sqrt{T\log(T/\delta)}) 
    \end{equation}
    where $\Delta = |\theta^1 - \theta^2|$,  $L_2$ is the duration of one phase in the initial sampling stage and $\frac{1}{\rho}$ is the exploration probability in the sampling stage.
\end{restatable}

With the number of samples of each arm collected in the sampling stage $L_2$, the number of sampling stage phases $\rho$, and the accuracy guarantee of our estimate $\delta$, our sampling stage and racing stage algorithms achieve sub-linear Bayesian regret over the randomness in the priors of the agents. Lemma $\ref{lemma:expected-regret-two-arms}$ provides a basic performance guarantee of our algorithm. 
\begin{restatable}[Expected Regret]{lemma}{expectedregrettwoarms}\label{lemma:expected-regret-two-arms}  
    Algorithm with parameters $L_2. \rho \in \mathbb{N}$ and $\delta \in (0,1)$ achieves expected ex-post regret.
    \begin{equation}
        \E[R(T)] = O\left( \sqrt{T\log(T)} \right)
    \end{equation}
    where $T$ is the time horizon.
\end{restatable}

From the regret analyzed in Lemma~\ref{lemma:ex-post-2-arm}, we can derive the type-specific regret of each type of agent. Since our algorithm does not guarantee that all agents follow our recommendations in the sampling stage and the first racing stage, the type-specific regret is divided into two cases, depending on the best arm overall. In addition to the regret in Lemma \ref{lemma:ex-post-2-arm}, this regret also depends on the proportion of each type of agents in the population, which consider to be equal between the two types. Lemma \ref{lemma:type-specific-two-arm} below demonstrates our type-specific regrets guarantee.

\begin{restatable}[Type-specific regret of a partially BIC algorithm]{lemma}{typespecifictwoarms}\label{lemma:type-specific-two-arm} 
   The following type-specific expected regret bounds in Table \ref{tab:type-specific-regret-heterogeneous} hold.
    
   % We observe the following type-specific regret bounds (for confidence $\delta>0$):
    \begin{table}[H]
    \centering
    \begin{tabular}{|l|l|}
    \hline
    Best arm/Type & Type-specific Regret \\ \hline
    Arm 1: Type 1 & $O(\log(T/\delta))$                     \\ \hline
    Arm 1: Type 2 & $O\left(\frac{\log(T/\delta)}{\tau^2 \Prob_{\cP_2}[G \geq \tau]^2}\right) +O(\log(T/\delta))$                     \\ \hline
    Arm 2: Type 1 & $O\left(\frac{\log(T/\delta)}{\tau^2 \Prob_{\cP_2}[G \geq \tau]^2}\right) + O(\sqrt{T\log(T/\delta)})$                     \\ \hline
    Arm 2: Type 2 & $O\left(\frac{\log(T/\delta)}{\tau^2 \Prob_{\cP_2}[G \geq \tau]^2}\right) + O(\sqrt{T\log(T/\delta)})$                     \\ \hline
    \end{tabular}
    \caption{Type-Specific Regret for Two Arms \& Two Types with partially BIC Algorithm}
    \label{tab:type-specific-regret-heterogeneous}
    \end{table}
\end{restatable}

 
% We compare the type-specific regrets of our algorithm to those of a fully BIC algorithm ( Definition~\ref{def:fully-bic-algo}) to demonstrate our advantage in a general setting and a specific realization of the agents' priors.

\begin{definition}\label{def:fully-bic-algo}[Fully BIC Algorithm]
A \textit{fully BIC} algorithm is BIC for all agents at all rounds, similar to the detail-free algorithm in \cite{mansour2015bic}. We implement Sub-algorithm~\eqref{alg:sampling-two-types} to be BIC for agents of type 1 (which will also be BIC for agents of type 2). Then, we run Sub-algorithm~\eqref{alg:racing-two-types} starting from the second racing stage, wherein recommendations are BIC for all agents.
\end{definition}

\begin{remark}[Regret Comparison Between Fully BIC and Partially BIC Algorithms]\label{remark:regret-comparison-2-arm}
The type-specific regret for the fully BIC algorithm (Definition~\ref{def:fully-bic-algo}) is the same as the type-specific regret for our partially BIC algorithm (see Table~\ref{tab:type-specific-regret-heterogeneous}) wherein we replace the prior-dependent constant term $\tau^2 \Prob_{\cP_2}[G \geq \tau]^2$ for type 2 with the prior-dependent constant term $\tau^2 \Prob_{\cP_1}[G \geq \tau]^2$ for type 1, which can be arbitrarily large. In the full version of our paper, we work out a case wherein the priors over the treatment reward vector $\theta$ for each type are Gaussian and the fully BIC algorithm (Definition~\ref{def:fully-bic-algo}) achieves linear regret $\Omega(T)$, but our algorithm achieves sub-linear regret $O(\sqrt{T\log(T)})$.
\end{remark}

\begin{restatable}[Regret comparison with fully BIC algorithm]{lemma}{regretcomparisontwoarms}\label{remark:regret-comparison-2-arm} 
With our Algorithms~\eqref{alg:sampling-two-types} and~\eqref{alg:racing-two-types}, we achieve a better type-specific regret compared to a fully BIC bandit algorithm (an extension of the "detail-free" algorithm in \cite{mansour2015bic}) in the two-arm case.

\begin{table}[ht]
    \centering
\begin{tabular}{|l|l|}
\hline
Best arm/Type & Type-specific Regret \\ \hline
Arm 1: Type 1 &$\frac{294912(\log(3T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\tau^2 (\Prob_{\cP_1}[G \geq \tau]^2)}+O(\sqrt{T\log(T/\delta)})$                      \\ \hline
Arm 1: Type 2 & $\frac{294912(\log(3T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\tau^2 (\Prob_{\cP_1}[G \geq \tau]^2)} +O(\sqrt{T\log(T/\delta)})$                     \\ \hline
Arm 2: Type 1 & $\frac{294912(\log(3T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\tau^2 (\Prob_{\cP_1}[G \geq \tau]^2)} + O(\sqrt{T\log(T/\delta)})$                     \\ \hline
Arm 2: Type 2 & $\frac{294912(\log(3T/\delta) + 3\log(2T(2+\Upsilon^2)))}{\tau^2 (\Prob_{\cP_1}[G \geq \tau]^2)} + O(\sqrt{T\log(T/\delta)})$                     \\ \hline
\end{tabular}
\caption{Type-Specific Regret for Two Arms \& Two Types with Fully BIC Algorithm}
\label{tab:type-specific-regret-fully-bic}
\end{table}
\end{restatable}
